Structured Pruning for Deep Convolutional Neural Networks: A survey

The remarkable performance of deep Convolutional neural networks (CNNs) is generally attributed to their deeper and wider architectures, which can come with significant computational costs. Pruning neural networks has thus gained interest since it effectively lowers storage and computational costs. In contrast to weight pruning, which results in unstructured models, structured pruning provides the benefit of realistic acceleration by producing models that are friendly to hardware implementation. The special requirements of structured pruning have led to the discovery of numerous new challenges and the development of innovative solutions. This article surveys the recent progress towards structured pruning of deep CNNs. We summarize and compare the state-of-the-art structured pruning techniques with respect to filter ranking methods, regularization methods, dynamic execution, neural architecture search, the lottery ticket hypothesis, and the applications of pruning. While discussing structured pruning algorithms, we briefly introduce the unstructured pruning counterpart to emphasize their differences. Furthermore, we provide insights into potential research opportunities in the field of structured pruning. A curated list of neural network pruning papers can be found at https://github.com/he-y/Awesome-Pruning . A dedicated website offering a more interactive comparison of structured pruning methods can be found at: https://huggingface.co/spaces/he-yang/Structured-Pruning-Survey .

==> tables/cifar10/MobileNet.tex <==
\begin{strip}
\centering
\scriptsize
\begin{tabularx}{\textwidth}{@{}>{\hsize=0.067\hsize}X>{\hsize=0.067\hsize}X>{\hsize=0.2\hsize}X>{\hsize=0.067\hsize}X>{\hsize=0.067\hsize}X>{\hsize=0.067\hsize}X>{\hsize=0.067\hsize}X>{\hsize=0.067\hsize}X>{\hsize=0.067\hsize}X>{\hsize=0.067\hsize}X>{\hsize=0.067\hsize}X>{\hsize=0.067\hsize}X>{\hsize=0.067\hsize}X@{}}
\toprule
\tabletitle \\
\midrule
\multicolumn{3}{l}{MobileNet-V1} \\
\midrule
2.3.1 & 2020 & EagleEye~\cite{liEagleEyeFastSubnet2020} & - & 88.01 & - & 34.20 & 3.30 & 90.35 & 4.20 & - & - \\
2.5.2 & 2022 & FTWT~\cite{elkerdawyFireTogetherWire2022} & 90.89 & 91.21 & 0.32 & 34.20 & 7.52 & 78.00 & 4.20 & - & - \\
2.6.2 & 2022 & DAIS~\cite{guanDAISAutomaticChannel2022} & 90.87 & 91.87 & 1.00 & 34.20 & 11.42 & 66.60 & 4.20 & - & - \\
2.3.1 & 2020 & EagleEye~\cite{liEagleEyeFastSubnet2020} & - & 91.44 & - & 34.20 & 12.10 & 64.62 & 4.20 & - & - \\
2.2.3 & 2018 & DCP~\cite{zhuangDiscriminationawareChannelPruning2018} & 93.96 & 94.37 & 0.41 & 34.20 & 19.54 & 42.86 & 4.20 & 2.94 & 30.07 \\
2.3.1 & 2020 & EagleEye~\cite{liEagleEyeFastSubnet2020} & - & 91.89 & - & 34.20 & 26.50 & 22.51 & 4.20 & - & - \\
2.7.3 & 2022 & DPP~\cite{gonzalez-carabarinDynamicProbabilisticPruning2022} & 93.78 & 93.96 & 0.18 & 34.20 & - & - & 4.20 & 1.57 & 62.70 \\
\midrule
\multicolumn{3}{l}{MobileNet-V2} \\
\midrule
2.4.3 & 2022 & StructADMM~\cite{zhangStructADMMAchievingUltrahigh2022} & - & 95.10 & - & 89.00 & 22.82 & 74.36 & 3.50 & - & - \\
2.6.2 & 2022 & DNCP~\cite{zhengModelCompressionBased2022} & 94.15 & 93.30 & -0.85 & 89.00 & 25.00 & 71.91 & 3.50 & - & - \\
2.4.3 & 2022 & EKG~\cite{leeEnsembleKnowledgeGuided2022} & 94.21 & 94.52 & 0.31 & 89.00 & 44.50 & 50.00 & 3.50 & - & - \\
2.3.2 & 2021 & GDP-Guo~\cite{guoGDPStabilizedNeural2021} & 94.89 & 95.15 & 0.26 & 89.00 & 47.86 & 46.22 & 3.50 & - & - \\
2.6.2 & 2022 & DDNP~\cite{gaoDisentangledDifferentiableNetwork2022} & 94.58 & 94.81 & 0.23 & 89.00 & 50.73 & 43.00 & 3.50 & - & - \\
2.6.2 & 2022 & DNCP~\cite{zhengModelCompressionBased2022} & 94.15 & 93.71 & -0.44 & 89.00 & 52.00 & 41.57 & 3.50 & - & - \\
2.3.2 & 2020 & SCOP~\cite{tangSCOPScientificControl2020} & 94.48 & 94.24 & -0.24 & 89.00 & 53.13 & 40.30 & 3.50 & 2.24 & 36.10 \\
2.3.2 & 2020 & DMC~\cite{gaoDiscreteModelCompression2020} & 94.23 & 94.49 & 0.26 & 89.00 & 53.40 & 40.00 & 3.50 & - & - \\
2.3.2 & 2022 & WhiteBox~\cite{zhangCarryingOutCNN2022} & 95.02 & 95.28 & 0.26 & 89.00 & 63.01 & 29.20 & 3.50 & - & - \\
2.2.3 & 2018 & DCP~\cite{zhuangDiscriminationawareChannelPruning2018} & 94.47 & 94.69 & 0.22 & 89.00 & 65.44 & 26.47 & 3.50 & 2.67 & 23.66 \\
\bottomrule
\end{tabularx}

\captionof{table}{MobileNet-V1/V2 on CIFAR-10.}
\end{strip}

==> tables/cifar10/Other.tex <==
\begin{strip}
\centering
\scriptsize
\begin{tabularx}{\textwidth}{@{}>{\hsize=0.067\hsize}X>{\hsize=0.067\hsize}X>{\hsize=0.2\hsize}X>{\hsize=0.067\hsize}X>{\hsize=0.067\hsize}X>{\hsize=0.067\hsize}X>{\hsize=0.067\hsize}X>{\hsize=0.067\hsize}X>{\hsize=0.067\hsize}X>{\hsize=0.067\hsize}X>{\hsize=0.067\hsize}X>{\hsize=0.067\hsize}X>{\hsize=0.067\hsize}X@{}}
\toprule
\tabletitle \\
\midrule
\multicolumn{3}{l}{DenseNet-40} \\
\midrule
2.3.2 & 2019 & GAL~\cite{linOptimalStructuredCNN2019} & 94.81 & 93.23 & -1.58 & 283.00 & 80.91 & 71.41 & 1.04 & 0.26 & 75.00 \\
2.3.2 & 2019 & GAL~\cite{linOptimalStructuredCNN2019} & 94.81 & 91.90 & -2.91 & 283.00 & 80.91 & 71.41 & 1.04 & 0.26 & 75.00 \\
2.3.1 & 2020 & SCP~\cite{kangOperationAwareSoftChannel2020} & 94.39 & 93.77 & 0.62 & 283.00 & 82.72 & 70.77 & 1.04 & 0.26 & 75.41 \\
2.2.1 & 2020 & HRank~\cite{linHRankFilterPruning2020} & 94.81 & 93.68 & -1.13 & 283.00 & 110.54 & 60.94 & 1.04 & 0.48 & 53.85 \\
2.7.2 & 2021 & CC~\cite{liCompactCNNsCollaborative2021} & 94.81 & 94.40 & -0.41 & 283.00 & 112.00 & 60.42 & 1.04 & 0.37 & 64.42 \\
2.4.3 & 2019 & C-SGD~\cite{dingCentripetalSGDPruning2019} & 93.81 & 94.44 & 0.63 & 283.00 & 113.06 & 60.05 & 1.04 & - & - \\
2.3.1 & 2017 & NS~\cite{liuLearningEfficientConvolutional2017} & 93.89 & 94.35 & 0.46 & 283.00 & 127.43 & 54.97 & 1.04 & 0.36 & 65.69 \\
2.3.2 & 2019 & GAL~\cite{linOptimalStructuredCNN2019} & 94.81 & 94.50 & -0.31 & 283.00 & 128.15 & 54.72 & 1.04 & 0.45 & 56.73 \\
2.3.2 & 2019 & GAL~\cite{linOptimalStructuredCNN2019} & 94.81 & 93.53 & -1.28 & 283.00 & 128.15 & 54.72 & 1.04 & 0.45 & 56.73 \\
2.6.1 & 2022 & DECORE~\cite{alwaniDECOREDeepCompression2022} & 94.81 & 94.04 & -0.77 & 283.00 & 128.17 & 54.71 & 1.04 & 0.37 & 64.42 \\
2.7.2 & 2021 & CC~\cite{liCompactCNNsCollaborative2021} & 94.81 & 94.67 & -0.14 & 283.00 & 150.00 & 47.00 & 1.04 & 0.50 & 51.92 \\
2.4.2 & 2019 & VP~\cite{zhaoVariationalConvolutionalNeural2019} & 94.11 & 93.16 & -0.95 & 283.00 & 156.55 & 44.68 & 1.04 & 0.42 & 59.62 \\
2.7.2 & 2020 & Hinge~\cite{liGroupSparsityHinge2020} & 94.74 & 94.67 & -0.07 & 283.00 & 157.35 & 44.40 & 1.04 & 0.75 & 27.54 \\
2.2.1 & 2020 & HRank~\cite{linHRankFilterPruning2020} & 94.81 & 94.24 & -0.57 & 283.00 & 168.00 & 40.63 & 1.04 & 0.66 & 36.54 \\
2.6.1 & 2022 & DECORE~\cite{alwaniDECOREDeepCompression2022} & 94.81 & 94.59 & -0.22 & 283.00 & 171.41 & 39.43 & 1.04 & 0.56 & 46.15 \\
2.3.2 & 2019 & GAL~\cite{linOptimalStructuredCNN2019} & 94.81 & 94.61 & -0.20 & 283.00 & 182.97 & 35.35 & 1.04 & 0.67 & 35.58 \\
2.3.2 & 2019 & GAL~\cite{linOptimalStructuredCNN2019} & 94.81 & 94.29 & -0.52 & 283.00 & 182.97 & 35.35 & 1.04 & 0.67 & 35.58 \\
2.3.1 & 2017 & NS~\cite{liuLearningEfficientConvolutional2017} & 93.89 & 94.81 & 0.92 & 283.00 & 202.29 & 28.52 & 1.04 & 0.67 & 35.29 \\
2.4.1 & 2022 & SOSP~\cite{nonnenmacherSOSPEfficientlyCapturing2022} & 94.58 & 94.41 & -0.17 & 283.00 & 209.02 & 26.14 & 1.04 & 0.68 & 34.78 \\
2.4.1 & 2022 & SOSP~\cite{nonnenmacherSOSPEfficientlyCapturing2022} & 94.58 & 94.42 & -0.16 & 283.00 & 220.66 & 22.03 & 1.04 & 0.71 & 32.21 \\
2.6.1 & 2022 & DECORE~\cite{alwaniDECOREDeepCompression2022} & 94.81 & 94.85 & 0.04 & 283.00 & 229.02 & 19.07 & 1.04 & 0.83 & 20.19 \\
\midrule
\multicolumn{3}{l}{GoogLeNet} \\
\midrule
2.6.1 & 2022 & DECORE~\cite{alwaniDECOREDeepCompression2022} & 95.05 & 94.33 & -0.72 & 1535.00 & 232.27 & 84.87 & 6.17 & 0.86 & 86.02 \\
2.6.1 & 2022 & DECORE~\cite{alwaniDECOREDeepCompression2022} & 95.05 & 94.51 & -0.54 & 1535.00 & 333.26 & 78.29 & 6.17 & 1.17 & 80.98 \\
2.2.1 & 2020 & HRank~\cite{linHRankFilterPruning2020} & 95.05 & 94.07 & -0.98 & 1535.00 & 454.44 & 70.39 & 6.17 & 1.87 & 69.76 \\
2.1.2 & 2022 & CLR-RNF~\cite{linPruningNetworksCrossLayer2022} & 95.03 & 94.85 & -0.18 & 1535.00 & 492.73 & 67.90 & 6.17 & 2.18 & 64.70 \\
2.1.2 & 2022 & EPruner~\cite{linNetworkPruningUsing2022} & 95.05 & 94.99 & -0.06 & 1535.00 & 501.02 & 67.36 & 6.17 & 2.22 & 64.02 \\
2.6.3 & 2020 & ABCPruner~\cite{linChannelPruningAutomatic2020} & 95.05 & 94.84 & -0.21 & 1535.00 & 513.34 & 66.56 & 6.17 & 2.46 & 60.13 \\
2.7.2 & 2021 & CC~\cite{liCompactCNNsCollaborative2021} & 95.05 & 94.88 & -0.17 & 1535.00 & 616.02 & 59.87 & 6.17 & 2.27 & 63.25 \\
2.2.1 & 2020 & HRank~\cite{linHRankFilterPruning2020} & 95.05 & 94.53 & -0.52 & 1535.00 & 696.81 & 54.61 & 6.17 & 2.75 & 55.45 \\
2.7.2 & 2021 & CC~\cite{liCompactCNNsCollaborative2021} & 95.05 & 95.18 & 0.13 & 1535.00 & 767.50 & 50.00 & 6.17 & 2.84 & 53.98 \\
2.3.2 & 2019 & GAL~\cite{linOptimalStructuredCNN2019} & 95.05 & 93.93 & -1.12 & 1535.00 & 949.28 & 38.16 & 6.17 & 3.13 & 49.27 \\
2.3.2 & 2019 & GAL~\cite{linOptimalStructuredCNN2019} & 95.05 & 94.56 & -0.49 & 1535.00 & 949.28 & 38.16 & 6.17 & 3.13 & 49.27 \\
2.6.1 & 2022 & DECORE~\cite{alwaniDECOREDeepCompression2022} & 95.05 & 95.20 & 0.15 & 1535.00 & 1232.04 & 19.74 & 6.17 & 4.75 & 23.09 \\
\\ \midrule
\multicolumn{3}{l}{PreResNet-29} \\
\midrule
2.4.1 & 2019 & ED~\cite{wangEigenDamageStructuredPruning2019} & 94.42 & 89.10 & -5.32 & 41.28 & 3.85 & 90.67 & 0.27 & 0.02 & 93.45 \\
2.4.1 & 2019 & ED~\cite{wangEigenDamageStructuredPruning2019} & 94.42 & 93.80 & -0.62 & 41.28 & 15.22 & 63.13 & 0.27 & 0.08 & 70.09
\\ \midrule
\multicolumn{3}{l}{PreResNet-101} \\
\midrule
2.7.1 & 2020 & EB~\cite{youDrawingEarlyBirdTickets2020} & - & 92.49 & - & 7595.00 & 3452.27 & 54.55 & 44.54 & 13.36 & 70.00 \\
2.7.1 & 2020 & EB~\cite{youDrawingEarlyBirdTickets2020} & - & 93.90 & - & 7595.00 & 5425.00 & 28.57 & 44.54 & 22.27 & 50.00 \\
2.7.1 & 2020 & EB~\cite{youDrawingEarlyBirdTickets2020} & - & 93.91 & - & 7595.00 & 6904.55 & 9.09 & 44.54 & 31.18 & 30.00 \\
\midrule
\multicolumn{3}{l}{ResNeXt-20} \\
\midrule
2.7.2 & 2020 & Hinge~\cite{liGroupSparsityHinge2020} & 92.54 & 91.96 & -0.58 & 36.00 & 21.24 & 41.00 & 0.21 & 0.13 & 36.05 \\
\midrule
\multicolumn{3}{l}{ResNeXt-164} \\
\midrule
2.7.2 & 2020 & Hinge~\cite{liGroupSparsityHinge2020} & 95.18 & 94.87 & -0.31 & 210.00 & 93.28 & 55.58 & 1.70 & 0.86 & 49.47 \\
\midrule
\multicolumn{3}{l}{NAS} \\
\midrule
2.6.2 & 2022 & ReCNAS~\cite{pengReCNASResourceConstrainedNeural2022} & - & 97.48 & - & - & 300 & - & - & 4.10 & - \\
2.6.2 & 2022 & ReCNAS~\cite{pengReCNASResourceConstrainedNeural2022} & - & 97.71 & - & - & 500 & - & - & 5.20 & - \\
\bottomrule
\end{tabularx}

\captionof{table}{Other models on CIFAR-10, including DenseNet-40, GoogLeNet, PreResNet-29/101, ResNeXt-20/164, and models searched
by Neural Architecture Search (NAS).}
\end{strip}

==> tables/cifar10/ResNet-110.tex <==
\begin{strip}
\centering
\scriptsize
\begin{tabularx}{\textwidth}{@{}>{\hsize=0.067\hsize}X>{\hsize=0.067\hsize}X>{\hsize=0.2\hsize}X>{\hsize=0.067\hsize}X>{\hsize=0.067\hsize}X>{\hsize=0.067\hsize}X>{\hsize=0.067\hsize}X>{\hsize=0.067\hsize}X>{\hsize=0.067\hsize}X>{\hsize=0.067\hsize}X>{\hsize=0.067\hsize}X>{\hsize=0.067\hsize}X>{\hsize=0.067\hsize}X@{}}
\toprule
\tabletitle \\
\midrule
\multicolumn{3}{l}{ResNet-110} \\
\midrule
2.2.3 & 2020 & PFP~\cite{liebenweinProvableFilterPruning2020} & 93.57 & 93.21 & -0.36 & 253.15 & 25.92 & 89.76 & 1.73 & 0.14 & 92.07 \\
2.6.1 & 2022 & DECORE~\cite{alwaniDECOREDeepCompression2022} & 93.50 & 92.71 & -0.79 & 253.15 & 58.43 & 76.92 & 1.73 & 0.35 & 79.65 \\
2.2.1 & 2021 & CHIP~\cite{suiCHIPCHannelIndependencebased2021} & 93.50 & 93.63 & 0.13 & 253.15 & 71.89 & 71.60 & 1.73 & 0.55 & 68.30 \\
2.2.1 & 2020 & HRank~\cite{linHRankFilterPruning2020} & 93.50 & 92.65 & -0.85 & 253.15 & 79.38 & 68.64 & 1.73 & 0.53 & 69.19 \\
2.5.2 & 2021 & DDG~\cite{liDynamicDualGating2021} & 94.25 & 93.87 & -0.38 & 253.15 & 83.03 & 67.20 & 1.73 & - & - \\
2.6.3 & 2022 & CCEP~\cite{shangNeuralNetworkPruning2022} & 93.68 & 93.46 & -0.22 & 253.15 & 83.31 & 67.09 & 1.73 & - & - \\
2.3.2 & 2022 & WhiteBox~\cite{zhangCarryingOutCNN2022} & 93.50 & 94.12 & 0.62 & 253.15 & 86.07 & 66.00 & 1.73 & - & - \\
2.1.2 & 2022 & CLR-RNF~\cite{linPruningNetworksCrossLayer2022} & 93.57 & 93.71 & 0.14 & 253.15 & 86.07 & 66.00 & 1.73 & 0.53 & 69.10 \\
2.1.2 & 2022 & EPruner~\cite{linNetworkPruningUsing2022} & 93.50 & 93.62 & 0.12 & 253.15 & 86.31 & 65.91 & 1.73 & 0.41 & 76.30 \\
2.6.3 & 2020 & ABCPruner~\cite{linChannelPruningAutomatic2020} & 93.50 & 93.58 & 0.08 & 253.15 & 88.49 & 65.04 & 1.73 & 0.56 & 67.63 \\
2.2.1 & 2021 & LRMF~\cite{zhangFilterPruningLearned2021} & 93.68 & 93.61 & -0.07 & 253.15 & 94.17 & 62.80 & 1.73 & - & - \\
2.6.2 & 2022 & MFP~\cite{heFilterPruningSwitching2022} & 93.68 & 93.38 & -0.30 & 253.15 & 94.17 & 62.80 & 1.73 & - & - \\
2.6.1 & 2022 & DECORE~\cite{alwaniDECOREDeepCompression2022} & 93.50 & 93.50 & 0.00 & 253.15 & 96.76 & 61.78 & 1.73 & 0.61 & 64.53 \\
2.4.3 & 2019 & C-SGD~\cite{dingCentripetalSGDPruning2019} & 94.38 & 94.44 & 0.06 & 253.15 & 99.01 & 60.89 & 1.73 & - & - \\
2.6.2 & 2020 & LFPC~\cite{heLearningFilterPruning2020} & 93.68 & 93.07 & -0.61 & 253.15 & 100.50 & 60.30 & 1.73 & - & - \\
2.6.2 & 2020 & LFPC~\cite{heLearningFilterPruning2020} & 93.68 & 93.79 & 0.11 & 253.15 & 100.50 & 60.30 & 1.73 & - & - \\
2.6.2 & 2022 & DAIS~\cite{guanDAISAutomaticChannel2022} & 95.62 & 95.02 & -0.60 & 253.15 & 101.26 & 60.00 & 1.73 & - & - \\
2.3.2 & 2021 & ResRep~\cite{dingResRepLosslessCNN2021} & 94.64 & 94.62 & 0.02 & 253.15 & 105.79 & 58.21 & 1.73 & - & - \\
2.5.2 & 2021 & DDG~\cite{liDynamicDualGating2021} & 94.25 & 94.33 & 0.08 & 253.15 & 111.13 & 56.10 & 1.73 & - & - \\
2.6.2 & 2022 & MFP~\cite{heFilterPruningSwitching2022} & 93.68 & 93.31 & -0.37 & 253.15 & 120.75 & 52.30 & 1.73 & - & - \\
2.6.2 & 2022 & MFP~\cite{heFilterPruningSwitching2022} & 93.68 & 93.69 & 0.01 & 253.15 & 120.75 & 52.30 & 1.73 & - & - \\
2.6.2 & 2019 & TAS~\cite{dongNetworkPruningTransformable2019} & 94.97 & 94.33 & -0.64 & 253.15 & 120.75 & 52.30 & 1.73 & - & - \\
2.2.1 & 2021 & LRMF~\cite{zhangFilterPruningLearned2021} & 93.68 & 93.88 & 0.20 & 253.15 & 120.75 & 52.30 & 1.73 & - & - \\
2.1.2 & 2019 & FPGM~\cite{heFilterPruningGeometric2019} & 93.68 & 93.85 & 0.17 & 253.15 & 120.75 & 52.30 & 1.73 & - & - \\
2.2.1 & 2021 & LRMF~\cite{zhangFilterPruningLearned2021} & 93.68 & 93.73 & 0.05 & 253.15 & 120.75 & 52.30 & 1.73 & - & - \\
2.2.1 & 2021 & CHIP~\cite{suiCHIPCHannelIndependencebased2021} & 93.50 & 94.44 & 0.94 & 253.15 & 121.26 & 52.10 & 1.73 & 0.89 & 48.30 \\
2.6.1 & 2022 & GNN-RL~\cite{yuTopologyAwareNetworkPruning2022} & 93.68 & 94.31 & 0.63 & 253.15 & 121.51 & 52.00 & 1.73 & - & - \\
2.5.1 & 2021 & DCP-CAC~\cite{chenDynamicalChannelPruning2021} & 93.38 & 93.86 & 0.48 & 253.15 & 126.52 & 50.02 & 1.73 & 0.89 & 48.84 \\
2.6.1 & 2021 & AGMC~\cite{yuAutoGraphEncoderDecoder2021} & 93.68 & 93.08 & -0.60 & 253.15 & 126.58 & 50.00 & 1.73 & - & - \\
2.3.2 & 2019 & GAL~\cite{linOptimalStructuredCNN2019} & 93.50 & 92.74 & -0.76 & 253.15 & 130.33 & 48.52 & 1.73 & 0.96 & 44.77 \\
2.3.2 & 2019 & GAL~\cite{linOptimalStructuredCNN2019} & 93.50 & 92.55 & -0.95 & 253.15 & 130.33 & 48.52 & 1.73 & 0.96 & 44.77 \\
2.3.2 & 2021 & ABP~\cite{tianAddingPruningSparse2021} & 93.63 & 93.95 & 0.32 & 253.15 & 136.19 & 46.20 & 1.73 & 0.95 & 44.90 \\
2.2.3 & 2018 & NISP~\cite{yuNISPPruningNetworks2018a} & - & - & 0.18 & 253.15 & 142.32 & 43.78 & 1.73 & 0.98 & 43.25 \\
2.7.3 & 2022 & GKP-TMI~\cite{zhongRevisitKernelPruning2022} & 94.26 & 94.90 & 0.64 & 253.15 & 143.51 & 43.31 & 1.73 & 0.98 & 43.52 \\
2.2.1 & 2020 & HRank~\cite{linHRankFilterPruning2020} & 93.50 & 94.23 & 0.73 & 253.15 & 148.85 & 41.20 & 1.73 & 1.05 & 39.53 \\
2.5.1 & 2018 & SFP~\cite{heSoftFilterPruning2018} & 93.68 & 93.38 & -0.30 & 253.15 & 149.86 & 40.80 & 1.73 & - & - \\
2.5.1 & 2018 & SFP~\cite{heSoftFilterPruning2018} & 93.68 & 93.86 & 0.18 & 253.15 & 149.86 & 40.80 & 1.73 & - & - \\
2.1.1 & 2017 & PFEC~\cite{liPruningFiltersEfficient2017} & 93.53 & 93.30 & -0.23 & 253.15 & 155.43 & 38.60 & 1.73 & 1.17 & 32.40 \\
2.4.2 & 2019 & VP~\cite{zhaoVariationalConvolutionalNeural2019} & 93.21 & 92.96 & -0.25 & 253.15 & 160.61 & 36.56 & 1.73 & 1.02 & 41.07 \\
2.6.1 & 2022 & DECORE~\cite{alwaniDECOREDeepCompression2022} & 93.50 & 93.88 & 0.38 & 253.15 & 163.47 & 35.43 & 1.73 & 1.12 & 35.47 \\
2.5.1 & 2021 & DCP-CAC~\cite{chenDynamicalChannelPruning2021} & 93.38 & 94.11 & 0.73 & 253.15 & 176.97 & 30.09 & 1.73 & 1.23 & 29.07 \\
2.5.1 & 2018 & SFP~\cite{heSoftFilterPruning2018} & 93.68 & 93.93 & 0.25 & 253.15 & 181.76 & 28.20 & 1.73 & - & - \\
2.3.2 & 2019 & GAL~\cite{linOptimalStructuredCNN2019} & 93.50 & 93.59 & 0.09 & 253.15 & 205.91 & 18.66 & 1.73 & 1.66 & 4.07 \\
2.3.2 & 2019 & GAL~\cite{linOptimalStructuredCNN2019} & 93.50 & 92.55 & -0.95 & 253.15 & 205.91 & 18.66 & 1.73 & 1.66 & 4.07 \\
2.1.1 & 2017 & PFEC~\cite{liPruningFiltersEfficient2017} & 93.53 & 93.55 & 0.02 & 253.15 & 213.13 & 15.81 & 1.73 & 1.69 & 2.33 \\
\midrule
\multicolumn{3}{l}{ResNet-164} \\
\midrule
2.4.3 & 2019 & C-SGD~\cite{dingCentripetalSGDPruning2019} & 94.83 & 94.75 & -0.08 & 247.65 & 96.81 & 60.91 & 1.70 & - & - \\
2.7.2 & 2020 & Hinge~\cite{liGroupSparsityHinge2020} & 95.18 & 94.60 & -0.58 & 247.65 & 110.01 & 55.58 & 1.70 & 0.86 & 49.47 \\
2.4.2 & 2019 & VP~\cite{zhaoVariationalConvolutionalNeural2019} & 93.58 & 93.16 & -0.42 & 247.65 & 126.21 & 49.04 & 1.70 & 0.74 & 56.55 \\
2.3.1 & 2017 & NS~\cite{liuLearningEfficientConvolutional2017} & 94.58 & 94.73 & 0.15 & 247.65 & 136.48 & 44.89 & 1.70 & 1.10 & 35.29 \\
2.6.2 & 2019 & TAS~\cite{dongNetworkPruningTransformable2019} & 95.47 & 94.00 & -1.47 & 247.65 & 178.06 & 28.10 & 1.70 & - & - \\
2.3.1 & 2017 & NS~\cite{liuLearningEfficientConvolutional2017} & 94.58 & 94.92 & 0.34 & 247.65 & 189.09 & 23.65 & 1.70 & 1.44 & 15.29 \\
\bottomrule
\end{tabularx}

\captionof{table}{ResNet-110/164 on CIFAR-10.}
\end{strip}

==> tables/cifar10/ResNet-20-32.tex <==
\begin{strip}
\centering
\scriptsize
\begin{tabularx}{\textwidth}{@{}>{\hsize=0.067\hsize}X>{\hsize=0.067\hsize}X>{\hsize=0.2\hsize}X>{\hsize=0.067\hsize}X>{\hsize=0.067\hsize}X>{\hsize=0.067\hsize}X>{\hsize=0.067\hsize}X>{\hsize=0.067\hsize}X>{\hsize=0.067\hsize}X>{\hsize=0.067\hsize}X>{\hsize=0.067\hsize}X>{\hsize=0.067\hsize}X>{\hsize=0.067\hsize}X@{}}
\toprule
\tabletitle
\\ \midrule
\multicolumn{3}{l}{ResNet-20}
\\ \midrule
2.6.2 & 2020 & DSA~\cite{ningDSAMoreEfficient2020} & 92.17 & 90.24 & -1.93 & 40.81 & 13.26 & 67.50 & 0.27 & - & - \\
2.7.3 & 2022 & SOKS~\cite{liuSOKSAutomaticSearching2022} & 92.05 & 90.78 & -1.27 & 40.81 & 15.49 & 62.04 & 0.27 & 0.14 & 48.15 \\
2.3.2 & 2020 & SCOP~\cite{tangSCOPScientificControl2020} & 92.22 & 90.75 & -1.47 & 40.81 & 18.08 & 55.70 & 0.27 & 0.12 & 56.30 \\
2.7.2 & 2020 & Hinge~\cite{liGroupSparsityHinge2020} & 92.54 & 91.84 & -0.70 & 40.81 & 18.57 & 54.50 & 0.27 & 0.12 & 55.45 \\
2.5.2 & 2021 & ManiDP~\cite{tangManifoldRegularizedDynamic2021} & 92.22 & 92.05 & -0.17 & 40.81 & 18.69 & 54.20 & 0.27 & - & - \\
2.2.1 & 2021 & LRMF~\cite{zhangFilterPruningLearned2021} & 92.20 & 90.47 & -1.73 & 40.81 & 18.77 & 54.00 & 0.27 & - & - \\
2.1.2 & 2019 & FPGM~\cite{heFilterPruningGeometric2019} & 92.20 & 91.99 & -0.21 & 40.81 & 18.77 & 54.00 & 0.27 & - & - \\
2.5.2 & 2021 & DDG~\cite{liDynamicDualGating2021} & 92.24 & 91.90 & -0.34 & 40.81 & 19.43 & 52.40 & 0.27 & - & - \\
2.6.2 & 2022 & DAIS~\cite{guanDAISAutomaticChannel2022} & 93.25 & 92.89 & -0.36 & 40.81 & 19.96 & 51.10 & 0.27 & - & - \\
2.6.1 & 2022 & GNN-RL~\cite{yuTopologyAwareNetworkPruning2022} & 91.73 & 91.31 & -0.42 & 40.81 & 20.00 & 51.00 & 0.27 & - & - \\
2.2.1 & 2022 & GCNP~\cite{jiangChannelPruningUsing2022} & 92.25 & 91.58 & -0.67 & 40.81 & 20.18 & 50.54 & 0.27 & 0.17 & 38.51 \\
2.6.2 & 2020 & DSA~\cite{ningDSAMoreEfficient2020} & 92.17 & 91.38 & -0.79 & 40.81 & 20.28 & 50.30 & 0.27 & - & - \\
2.6.1 & 2021 & AGMC~\cite{yuAutoGraphEncoderDecoder2021} & 91.73 & 91.42 & -0.31 & 40.81 & 20.41 & 50.00 & 0.27 & - & - \\
2.3.2 & 2021 & ABP~\cite{tianAddingPruningSparse2021} & 92.15 & 91.03 & -1.12 & 40.81 & 21.34 & 47.70 & 0.27 & 0.15 & 45.10 \\
2.1.2 & 2021 & SRR~\cite{wangConvolutionalNeuralNetwork2021} & 92.27 & 92.48 & 0.21 & 40.81 & 22.12 & 45.80 & 0.27 & - & - \\
2.2.3 & 2020 & PFP~\cite{liebenweinProvableFilterPruning2020} & 91.40 & 90.91 & -0.49 & 40.81 & 22.26 & 45.46 & 0.27 & 0.10 & 62.67 \\
2.6.2 & 2019 & TAS~\cite{dongNetworkPruningTransformable2019} & 92.88 & 92.88 & 0.00 & 40.81 & 22.45 & 45.00 & 0.27 & - & - \\
2.7.3 & 2022 & GKP-TMI~\cite{zhongRevisitKernelPruning2022} & 92.35 & 92.01 & -0.34 & 40.81 & 23.30 & 42.90 & 0.27 & 0.15 & 43.40 \\
2.5.2 & 2021 & DDG~\cite{liDynamicDualGating2021} & 92.24 & 92.27 & 0.03 & 40.81 & 23.38 & 42.70 & 0.27 & - & - \\
2.5.1 & 2018 & SFP~\cite{heSoftFilterPruning2018} & 92.20 & 90.83 & -1.37 & 40.81 & 23.59 & 42.20 & 0.27 & - & - \\
2.2.1 & 2021 & LRMF~\cite{zhangFilterPruningLearned2021} & 92.20 & 91.04 & -1.16 & 40.81 & 23.59 & 42.20 & 0.27 & - & - \\
2.7.3 & 2022 & SOKS~\cite{liuSOKSAutomaticSearching2022} & 92.05 & 91.83 & -0.22 & 40.81 & 23.63 & 42.09 & 0.27 & 0.16 & 40.74 \\
2.2.1 & 2022 & GCNP~\cite{jiangChannelPruningUsing2022} & 92.25 & 92.22 & -0.03 & 40.81 & 28.38 & 30.47 & 0.27 & 0.20 & 27.42 \\
2.5.1 & 2018 & SFP~\cite{heSoftFilterPruning2018} & 92.20 & 91.20 & -1.00 & 40.81 & 28.85 & 29.30 & 0.27 & - & - \\
2.6.2 & 2020 & DSA~\cite{ningDSAMoreEfficient2020} & 92.17 & 92.10 & -0.07 & 40.81 & 30.20 & 26.00 & 0.27 & - & - \\
2.4.2 & 2019 & VP~\cite{zhaoVariationalConvolutionalNeural2019} & 92.01 & 91.66 & -0.35 & 40.81 & 34.39 & 15.73 & 0.27 & 0.22 & 19.05
\\ \midrule
\multicolumn{3}{l}{ResNet-32}
\\ \midrule
2.4.1 & 2019 & ED~\cite{wangEigenDamageStructuredPruning2019} & 95.30 & 93.05 & -2.25 & 69.12 & 3.64 & 94.74 & 0.47 & 0.02 & 96.05 \\
2.4.1 & 2019 & ED~\cite{wangEigenDamageStructuredPruning2019} & 95.30 & 95.17 & -0.13 & 69.12 & 20.56 & 70.25 & 0.47 & 0.13 & 71.99 \\
2.4.1 & 2022 & SOSP~\cite{nonnenmacherSOSPEfficientlyCapturing2022} & 95.30 & 95.22 & -0.08 & 69.12 & 22.22 & 67.85 & 0.47 & 0.13 & 72.85 \\
2.4.1 & 2022 & SOSP~\cite{nonnenmacherSOSPEfficientlyCapturing2022} & 95.30 & 95.06 & -0.24 & 69.12 & 22.56 & 67.36 & 0.47 & 0.13 & 72.33 \\
2.5.2 & 2021 & ManiDP~\cite{tangManifoldRegularizedDynamic2021} & 92.66 & 92.15 & -0.51 & 69.12 & 25.44 & 63.20 & 0.47 & - & - \\
2.3.2 & 2020 & SCOP~\cite{tangSCOPScientificControl2020} & 92.66 & 92.13 & -0.53 & 69.12 & 30.55 & 55.80 & 0.47 & 0.21 & 56.20 \\
2.7.3 & 2022 & SOKS~\cite{liuSOKSAutomaticSearching2022} & 92.82 & 92.02 & -0.80 & 69.12 & 31.39 & 54.58 & 0.47 & 0.21 & 54.35 \\
2.5.2 & 2021 & DDG~\cite{liDynamicDualGating2021} & 93.22 & 92.96 & -0.26 & 69.12 & 31.52 & 54.40 & 0.47 & - & - \\
2.6.2 & 2022 & DAIS~\cite{guanDAISAutomaticChannel2022} & 92.92 & 93.49 & 0.57 & 69.12 & 31.86 & 53.90 & 0.47 & - & - \\
2.1.2 & 2019 & COP~\cite{wangCOPCustomizedDeep2019} & 92.64 & 91.97 & -0.67 & 69.12 & 31.86 & 53.90 & 0.47 & 0.20 & 57.50 \\
2.6.2 & 2022 & MFP~\cite{heFilterPruningSwitching2022} & 92.63 & 91.85 & -0.78 & 69.12 & 32.35 & 53.20 & 0.47 & - & - \\
2.2.1 & 2021 & LRMF~\cite{zhangFilterPruningLearned2021} & 92.63 & 92.08 & -0.55 & 69.12 & 32.35 & 53.20 & 0.47 & - & - \\
2.2.1 & 2021 & LRMF~\cite{zhangFilterPruningLearned2021} & 92.63 & 92.08 & -0.55 & 69.12 & 32.35 & 53.20 & 0.47 & - & - \\
2.1.2 & 2019 & FPGM~\cite{heFilterPruningGeometric2019} & 92.63 & 92.82 & 0.19 & 69.12 & 32.35 & 53.20 & 0.47 & - & - \\
2.6.2 & 2020 & LFPC~\cite{heLearningFilterPruning2020} & 92.63 & 92.12 & -0.51 & 69.12 & 32.76 & 52.60 & 0.47 & - & - \\
2.6.1 & 2022 & GNN-RL~\cite{yuTopologyAwareNetworkPruning2022} & 92.63 & 92.58 & -0.05 & 69.12 & 33.87 & 51.00 & 0.47 & - & - \\
2.5.1 & 2021 & DCP-CAC~\cite{chenDynamicalChannelPruning2021} & 92.36 & 92.21 & -0.15 & 69.12 & 34.49 & 50.10 & 0.47 & 0.25 & 47.83 \\
2.6.1 & 2021 & AGMC~\cite{yuAutoGraphEncoderDecoder2021} & 92.63 & 90.96 & -1.67 & 69.12 & 34.56 & 50.00 & 0.47 & - & - \\
2.6.2 & 2019 & TAS~\cite{dongNetworkPruningTransformable2019} & 93.89 & 93.16 & -0.73 & 69.12 & 34.97 & 49.40 & 0.47 & - & - \\
2.7.3 & 2022 & SOKS~\cite{liuSOKSAutomaticSearching2022} & 92.82 & 92.44 & -0.38 & 69.12 & 36.74 & 46.85 & 0.47 & 0.27 & 43.48 \\
2.3.2 & 2021 & ABP~\cite{tianAddingPruningSparse2021} & 92.63 & 92.55 & -0.08 & 69.12 & 37.12 & 46.30 & 0.47 & 0.27 & 43.60 \\
2.5.2 & 2021 & DDG~\cite{liDynamicDualGating2021} & 93.22 & 93.21 & -0.01 & 69.12 & 39.12 & 43.40 & 0.47 & - & - \\
2.7.3 & 2022 & GKP-TMI~\cite{zhongRevisitKernelPruning2022} & 92.82 & 93.04 & 0.22 & 69.12 & 39.33 & 43.10 & 0.47 & 0.27 & 43.40 \\
2.5.1 & 2018 & SFP~\cite{heSoftFilterPruning2018} & 92.63 & 90.08 & -2.55 & 69.12 & 40.44 & 41.50 & 0.47 & - & - \\
2.5.1 & 2021 & DCP-CAC~\cite{chenDynamicalChannelPruning2021} & 92.36 & 92.85 & 0.49 & 69.12 & 48.35 & 30.04 & 0.47 & 0.35 & 26.09 \\
2.5.1 & 2018 & SFP~\cite{heSoftFilterPruning2018} & 92.63 & 90.63 & -2.00 & 69.12 & 49.21 & 28.80 & 0.47 & - & - \\
\midrule
\multicolumn{3}{l}{ResNet-44} \\
\midrule
2.5.1 & 2021 & DCP-CAC~\cite{chenDynamicalChannelPruning2021} & 92.45 & 92.42 & -0.03 & 97.15 & 48.54 & 50.04 & 0.66 & 0.35 & 47.69 \\
2.6.1 & 2021 & AGMC~\cite{yuAutoGraphEncoderDecoder2021} & 93.10 & 92.28 & -0.82 & 97.15 & 48.58 & 50.00 & 0.66 & - & - \\
2.5.1 & 2021 & DCP-CAC~\cite{chenDynamicalChannelPruning2021} & 92.45 & 93.26 & 0.81 & 97.15 & 67.98 & 30.03 & 0.66 & 0.46 & 30.77 \\
\bottomrule
\end{tabularx}

\captionof{table}{ResNet-20/32/44 on CIFAR-10.}

\end{strip}

==> tables/cifar10/ResNet-56-cont.tex <==
\begin{strip}
\centering
\scriptsize
\begin{tabularx}{\textwidth}{@{}>{\hsize=0.067\hsize}X>{\hsize=0.067\hsize}X>{\hsize=0.2\hsize}X>{\hsize=0.067\hsize}X>{\hsize=0.067\hsize}X>{\hsize=0.067\hsize}X>{\hsize=0.067\hsize}X>{\hsize=0.067\hsize}X>{\hsize=0.067\hsize}X>{\hsize=0.067\hsize}X>{\hsize=0.067\hsize}X>{\hsize=0.067\hsize}X>{\hsize=0.067\hsize}X@{}}
\toprule
\tabletitle \\
\midrule
\multicolumn{3}{l}{ResNet-56 (cont.)}
\\ \midrule
2.6.2 & 2020 & LFPC~\cite{heLearningFilterPruning2020} & 93.59 & 93.56 & -0.03 & 125.75 & 66.52 & 47.10 & 0.86 & - & - \\
2.2.3 & 2018 & DCP~\cite{zhuangDiscriminationawareChannelPruning2018} & 93.80 & 93.81 & 0.01 & 125.75 & 66.53 & 47.09 & 0.86 & 0.26 & 70.33 \\
2.4.1 & 2019 & CCP~\cite{pengCollaborativeChannelPruning2019} & 93.50 & - & -0.19 & 125.75 & 66.65 & 47.00 & 0.86 & - & - \\
2.3.1 & 2020 & PR~\cite{zhuangNeuronlevelStructuredPruning2020} & 93.80 & 93.83 & -0.03 & 125.75 & 66.65 & 47.00 & 0.86 & - & - \\
2.3.2 & 2021 & ABP~\cite{tianAddingPruningSparse2021} & 93.41 & 93.10 & -0.31 & 125.75 & 68.91 & 45.20 & 0.86 & 0.47 & 45.70 \\
2.2.3 & 2018 & NISP~\cite{yuNISPPruningNetworks2018a} & - & - & 0.03 & 125.75 & 70.91 & 43.61 & 0.86 & 0.49 & 42.60 \\
2.7.3 & 2022 & GKP-TMI~\cite{zhongRevisitKernelPruning2022} & 93.78 & 94.00 & 0.22 & 125.75 & 71.39 & 43.23 & 0.86 & 0.49 & 43.49 \\
2.7.2 & 2021 & CC~\cite{liCompactCNNsCollaborative2021} & 93.33 & 93.87 & 0.54 & 125.75 & 72.43 & 42.40 & 0.86 & 0.55 & 36.47 \\
2.5.1 & 2018 & SFP~\cite{heSoftFilterPruning2018} & 93.59 & 93.78 & 0.19 & 125.75 & 74.07 & 41.10 & 0.86 & - & - \\
2.5.1 & 2018 & SFP~\cite{heSoftFilterPruning2018} & 93.59 & 93.10 & -0.49 & 125.75 & 74.07 & 41.10 & 0.86 & - & - \\
2.4.1 & 2022 & HAP~\cite{yuHessianAwarePruningOptimal2022} & 93.88 & 93.55 & 0.33 & 125.75 & 74.57 & 40.70 & 0.86 & - & - \\
2.3.2 & 2019 & GAL~\cite{linOptimalStructuredCNN2019} & 93.26 & 93.38 & 0.12 & 125.75 & 78.46 & 37.60 & 0.86 & 0.76 & 11.76 \\
2.3.2 & 2019 & GAL~\cite{linOptimalStructuredCNN2019} & 93.26 & 92.98 & -0.28 & 125.75 & 78.46 & 37.60 & 0.86 & 0.76 & 11.76 \\
2.7.3 & 2022 & SOKS~\cite{liuSOKSAutomaticSearching2022} & 93.06 & 93.22 & 0.16 & 125.75 & 80.60 & 35.91 & 0.86 & 0.52 & 40.00 \\
2.7.3 & 2019 & SDN~\cite{chenShallowingDeepNetworks2019} & 93.03 & 93.29 & 0.26 & 125.75 & 81.99 & 34.80 & 0.86 & 0.50 & 42.30 \\
2.5.1 & 2021 & SEP~\cite{dingWherePruneUsing2021} & 93.04 & 94.05 & 1.01 & 125.75 & 82.89 & 34.08 & 0.86 & 0.62 & 27.91 \\
2.5.1 & 2021 & DCP-CAC~\cite{chenDynamicalChannelPruning2021} & 92.88 & 93.47 & 0.59 & 125.75 & 88.01 & 30.01 & 0.86 & 0.60 & 30.59 \\
2.3.2 & 2020 & LeGR~\cite{chinEfficientModelCompression2020} & 93.90 & 94.10 & 0.20 & 125.75 & 88.02 & 30.00 & 0.86 & - & - \\
2.2.1 & 2020 & HRank~\cite{linHRankFilterPruning2020} & 93.26 & 93.52 & 0.26 & 125.75 & 88.90 & 29.30 & 0.86 & 0.72 & 16.47 \\
2.6.2 & 2020 & DSA~\cite{ningDSAMoreEfficient2020} & 93.12 & 93.08 & -0.04 & 125.75 & 88.91 & 29.30 & 0.86 & - & - \\
2.1.1 & 2017 & PFEC~\cite{liPruningFiltersEfficient2017} & 93.04 & 93.06 & 0.02 & 125.75 & 91.04 & 27.60 & 0.86 & 0.74 & 13.73 \\
2.6.1 & 2022 & DECORE~\cite{alwaniDECOREDeepCompression2022} & 93.26 & 93.34 & 0.08 & 125.75 & 92.67 & 26.30 & 0.86 & 0.65 & 24.71 \\
2.4.1 & 2022 & HAP~\cite{yuHessianAwarePruningOptimal2022} & 93.88 & 92.92 & 0.96 & 125.75 & 95.70 & 23.90 & 0.86 & - & - \\
2.4.2 & 2019 & VP~\cite{zhaoVariationalConvolutionalNeural2019} & 93.04 & 92.26 & -0.78 & 125.75 & 100.37 & 20.18 & 0.86 & 0.69 & 19.30 \\
2.1.1 & 2017 & PFEC~\cite{liPruningFiltersEfficient2017} & 93.04 & 93.10 & 0.06 & 125.75 & 112.67 & 10.40 & 0.86 & 0.78 & 9.41 \\
\bottomrule
\end{tabularx}

\captionof{table}{ResNet-56 on CIFAR-10. (Part 2)}
\end{strip}

==> tables/cifar10/ResNet-56.tex <==
\begin{strip}
\centering
\scriptsize
\begin{tabularx}{\textwidth}{@{}>{\hsize=0.067\hsize}X>{\hsize=0.067\hsize}X>{\hsize=0.2\hsize}X>{\hsize=0.067\hsize}X>{\hsize=0.067\hsize}X>{\hsize=0.067\hsize}X>{\hsize=0.067\hsize}X>{\hsize=0.067\hsize}X>{\hsize=0.067\hsize}X>{\hsize=0.067\hsize}X>{\hsize=0.067\hsize}X>{\hsize=0.067\hsize}X>{\hsize=0.067\hsize}X@{}}
\toprule
\tabletitle \\
\midrule
\multicolumn{3}{l}{ResNet-56} \\
\midrule
2.2.3 & 2020 & PFP~\cite{liebenweinProvableFilterPruning2020} & 92.95 & 92.67 & -0.28 & 125.75 & 19.59 & 84.42 & 0.86 & 0.09 & 88.98 \\
2.6.1 & 2022 & DECORE~\cite{alwaniDECOREDeepCompression2022} & 93.26 & 90.85 & -2.41 & 125.75 & 23.27 & 81.50 & 0.86 & 0.13 & 84.71 \\
2.3.2 & 2021 & ResRep~\cite{dingResRepLosslessCNN2021} & 93.71 & 92.66 & 1.05 & 125.75 & 27.88 & 77.83 & 0.86 & - & - \\
2.2.1 & 2022 & GCNP~\cite{jiangChannelPruningUsing2022} & 93.72 & 92.75 & -0.97 & 125.75 & 28.65 & 77.22 & 0.86 & 0.25 & 70.50 \\
2.7.2 & 2020 & Hinge~\cite{liGroupSparsityHinge2020} & 92.95 & 92.65 & -0.30 & 125.75 & 30.18 & 76.00 & 0.86 & 0.18 & 79.20 \\
2.7.3 & 2020 & SWP~\cite{mengPruningFilterFilter2020} & 93.10 & 92.98 & -0.12 & 125.75 & 30.68 & 75.60 & 0.86 & 0.19 & 77.70 \\
2.2.1 & 2020 & HRank~\cite{linHRankFilterPruning2020} & 93.26 & 90.72 & -2.54 & 125.75 & 32.59 & 74.09 & 0.86 & 0.27 & 68.24 \\
2.2.1 & 2021 & CHIP~\cite{suiCHIPCHannelIndependencebased2021} & 93.26 & 92.05 & -1.21 & 125.75 & 34.83 & 72.30 & 0.86 & 0.24 & 71.80 \\
2.6.2 & 2022 & DAIS~\cite{guanDAISAutomaticChannel2022} & 92.53 & 93.53 & 1.00 & 125.75 & 36.59 & 70.90 & 0.86 & - & - \\
2.3.1 & 2019 & GBN~\cite{youGateDecoratorGlobal2019} & - & - & 0.03 & 125.75 & 37.35 & 70.30 & 0.86 & 0.29 & 66.70 \\
2.6.2 & 2020 & DSA~\cite{ningDSAMoreEfficient2020} & 93.12 & 92.20 & -0.92 & 125.75 & 40.99 & 67.40 & 0.86 & - & - \\
2.5.2 & 2022 & FTWT~\cite{elkerdawyFireTogetherWire2022} & 93.66 & 92.63 & -1.03 & 125.75 & 42.75 & 66.00 & 0.86 & - & - \\
2.3.2 & 2021 & GDP-Guo~\cite{guoGDPStabilizedNeural2021} & 93.90 & 93.55 & -0.35 & 125.75 & 43.21 & 65.64 & 0.86 & - & - \\
2.4.3 & 2022 & EKG~\cite{leeEnsembleKnowledgeGuided2022} & 93.84 & 93.69 & -0.15 & 125.75 & 43.87 & 65.11 & 0.86 & - & - \\
2.6.3 & 2022 & CCEP~\cite{shangNeuralNetworkPruning2022} & 93.48 & 93.24 & -0.24 & 125.75 & 46.00 & 63.42 & 0.86 & - & - \\
2.5.2 & 2021 & ManiDP~\cite{tangManifoldRegularizedDynamic2021} & 93.70 & 93.64 & -0.06 & 125.75 & 47.28 & 62.40 & 0.86 & - & - \\
2.1.2 & 2022 & EPruner~\cite{linNetworkPruningUsing2022} & 93.26 & 93.18 & -0.08 & 125.75 & 48.63 & 61.33 & 0.86 & 0.39 & 54.12 \\
2.4.3 & 2019 & C-SGD~\cite{dingCentripetalSGDPruning2019} & 93.39 & 93.44 & 0.05 & 125.75 & 49.23 & 60.85 & 0.86 & - & - \\
2.3.3 & 2021 & GREG~\cite{wangNeuralPruningGrowing2022} & 93.36 & 93.36 & 0.00 & 125.75 & 49.32 & 60.78 & 0.86 & - & - \\
2.3.3 & 2021 & GREG~\cite{wangNeuralPruningGrowing2022} & 93.36 & 93.18 & -0.18 & 125.75 & 49.32 & 60.78 & 0.86 & - & - \\
2.3.2 & 2019 & GAL~\cite{linOptimalStructuredCNN2019} & 93.26 & 91.58 & -1.68 & 125.75 & 50.09 & 60.16 & 0.86 & 0.29 & 65.88 \\
2.3.2 & 2019 & GAL~\cite{linOptimalStructuredCNN2019} & 93.26 & 90.36 & -2.90 & 125.75 & 50.09 & 60.16 & 0.86 & 0.29 & 65.88 \\
2.3.1 & 2019 & GBN~\cite{youGateDecoratorGlobal2019} & - & - & -0.33 & 125.75 & 50.17 & 60.10 & 0.86 & 0.40 & 53.50 \\
2.7.2 & 2021 & EDP~\cite{ruanEDPEfficientDecomposition2021} & 93.61 & 93.61 & 0.00 & 125.75 & 53.18 & 57.71 & 0.86 & 0.39 & 54.18 \\
2.1.2 & 2022 & CLR-RNF~\cite{linPruningNetworksCrossLayer2022} & 93.26 & 93.27 & 0.01 & 125.75 & 53.70 & 57.30 & 0.86 & 0.38 & 55.50 \\
2.3.2 & 2020 & SCOP~\cite{tangSCOPScientificControl2020} & 93.70 & 93.64 & -0.06 & 125.75 & 55.33 & 56.00 & 0.86 & 0.38 & 56.30 \\
2.6.2 & 2021 & EE~\cite{zhangExplorationEstimationModel2021} & 93.62 & 93.68 & 0.06 & 125.75 & 55.33 & 56.00 & 0.86 & - & - \\
2.3.2 & 2022 & WhiteBox~\cite{zhangCarryingOutCNN2022} & 93.26 & 93.54 & 0.28 & 125.75 & 55.83 & 55.60 & 0.86 & - & - \\
2.6.1 & 2022 & RL-MCTS~\cite{wangChannelPruningLookahead2022} & 93.20 & 93.56 & 0.36 & 125.75 & 56.59 & 55.00 & 0.86 & - & - \\
2.6.3 & 2020 & ABCPruner~\cite{linChannelPruningAutomatic2020} & 93.26 & 93.23 & -0.03 & 125.75 & 57.68 & 54.13 & 0.86 & 0.39 & 54.12 \\
2.6.1 & 2022 & GNN-RL~\cite{yuTopologyAwareNetworkPruning2022} & 93.39 & 93.49 & 0.10 & 125.75 & 57.84 & 54.00 & 0.86 & - & - \\
2.5.2 & 2022 & FTWT~\cite{elkerdawyFireTogetherWire2022} & 93.66 & 92.28 & -1.38 & 125.75 & 57.84 & 54.00 & 0.86 & - & - \\
2.1.2 & 2021 & SRR~\cite{wangConvolutionalNeuralNetwork2021} & 93.38 & 93.75 & 0.37 & 125.75 & 58.10 & 53.80 & 0.86 & - & - \\
2.3.2 & 2021 & GDP-Guo~\cite{guoGDPStabilizedNeural2021} & 93.90 & 93.97 & 0.07 & 125.75 & 58.66 & 53.35 & 0.86 & - & - \\
2.3.2 & 2020 & LeGR~\cite{chinEfficientModelCompression2020} & 93.90 & 93.70 & -0.20 & 125.75 & 59.10 & 53.00 & 0.86 & - & - \\
2.3.2 & 2021 & ResRep~\cite{dingResRepLosslessCNN2021} & 93.71 & 93.71 & 0.00 & 125.75 & 59.22 & 52.91 & 0.86 & - & - \\
2.6.2 & 2020 & LFPC~\cite{heLearningFilterPruning2020} & 93.59 & 93.34 & -0.25 & 125.75 & 59.23 & 52.90 & 0.86 & - & - \\
2.6.2 & 2020 & LFPC~\cite{heLearningFilterPruning2020} & 93.59 & 93.24 & -0.35 & 125.75 & 59.23 & 52.90 & 0.86 & - & - \\
2.6.2 & 2019 & TAS~\cite{dongNetworkPruningTransformable2019} & 94.46 & 93.69 & -0.77 & 125.75 & 59.48 & 52.70 & 0.86 & - & - \\
2.6.2 & 2022 & MFP~\cite{heFilterPruningSwitching2022} & 93.59 & 93.56 & -0.03 & 125.75 & 59.61 & 52.60 & 0.86 & - & - \\
2.6.2 & 2022 & MFP~\cite{heFilterPruningSwitching2022} & 93.59 & 92.76 & -0.83 & 125.75 & 59.61 & 52.60 & 0.86 & - & - \\
2.5.1 & 2018 & SFP~\cite{heSoftFilterPruning2018} & 93.59 & 93.35 & -0.24 & 125.75 & 59.61 & 52.60 & 0.86 & - & - \\
2.5.1 & 2018 & SFP~\cite{heSoftFilterPruning2018} & 93.59 & 92.26 & -1.33 & 125.75 & 59.61 & 52.60 & 0.86 & - & - \\
2.4.1 & 2019 & CCP~\cite{pengCollaborativeChannelPruning2019} & 93.50 & - & 0.08 & 125.75 & 59.61 & 52.60 & 0.86 & - & - \\
2.2.1 & 2021 & LRMF~\cite{zhangFilterPruningLearned2021} & 93.59 & 93.25 & -0.34 & 125.75 & 59.61 & 52.60 & 0.86 & - & - \\
2.2.1 & 2021 & LRMF~\cite{zhangFilterPruningLearned2021} & 93.59 & 93.29 & -0.30 & 125.75 & 59.61 & 52.60 & 0.86 & - & - \\
2.1.2 & 2019 & FPGM~\cite{heFilterPruningGeometric2019} & 93.59 & 93.49 & -0.10 & 125.75 & 59.61 & 52.60 & 0.86 & - & - \\
2.2.3 & 2022 & DLRFC~\cite{heFilterPruningFeature2022} & 93.06 & 93.57 & -0.51 & 125.75 & 59.63 & 52.58 & 0.86 & 0.38 & 55.63 \\
2.6.2 & 2020 & DSA~\cite{ningDSAMoreEfficient2020} & 93.12 & 92.91 & -0.21 & 125.75 & 60.11 & 52.20 & 0.86 & - & - \\
2.7.2 & 2021 & CC~\cite{liCompactCNNsCollaborative2021} & 93.33 & 93.64 & 0.31 & 125.75 & 60.36 & 52.00 & 0.86 & 0.45 & 48.24 \\
2.7.3 & 2022 & SOKS~\cite{liuSOKSAutomaticSearching2022} & 93.06 & 93.08 & 0.02 & 125.75 & 60.70 & 51.73 & 0.86 & 0.39 & 54.12 \\
2.3.1 & 2020 & SCP~\cite{kangOperationAwareSoftChannel2020} & 93.69 & 93.23 & 0.46 & 125.75 & 60.99 & 51.50 & 0.86 & 0.44 & 48.47 \\
2.6.2 & 2022 & DDNP~\cite{gaoDisentangledDifferentiableNetwork2022} & 93.62 & 93.83 & 0.21 & 125.75 & 61.62 & 51.00 & 0.86 & - & - \\
2.3.1 & 2020 & EagleEye~\cite{liEagleEyeFastSubnet2020} & - & 94.66 & - & 125.75 & 62.23 & 50.51 & 0.86 & - & - \\
2.5.1 & 2021 & DCP-CAC~\cite{chenDynamicalChannelPruning2021} & 92.88 & 93.10 & 0.22 & 125.75 & 62.82 & 50.04 & 0.86 & 0.44 & 49.41 \\
2.2.1 & 2020 & HRank~\cite{linHRankFilterPruning2020} & 93.26 & 93.17 & -0.09 & 125.75 & 62.85 & 50.02 & 0.86 & 0.50 & 42.35 \\
2.3.2 & 2020 & DMC~\cite{gaoDiscreteModelCompression2020} & 93.62 & 93.69 & 0.07 & 125.75 & 62.88 & 50.00 & 0.86 & - & - \\
2.6.1 & 2018 & AMC~\cite{heAMCAutoMLModel2018} & 92.80 & 90.10 & -2.70 & 125.75 & 62.88 & 50.00 & 0.86 & - & - \\
2.4.3 & 2022 & EKG~\cite{leeEnsembleKnowledgeGuided2022} & 93.84 & 94.09 & 0.25 & 125.75 & 62.88 & 50.00 & 0.86 & - & - \\
2.6.1 & 2021 & AGMC~\cite{yuAutoGraphEncoderDecoder2021} & 93.39 & 92.76 & -0.63 & 125.75 & 62.88 & 50.00 & 0.86 & - & - \\
2.7.2 & 2020 & Hinge~\cite{liGroupSparsityHinge2020} & 92.95 & 93.69 & 0.74 & 125.75 & 62.88 & 50.00 & 0.86 & 0.42 & 51.27 \\
2.6.1 & 2018 & AMC~\cite{heAMCAutoMLModel2018} & 92.80 & 91.90 & -0.90 & 125.75 & 62.88 & 50.00 & 0.86 & - & - \\
2.4.3 & 2022 & RollBack~\cite{fanBayesianOptimizationClustering2022} & - & 92.53 & - & 125.75 & 62.88 & 50.00 & 0.86 & - & - \\
2.6.1 & 2022 & DECORE~\cite{alwaniDECOREDeepCompression2022} & 93.26 & 93.26 & 0.00 & 125.75 & 63.06 & 49.85 & 0.86 & 0.44 & 49.41 \\
2.2.3 & 2018 & DCP~\cite{zhuangDiscriminationawareChannelPruning2018} & 93.80 & 93.49 & -0.31 & 125.75 & 63.19 & 49.75 & 0.86 & 0.44 & 49.24 \\
2.7.1 & 2022 & RRCP~\cite{liRevisitingRandomChannel2022} & - & 93.48 & - & 125.75 & 64.17 & 48.97 & 0.86 & 0.47 & 44.92 \\
2.2.1 & 2022 & GCNP~\cite{jiangChannelPruningUsing2022} & 93.72 & 93.85 & 0.13 & 125.75 & 65.00 & 48.31 & 0.86 & 0.56 & 35.01 \\
2.5.1 & 2021 & SEP~\cite{dingWherePruneUsing2021} & 93.04 & 93.85 & 0.81 & 125.75 & 65.99 & 47.52 & 0.86 & 0.62 & 27.91 \\
2.2.1 & 2021 & CHIP~\cite{suiCHIPCHannelIndependencebased2021} & 93.26 & 94.16 & 0.90 & 125.75 & 66.14 & 47.40 & 0.86 & 0.49 & 42.80 \\
2.6.2 & 2020 & LFPC~\cite{heLearningFilterPruning2020} & 93.59 & 93.72 & 0.13 & 125.75 & 66.52 & 47.10 & 0.86 & - & - \\
\midrule
\multicolumn{12}{l}{Continue on the next page...}\\
\bottomrule
\end{tabularx}

\captionof{table}{ResNet-56 on CIFAR-10. (Part 1)}
\end{strip}

\addtocounter{table}{-1}

==> tables/cifar10/Resnet-18-34.tex <==
\begin{strip}
\centering
\scriptsize
\begin{tabularx}{\textwidth}{@{}>{\hsize=0.067\hsize}X>{\hsize=0.067\hsize}X>{\hsize=0.2\hsize}X>{\hsize=0.067\hsize}X>{\hsize=0.067\hsize}X>{\hsize=0.067\hsize}X>{\hsize=0.067\hsize}X>{\hsize=0.067\hsize}X>{\hsize=0.067\hsize}X>{\hsize=0.067\hsize}X>{\hsize=0.067\hsize}X>{\hsize=0.067\hsize}X>{\hsize=0.067\hsize}X@{}}
\toprule
\tabletitle \\
\midrule
\multicolumn{3}{l}{ResNet-18} \\
\midrule
2.3.3 & 2019 & OICSR~\cite{liOICSROutInChannelSparsity2019} & 94.46 & 92.44 & -2.02 & 557.21 & 30.65 & 94.50 & 11.17 & - & - \\
2.4.3 & 2022 & StructADMM~\cite{zhangStructADMMAchievingUltrahigh2022} & - & 93.80 & - & 557.21 & 45.67 & 91.80 & 11.17 & - & - \\
2.6.1 & 2020 & AutoCompress~\cite{liuAutoCompressAutomaticDNN2020} & 93.90 & 93.81 & -0.09 & 557.21 & 45.67 & 91.80 & 11.17 & - & - \\
2.3.3 & 2019 & OICSR~\cite{liOICSROutInChannelSparsity2019} & 94.46 & 94.27 & -0.19 & 557.21 & 75.22 & 86.50 & 11.17 & - & - \\
2.6.2 & 2022 & DNCP~\cite{zhengModelCompressionBased2022} & 95.35 & 94.97 & -0.38 & 557.21 & 140.56 & 74.77 & 11.17 & - & - \\
2.5.2 & 2022 & CDG~\cite{mengContrastiveDualGating2022} & 91.26 & 90.37 & -0.89 & 557.21 & 257.97 & 53.70 & 11.17 & - & - \\
2.6.2 & 2022 & DNCP~\cite{zhengModelCompressionBased2022} & 95.35 & 95.31 & -0.04 & 557.21 & 314.25 & 43.60 & 11.17 & - & - \\
2.3.3 & 2019 & OICSR~\cite{liOICSROutInChannelSparsity2019} & 94.46 & 95.10 & 0.64 & 557.21 & 338.78 & 39.20 & 11.17 & - & - \\
2.6.3 & 2022 & EDropout~\cite{salehinejadEDropoutEnergyBasedDropout2022} & 92.81 & 90.96 & -1.85 & 557.21 & - & - & 11.17 & 5.49 & 50.89 \\
2.7.1 & 2022 & EarlyCroP~\cite{rachwanWinningLotteryAhead2022} & 91.50 & 91.00 & -0.50 & 557.21 & - & - & 11.17 & 0.55 & 95.10 \\
2.7.3 & 2022 & DPP~\cite{gonzalez-carabarinDynamicProbabilisticPruning2022} & 93.60 & 93.14 & -0.46 & 557.21 & - & - & 11.17 & 4.13 & 63.06 \\
\midrule
\multicolumn{3}{l}{ResNet-34} \\
\midrule
2.6.3 & 2022 & EDropout~\cite{salehinejadEDropoutEnergyBasedDropout2022} & 92.80 & 88.21 & -4.59 & 1160 & - & - & 21.60 & 8.42 & 61.03 \\
\midrule
\multicolumn{3}{l}{ResNet-50} \\
\midrule
2.3.3 & 2021 & OTO~\cite{chenOnlyTrainOnce2021} & 93.50 & 94.40 & 0.90 & 1307 & 167.30 & 87.20 & 23.52 & 2.07 & 91.20 \\
2.6.3 & 2022 & EDropout~\cite{salehinejadEDropoutEnergyBasedDropout2022} & 92.21 & 85.30 & -6.91 & 1307 & - & - & 23.52 & 10.91 & 53.62 \\
\midrule
\multicolumn{3}{l}{ResNet-101} \\
\midrule
2.7.1 & 2020 & EB~\cite{youDrawingEarlyBirdTickets2020} & - & 92.49 & - & 7595.00 & 3452.27 & 54.55 & 44.54 & 13.36 & 70.00 \\
2.7.1 & 2020 & EB~\cite{youDrawingEarlyBirdTickets2020} & - & 93.90 & - & 7595.00 & 5425.00 & 28.57 & 44.54 & 22.27 & 50.00 \\
2.7.1 & 2020 & EB~\cite{youDrawingEarlyBirdTickets2020} & - & 93.91 & - & 7595.00 & 6904.55 & 9.09 & 44.54 & 31.18 & 30.00 \\
2.6.3 & 2022 & EDropout~\cite{salehinejadEDropoutEnergyBasedDropout2022} & 92.66 & 86.57 & -6.09 & 2520.00 & - & - & 42.51 & 19.20 & 54.82 \\
\bottomrule
\end{tabularx}

\captionof{table}{ResNet-18/34/50/101 on CIFAR-10.}
\end{strip}

==> tables/cifar10/VGG-16.tex <==
% \begin{strip}
% \centering
% \scriptsize
% \begin{tabular}{@{}lllcccccccccc@{}}
% \toprule
% \tabletitle
% \\ \midrule
% VGG-16
% \\ \midrule
% 2.6.1 & 2020 & AutoCompress~\cite{liuAutoCompressAutomaticDNN2020} & 93.70 & 93.21 & -0.49 & 314.59 & 35.75 & 88.64 & 14.73 & - & - \\
% 2.6.1 & 2022 & DECORE~\cite{alwaniDECOREDeepCompression2022} & 93.96 & 91.68 & -2.28 & 314.59 & 36.95 & 88.25 & 14.73 & 0.26 & 98.26 \\
% 2.4.3 & 2022 & StructADMM~\cite{zhangStructADMMAchievingUltrahigh2022} & - & 93.10 & - & 314.59 & 37.90 & 87.95 & 14.73 & - & - \\
% 2.2.3 & 2020 & PFP~\cite{liebenweinProvableFilterPruning2020} & 92.89 & 92.39 & -0.50 & 314.59 & 47.09 & 85.03 & 14.73 & 0.84 & 94.32 \\
% 2.3.3 & 2021 & OTO~\cite{chenOnlyTrainOnce2021} & 91.60 & 91.00 & -0.60 & 314.59 & 51.28 & 83.70 & 14.73 & 0.37 & 97.50 \\
% 2.6.1 & 2022 & DECORE~\cite{alwaniDECOREDeepCompression2022} & 93.96 & 92.44 & -1.52 & 314.59 & 51.34 & 83.68 & 14.73 & 0.50 & 96.60 \\
% 2.3.2 & 2021 & ABP~\cite{tianAddingPruningSparse2021} & 93.96 & 92.65 & -1.31 & 314.59 & 52.81 & 83.21 & 14.73 & 1.50 & 89.79 \\
% 2.7.2 & 2021 & EDP~\cite{ruanEDPEfficientDecomposition2021} & 93.60 & 93.52 & -0.08 & 314.59 & 62.57 & 80.11 & 14.73 & 0.65 & 95.59 \\
% 2.6.1 & 2022 & RL-MCTS~\cite{wangChannelPruningLookahead2022} & 93.51 & 93.72 & 0.21 & 314.59 & 63.23 & 79.90 & 14.73 & - & - \\
% 2.2.1 & 2021 & CHIP~\cite{suiCHIPCHannelIndependencebased2021} & 93.96 & 93.18 & -0.78 & 314.59 & 67.32 & 78.60 & 14.73 & 1.87 & 87.30 \\
% 2.4.2 & 2018 & VIBNet~\cite{dai2018compressing} & - & 91.50 & - & 314.59 & 70.99 & 77.43 & 14.73 & 0.78 & 94.70 \\
% 2.2.3 & 2022 & DLRFC~\cite{heFilterPruningFeature2022} & 93.25 & 93.64 & -0.39 & 314.59 & 72.51 & 76.95 & 14.73 & 0.83 & 94.38 \\
% 2.2.1 & 2020 & HRank~\cite{linHRankFilterPruning2020} & 93.96 & 91.23 & -2.73 & 314.59 & 73.90 & 76.51 & 14.73 & 1.75 & 88.12 \\
% 2.3.2 & 2022 & WhiteBox~\cite{zhangCarryingOutCNN2022} & 93.02 & 93.47 & 0.45 & 314.59 & 74.24 & 76.40 & 14.73 & - & - \\
% 2.1.2 & 2022 & EPruner~\cite{linNetworkPruningUsing2022} & 93.02 & 93.08 & 0.06 & 314.59 & 74.42 & 76.34 & 14.73 & 1.65 & 88.80 \\
% 2.2.2 & 2019 & AOFP~\cite{dingApproximatedOracleFilter2019} & 93.38 & 93.28 & -0.10 & 314.59 & 77.39 & 75.40 & 14.73 & - & - \\
% 2.1.2 & 2022 & CLR-RNF~\cite{linPruningNetworksCrossLayer2022} & 93.02 & 93.32 & 0.30 & 314.59 & 81.48 & 74.10 & 14.73 & 0.74 & 95.00 \\
% 2.6.3 & 2020 & ABCPruner~\cite{linChannelPruningAutomatic2020} & 93.02 & 93.08 & 0.06 & 314.59 & 82.81 & 73.68 & 14.73 & 1.67 & 88.66 \\
% 2.1.2 & 2019 & COP~\cite{wangCOPCustomizedDeep2019} & 93.56 & 93.31 & -0.25 & 314.59 & 83.37 & 73.50 & 14.73 & 1.06 & 92.80 \\
% 2.3.3 & 2021 & OTO~\cite{chenOnlyTrainOnce2021} & 93.20 & 93.30 & 0.10 & 314.59 & 84.31 & 73.20 & 14.73 & 0.81 & 94.50 \\
% 2.2.1 & 2022 & GCNP~\cite{jiangChannelPruningUsing2022} & 93.10 & 93.08 & -0.02 & 314.59 & 84.72 & 73.07 & 14.73 & 1.02 & 93.06 \\
% 2.5.2 & 2022 & FTWT~\cite{elkerdawyFireTogetherWire2022} & 93.82 & 93.19 & -0.63 & 314.59 & 84.94 & 73.00 & 14.73 & - & - \\
% 2.4.2 & 2018 & VIBNet~\cite{dai2018compressing} & - & 93.90 & - & 314.59 & 87.26 & 72.26 & 14.73 & 0.80 & 94.55 \\
% 2.7.3 & 2022 & SOKS~\cite{liuSOKSAutomaticSearching2022} & 93.53 & 94.01 & 0.48 & 314.59 & 87.46 & 72.20 & 14.73 & 3.19 & 78.33 \\
% 2.4.2 & 2019 & RBP~\cite{zhouAccelerateCNNRecursive2019} & - & 91.00 & - & 314.59 & 89.88 & 71.43 & 14.73 & - & - \\
% 2.7.3 & 2020 & SWP~\cite{mengPruningFilterFilter2020} & 93.25 & 93.65 & 0.40 & 314.59 & 90.73 & 71.16 & 14.73 & 1.08 & 92.66 \\
% 2.3.2 & 2021 & GDP-Guo~\cite{guoGDPStabilizedNeural2021} & 93.89 & 93.99 & 0.10 & 314.59 & 96.11 & 69.45 & 14.73 & - & - \\
% 2.2.1 & 2021 & CHIP~\cite{suiCHIPCHannelIndependencebased2021} & 93.96 & 93.72 & -0.24 & 314.59 & 105.07 & 66.60 & 14.73 & 2.46 & 83.30 \\
% 2.3.1 & 2020 & SCP~\cite{kangOperationAwareSoftChannel2020} & 93.85 & 93.79 & 0.06 & 314.59 & 106.24 & 66.23 & 14.73 & 1.02 & 93.05 \\
% 2.3.2 & 2021 & ABP~\cite{tianAddingPruningSparse2021} & 93.96 & 93.50 & -0.46 & 314.59 & 106.59 & 66.12 & 14.73 & 2.66 & 81.96 \\
% 2.2.2 & 2019 & AOFP~\cite{dingApproximatedOracleFilter2019} & 93.38 & 93.47 & 0.09 & 314.59 & 108.55 & 65.50 & 14.73 & - & - \\
% 2.2.1 & 2020 & HRank~\cite{linHRankFilterPruning2020} & 93.96 & 92.34 & -1.62 & 314.59 & 108.91 & 65.38 & 14.73 & 2.60 & 82.38 \\
% 2.5.2 & 2022 & FTWT~\cite{elkerdawyFireTogetherWire2022} & 93.82 & 93.55 & -0.27 & 314.59 & 110.11 & 65.00 & 14.73 & - & - \\
% 2.6.1 & 2022 & DECORE~\cite{alwaniDECOREDeepCompression2022} & 93.96 & 93.56 & -0.40 & 314.59 & 110.81 & 64.78 & 14.73 & 1.63 & 88.92 \\
% 2.6.3 & 2022 & CCEP~\cite{shangNeuralNetworkPruning2022} & 93.71 & 93.52 & -0.19 & 314.59 & 115.77 & 63.20 & 14.73 & - & - \\
% 2.4.2 & 2018 & VIBNet~\cite{dai2018compressing} & - & 94.20 & - & 314.59 & 116.59 & 62.94 & 14.73 & 0.85 & 94.21 \\
% 2.2.3 & 2022 & DLRFC~\cite{heFilterPruningFeature2022} & 93.25 & 93.93 & -0.68 & 314.59 & 121.97 & 61.23 & 14.73 & 1.05 & 92.86 \\
% 2.7.2 & 2021 & CC~\cite{liCompactCNNsCollaborative2021} & 93.70 & 94.09 & 0.39 & 314.59 & 123.62 & 60.70 & 14.73 & 4.02 & 72.69 \\
% 2.7.3 & 2022 & SOKS~\cite{liuSOKSAutomaticSearching2022} & 93.53 & 94.11 & 0.58 & 314.59 & 124.23 & 60.51 & 14.73 & 4.50 & 69.47 \\
% 2.2.2 & 2019 & AOFP~\cite{dingApproximatedOracleFilter2019} & 93.38 & 93.84 & 0.46 & 314.59 & 124.63 & 60.38 & 14.73 & - & - \\
% 2.2.1 & 2021 & CHIP~\cite{suiCHIPCHannelIndependencebased2021} & 93.96 & 93.86 & -0.10 & 314.59 & 131.81 & 58.10 & 14.73 & 2.71 & 81.60 \\
% 2.2.1 & 2022 & GCNP~\cite{jiangChannelPruningUsing2022} & 93.10 & 93.27 & 0.17 & 314.59 & 134.36 & 57.29 & 14.73 & 2.14 & 85.50 \\
% 2.6.2 & 2021 & EE~\cite{zhangExplorationEstimationModel2021} & 93.36 & 93.63 & 0.27 & 314.59 & 136.53 & 56.60 & 14.73 & - & - \\
% 2.5.2 & 2022 & FTWT~\cite{elkerdawyFireTogetherWire2022} & 93.82 & 93.73 & -0.09 & 314.59 & 138.42 & 56.00 & 14.73 & - & - \\
% 2.3.1 & 2020 & PR~\cite{zhuangNeuronlevelStructuredPruning2020} & 93.88 & 93.92 & -0.04 & 314.59 & 144.71 & 54.00 & 14.73 & - & - \\
% 2.2.1 & 2020 & HRank~\cite{linHRankFilterPruning2020} & 93.96 & 93.43 & -0.53 & 314.59 & 146.01 & 53.59 & 14.73 & 2.47 & 83.24 \\
% 2.3.2 & 2021 & ABP~\cite{tianAddingPruningSparse2021} & 93.96 & 93.75 & -0.21 & 314.59 & 146.19 & 53.53 & 14.73 & 2.44 & 83.46 \\
% 2.7.2 & 2021 & CC~\cite{liCompactCNNsCollaborative2021} & 93.70 & 94.15 & 0.45 & 314.59 & 154.78 & 50.80 & 14.73 & 5.02 & 65.90 \\
% 2.6.1 & 2022 & RL-MCTS~\cite{wangChannelPruningLookahead2022} & 93.51 & 93.90 & 0.39 & 314.59 & 171.45 & 45.50 & 14.73 & - & - \\
% 2.3.2 & 2019 & GAL~\cite{linOptimalStructuredCNN2019} & 93.96 & 90.78 & -3.18 & 314.59 & 172.36 & 45.21 & 14.73 & 2.63 & 82.18 \\
% 2.3.2 & 2019 & GAL~\cite{linOptimalStructuredCNN2019} & 93.96 & 93.42 & -0.54 & 314.59 & 172.36 & 45.21 & 14.73 & 2.63 & 82.18 \\
% 2.7.1 & 2020 & EB~\cite{youDrawingEarlyBirdTickets2020} & - & 92.49 & - & 314.59 & 174.77 & 44.44 & 14.73 & 4.42 & 70.00 \\
% 2.2.2 & 2019 & AOFP~\cite{dingApproximatedOracleFilter2019} & 93.38 & 94.03 & 0.65 & 314.59 & 186.94 & 40.58 & 14.73 & - & - \\
% 2.3.2 & 2019 & GAL~\cite{linOptimalStructuredCNN2019} & 93.96 & 93.77 & -0.19 & 314.59 & 190.01 & 39.60 & 14.73 & 3.30 & 77.57 \\
% 2.3.2 & 2019 & GAL~\cite{linOptimalStructuredCNN2019} & 93.96 & 92.03 & -1.93 & 314.59 & 190.01 & 39.60 & 14.73 & 3.30 & 77.57 \\
% 2.4.2 & 2019 & VP~\cite{zhaoVariationalConvolutionalNeural2019} & 93.25 & 93.18 & -0.07 & 314.59 & 190.97 & 39.30 & 14.73 & 3.93 & 73.35 \\
% 2.7.2 & 2020 & Hinge~\cite{liGroupSparsityHinge2020} & 94.02 & 93.59 & -0.43 & 314.59 & 191.68 & 39.07 & 14.73 & 2.94 & 80.05 \\
% 2.7.3 & 2019 & SDN~\cite{chenShallowingDeepNetworks2019} & 93.50 & 93.47 & -0.03 & 314.59 & 192.21 & 38.90 & 14.73 & 1.78 & 87.90 \\
% 2.2.1 & 2021 & LRMF~\cite{zhangFilterPruningLearned2021} & 93.58 & 93.70 & 0.12 & 314.59 & 201.65 & 35.90 & 14.73 & - & - \\
% 2.2.1 & 2021 & LRMF~\cite{zhangFilterPruningLearned2021} & 93.58 & 93.20 & -0.38 & 314.59 & 201.65 & 35.90 & 14.73 & - & - \\
% 2.6.1 & 2022 & DECORE~\cite{alwaniDECOREDeepCompression2022} & 93.96 & 94.02 & 0.06 & 314.59 & 203.64 & 35.27 & 14.73 & 5.45 & 63.02 \\
% 2.1.1 & 2017 & PFEC~\cite{liPruningFiltersEfficient2017} & 93.25 & 93.40 & 0.15 & 314.59 & 207.05 & 34.19 & 14.73 & 5.30 & 64.00 \\
% 2.2.2 & 2019 & AOFP~\cite{dingApproximatedOracleFilter2019} & 93.38 & 93.81 & 0.43 & 314.59 & 216.09 & 31.31 & 14.73 & - & - \\
% 2.7.1 & 2020 & EB~\cite{youDrawingEarlyBirdTickets2020} & - & 93.90 & - & 314.59 & 224.71 & 28.57 & 14.73 & 7.37 & 50.00 \\
% 2.7.1 & 2020 & EB~\cite{youDrawingEarlyBirdTickets2020} & - & 93.91 & - & 314.59 & 262.16 & 16.67 & 14.73 & 10.31 & 30.00 \\
% 2.7.1 & 2022 & EarlyCroP~\cite{rachwanWinningLotteryAhead2022} & 90.20 & 93.00 & 2.80 & 314.59 & - & - & 14.73 & 0.29 & 98.00 \\
% 2.7.3 & 2022 & DPP~\cite{gonzalez-carabarinDynamicProbabilisticPruning2022} & 93.50 & 93.60 & 0.10 & 314.59 & - & - & 14.73 & 1.58 & 89.27 \\
% \bottomrule
% \end{tabular}

% \captionof{table}{VGG-16 on CIFAR-10.}
% \end{strip}

\begin{strip}
\centering
\scriptsize
\begin{tabularx}{\textwidth}{@{}>{\hsize=0.067\hsize}X>{\hsize=0.067\hsize}X>{\hsize=0.2\hsize}X>{\hsize=0.067\hsize}X>{\hsize=0.067\hsize}X>{\hsize=0.067\hsize}X>{\hsize=0.067\hsize}X>{\hsize=0.067\hsize}X>{\hsize=0.067\hsize}X>{\hsize=0.067\hsize}X>{\hsize=0.067\hsize}X>{\hsize=0.067\hsize}X>{\hsize=0.067\hsize}X@{}}
\toprule
\tabletitle
\\ \midrule
\multicolumn{3}{l}{VGG-16}
\\ \midrule
2.6.1 & 2020 & AutoCompress~\cite{liuAutoCompressAutomaticDNN2020} & 93.70 & 93.21 & -0.49 & 314.59 & 35.75 & 88.64 & 14.73 & - & - \\
2.6.1 & 2022 & DECORE~\cite{alwaniDECOREDeepCompression2022} & 93.96 & 91.68 & -2.28 & 314.59 & 36.95 & 88.25 & 14.73 & 0.26 & 98.26 \\
2.4.3 & 2022 & StructADMM~\cite{zhangStructADMMAchievingUltrahigh2022} & - & 93.10 & - & 314.59 & 37.90 & 87.95 & 14.73 & - & - \\
2.2.3 & 2020 & PFP~\cite{liebenweinProvableFilterPruning2020} & 92.89 & 92.39 & -0.50 & 314.59 & 47.09 & 85.03 & 14.73 & 0.84 & 94.32 \\
2.3.3 & 2021 & OTO~\cite{chenOnlyTrainOnce2021} & 91.60 & 91.00 & -0.60 & 314.59 & 51.28 & 83.70 & 14.73 & 0.37 & 97.50 \\
2.6.1 & 2022 & DECORE~\cite{alwaniDECOREDeepCompression2022} & 93.96 & 92.44 & -1.52 & 314.59 & 51.34 & 83.68 & 14.73 & 0.50 & 96.60 \\
2.3.2 & 2021 & ABP~\cite{tianAddingPruningSparse2021} & 93.96 & 92.65 & -1.31 & 314.59 & 52.81 & 83.21 & 14.73 & 1.50 & 89.79 \\
2.7.2 & 2021 & EDP~\cite{ruanEDPEfficientDecomposition2021} & 93.60 & 93.52 & -0.08 & 314.59 & 62.57 & 80.11 & 14.73 & 0.65 & 95.59 \\
2.6.1 & 2022 & RL-MCTS~\cite{wangChannelPruningLookahead2022} & 93.51 & 93.72 & 0.21 & 314.59 & 63.23 & 79.90 & 14.73 & - & - \\
2.2.1 & 2021 & CHIP~\cite{suiCHIPCHannelIndependencebased2021} & 93.96 & 93.18 & -0.78 & 314.59 & 67.32 & 78.60 & 14.73 & 1.87 & 87.30 \\
2.4.2 & 2018 & VIBNet~\cite{dai2018compressing} & - & 91.50 & - & 314.59 & 70.99 & 77.43 & 14.73 & 0.78 & 94.70 \\
2.2.3 & 2022 & DLRFC~\cite{heFilterPruningFeature2022} & 93.25 & 93.64 & -0.39 & 314.59 & 72.51 & 76.95 & 14.73 & 0.83 & 94.38 \\
2.2.1 & 2020 & HRank~\cite{linHRankFilterPruning2020} & 93.96 & 91.23 & -2.73 & 314.59 & 73.90 & 76.51 & 14.73 & 1.75 & 88.12 \\
2.3.2 & 2022 & WhiteBox~\cite{zhangCarryingOutCNN2022} & 93.02 & 93.47 & 0.45 & 314.59 & 74.24 & 76.40 & 14.73 & - & - \\
2.1.2 & 2022 & EPruner~\cite{linNetworkPruningUsing2022} & 93.02 & 93.08 & 0.06 & 314.59 & 74.42 & 76.34 & 14.73 & 1.65 & 88.80 \\
2.2.2 & 2019 & AOFP~\cite{dingApproximatedOracleFilter2019} & 93.38 & 93.28 & -0.10 & 314.59 & 77.39 & 75.40 & 14.73 & - & - \\
2.1.2 & 2022 & CLR-RNF~\cite{linPruningNetworksCrossLayer2022} & 93.02 & 93.32 & 0.30 & 314.59 & 81.48 & 74.10 & 14.73 & 0.74 & 95.00 \\
2.6.3 & 2020 & ABCPruner~\cite{linChannelPruningAutomatic2020} & 93.02 & 93.08 & 0.06 & 314.59 & 82.81 & 73.68 & 14.73 & 1.67 & 88.66 \\
2.1.2 & 2019 & COP~\cite{wangCOPCustomizedDeep2019} & 93.56 & 93.31 & -0.25 & 314.59 & 83.37 & 73.50 & 14.73 & 1.06 & 92.80 \\
2.3.3 & 2021 & OTO~\cite{chenOnlyTrainOnce2021} & 93.20 & 93.30 & 0.10 & 314.59 & 84.31 & 73.20 & 14.73 & 0.81 & 94.50 \\
2.2.1 & 2022 & GCNP~\cite{jiangChannelPruningUsing2022} & 93.10 & 93.08 & -0.02 & 314.59 & 84.72 & 73.07 & 14.73 & 1.02 & 93.06 \\
2.5.2 & 2022 & FTWT~\cite{elkerdawyFireTogetherWire2022} & 93.82 & 93.19 & -0.63 & 314.59 & 84.94 & 73.00 & 14.73 & - & - \\
2.4.2 & 2018 & VIBNet~\cite{dai2018compressing} & - & 93.90 & - & 314.59 & 87.26 & 72.26 & 14.73 & 0.80 & 94.55 \\
2.7.3 & 2022 & SOKS~\cite{liuSOKSAutomaticSearching2022} & 93.53 & 94.01 & 0.48 & 314.59 & 87.46 & 72.20 & 14.73 & 3.19 & 78.33 \\
2.4.2 & 2019 & RBP~\cite{zhouAccelerateCNNRecursive2019} & - & 91.00 & - & 314.59 & 89.88 & 71.43 & 14.73 & - & - \\
2.7.3 & 2020 & SWP~\cite{mengPruningFilterFilter2020} & 93.25 & 93.65 & 0.40 & 314.59 & 90.73 & 71.16 & 14.73 & 1.08 & 92.66 \\
2.3.2 & 2021 & GDP-Guo~\cite{guoGDPStabilizedNeural2021} & 93.89 & 93.99 & 0.10 & 314.59 & 96.11 & 69.45 & 14.73 & - & - \\
2.2.1 & 2021 & CHIP~\cite{suiCHIPCHannelIndependencebased2021} & 93.96 & 93.72 & -0.24 & 314.59 & 105.07 & 66.60 & 14.73 & 2.46 & 83.30 \\
2.3.1 & 2020 & SCP~\cite{kangOperationAwareSoftChannel2020} & 93.85 & 93.79 & 0.06 & 314.59 & 106.24 & 66.23 & 14.73 & 1.02 & 93.05 \\
2.3.2 & 2021 & ABP~\cite{tianAddingPruningSparse2021} & 93.96 & 93.50 & -0.46 & 314.59 & 106.59 & 66.12 & 14.73 & 2.66 & 81.96 \\
2.2.2 & 2019 & AOFP~\cite{dingApproximatedOracleFilter2019} & 93.38 & 93.47 & 0.09 & 314.59 & 108.55 & 65.50 & 14.73 & - & - \\
2.2.1 & 2020 & HRank~\cite{linHRankFilterPruning2020} & 93.96 & 92.34 & -1.62 & 314.59 & 108.91 & 65.38 & 14.73 & 2.60 & 82.38 \\
2.5.2 & 2022 & FTWT~\cite{elkerdawyFireTogetherWire2022} & 93.82 & 93.55 & -0.27 & 314.59 & 110.11 & 65.00 & 14.73 & - & - \\
2.6.1 & 2022 & DECORE~\cite{alwaniDECOREDeepCompression2022} & 93.96 & 93.56 & -0.40 & 314.59 & 110.81 & 64.78 & 14.73 & 1.63 & 88.92 \\
2.6.3 & 2022 & CCEP~\cite{shangNeuralNetworkPruning2022} & 93.71 & 93.52 & -0.19 & 314.59 & 115.77 & 63.20 & 14.73 & - & - \\
2.4.2 & 2018 & VIBNet~\cite{dai2018compressing} & - & 94.20 & - & 314.59 & 116.59 & 62.94 & 14.73 & 0.85 & 94.21 \\
2.2.3 & 2022 & DLRFC~\cite{heFilterPruningFeature2022} & 93.25 & 93.93 & -0.68 & 314.59 & 121.97 & 61.23 & 14.73 & 1.05 & 92.86 \\
2.7.2 & 2021 & CC~\cite{liCompactCNNsCollaborative2021} & 93.70 & 94.09 & 0.39 & 314.59 & 123.62 & 60.70 & 14.73 & 4.02 & 72.69 \\
2.7.3 & 2022 & SOKS~\cite{liuSOKSAutomaticSearching2022} & 93.53 & 94.11 & 0.58 & 314.59 & 124.23 & 60.51 & 14.73 & 4.50 & 69.47 \\
2.2.2 & 2019 & AOFP~\cite{dingApproximatedOracleFilter2019} & 93.38 & 93.84 & 0.46 & 314.59 & 124.63 & 60.38 & 14.73 & - & - \\
2.2.1 & 2021 & CHIP~\cite{suiCHIPCHannelIndependencebased2021} & 93.96 & 93.86 & -0.10 & 314.59 & 131.81 & 58.10 & 14.73 & 2.71 & 81.60 \\
2.2.1 & 2022 & GCNP~\cite{jiangChannelPruningUsing2022} & 93.10 & 93.27 & 0.17 & 314.59 & 134.36 & 57.29 & 14.73 & 2.14 & 85.50 \\
2.6.2 & 2021 & EE~\cite{zhangExplorationEstimationModel2021} & 93.36 & 93.63 & 0.27 & 314.59 & 136.53 & 56.60 & 14.73 & - & - \\
2.5.2 & 2022 & FTWT~\cite{elkerdawyFireTogetherWire2022} & 93.82 & 93.73 & -0.09 & 314.59 & 138.42 & 56.00 & 14.73 & - & - \\
2.3.1 & 2020 & PR~\cite{zhuangNeuronlevelStructuredPruning2020} & 93.88 & 93.92 & -0.04 & 314.59 & 144.71 & 54.00 & 14.73 & - & - \\
2.2.1 & 2020 & HRank~\cite{linHRankFilterPruning2020} & 93.96 & 93.43 & -0.53 & 314.59 & 146.01 & 53.59 & 14.73 & 2.47 & 83.24 \\
2.3.2 & 2021 & ABP~\cite{tianAddingPruningSparse2021} & 93.96 & 93.75 & -0.21 & 314.59 & 146.19 & 53.53 & 14.73 & 2.44 & 83.46 \\
2.7.2 & 2021 & CC~\cite{liCompactCNNsCollaborative2021} & 93.70 & 94.15 & 0.45 & 314.59 & 154.78 & 50.80 & 14.73 & 5.02 & 65.90 \\
2.6.1 & 2022 & RL-MCTS~\cite{wangChannelPruningLookahead2022} & 93.51 & 93.90 & 0.39 & 314.59 & 171.45 & 45.50 & 14.73 & - & - \\
2.3.2 & 2019 & GAL~\cite{linOptimalStructuredCNN2019} & 93.96 & 90.78 & -3.18 & 314.59 & 172.36 & 45.21 & 14.73 & 2.63 & 82.18 \\
2.3.2 & 2019 & GAL~\cite{linOptimalStructuredCNN2019} & 93.96 & 93.42 & -0.54 & 314.59 & 172.36 & 45.21 & 14.73 & 2.63 & 82.18 \\
2.7.1 & 2020 & EB~\cite{youDrawingEarlyBirdTickets2020} & - & 92.49 & - & 314.59 & 174.77 & 44.44 & 14.73 & 4.42 & 70.00 \\
2.2.2 & 2019 & AOFP~\cite{dingApproximatedOracleFilter2019} & 93.38 & 94.03 & 0.65 & 314.59 & 186.94 & 40.58 & 14.73 & - & - \\
2.3.2 & 2019 & GAL~\cite{linOptimalStructuredCNN2019} & 93.96 & 93.77 & -0.19 & 314.59 & 190.01 & 39.60 & 14.73 & 3.30 & 77.57 \\
2.3.2 & 2019 & GAL~\cite{linOptimalStructuredCNN2019} & 93.96 & 92.03 & -1.93 & 314.59 & 190.01 & 39.60 & 14.73 & 3.30 & 77.57 \\
2.4.2 & 2019 & VP~\cite{zhaoVariationalConvolutionalNeural2019} & 93.25 & 93.18 & -0.07 & 314.59 & 190.97 & 39.30 & 14.73 & 3.93 & 73.35 \\
2.7.2 & 2020 & Hinge~\cite{liGroupSparsityHinge2020} & 94.02 & 93.59 & -0.43 & 314.59 & 191.68 & 39.07 & 14.73 & 2.94 & 80.05 \\
2.7.3 & 2019 & SDN~\cite{chenShallowingDeepNetworks2019} & 93.50 & 93.47 & -0.03 & 314.59 & 192.21 & 38.90 & 14.73 & 1.78 & 87.90 \\
2.2.1 & 2021 & LRMF~\cite{zhangFilterPruningLearned2021} & 93.58 & 93.70 & 0.12 & 314.59 & 201.65 & 35.90 & 14.73 & - & - \\
2.2.1 & 2021 & LRMF~\cite{zhangFilterPruningLearned2021} & 93.58 & 93.20 & -0.38 & 314.59 & 201.65 & 35.90 & 14.73 & - & - \\
2.6.1 & 2022 & DECORE~\cite{alwaniDECOREDeepCompression2022} & 93.96 & 94.02 & 0.06 & 314.59 & 203.64 & 35.27 & 14.73 & 5.45 & 63.02 \\
2.1.1 & 2017 & PFEC~\cite{liPruningFiltersEfficient2017} & 93.25 & 93.40 & 0.15 & 314.59 & 207.05 & 34.19 & 14.73 & 5.30 & 64.00 \\
2.2.2 & 2019 & AOFP~\cite{dingApproximatedOracleFilter2019} & 93.38 & 93.81 & 0.43 & 314.59 & 216.09 & 31.31 & 14.73 & - & - \\
2.7.1 & 2020 & EB~\cite{youDrawingEarlyBirdTickets2020} & - & 93.90 & - & 314.59 & 224.71 & 28.57 & 14.73 & 7.37 & 50.00 \\
2.7.1 & 2020 & EB~\cite{youDrawingEarlyBirdTickets2020} & - & 93.91 & - & 314.59 & 262.16 & 16.67 & 14.73 & 10.31 & 30.00 \\
2.7.1 & 2022 & EarlyCroP~\cite{rachwanWinningLotteryAhead2022} & 90.20 & 93.00 & 2.80 & 314.59 & - & - & 14.73 & 0.29 & 98.00 \\
2.7.3 & 2022 & DPP~\cite{gonzalez-carabarinDynamicProbabilisticPruning2022} & 93.50 & 93.60 & 0.10 & 314.59 & - & - & 14.73 & 1.58 & 89.27 \\
\bottomrule
\end{tabularx}

\captionof{table}{VGG-16 on CIFAR-10.}
\end{strip}

==> tables/cifar10/VGG-19.tex <==
\begin{strip}
\centering
\scriptsize
\begin{tabularx}{\textwidth}{@{}>{\hsize=0.067\hsize}X>{\hsize=0.067\hsize}X>{\hsize=0.2\hsize}X>{\hsize=0.067\hsize}X>{\hsize=0.067\hsize}X>{\hsize=0.067\hsize}X>{\hsize=0.067\hsize}X>{\hsize=0.067\hsize}X>{\hsize=0.067\hsize}X>{\hsize=0.067\hsize}X>{\hsize=0.067\hsize}X>{\hsize=0.067\hsize}X>{\hsize=0.067\hsize}X@{}}
\toprule
\tabletitle
\\ \midrule
\multicolumn{3}{l}{VGG-19}
\\ \midrule
2.6.1 & 2022 & DECORE~\cite{alwaniDECOREDeepCompression2022} & 93.76 & 91.65 & -2.11 & 398.00& 43.85 & 88.98 & 20.04 & 0.30 & 98.50 \\
2.4.1 & 2019 & ED~\cite{wangEigenDamageStructuredPruning2019} & 94.17 & 92.29 & -1.88 & 398.00& 53.69 & 86.51 & 20.04 & 0.57 & 97.15 \\
2.5.1 & 2021 & SEP~\cite{dingWherePruneUsing2021} & 93.66 & 93.40 & -0.26 & 398.00& 59.80 & 84.97 & 20.04 & 4.01 & 79.99 \\
2.4.1 & 2019 & ED~\cite{wangEigenDamageStructuredPruning2019} & 93.71 & 91.79 & -1.92 & 398.00& 60.42 & 84.82 & 20.04 & 0.63 & 96.84 \\
2.3.1 & 2020 & SCP~\cite{kangOperationAwareSoftChannel2020} & 93.84 & 93.82 & 0.02 & 398.00& 103.24 & 74.06 & 20.04 & 0.96 & 95.21 \\
2.2.3 & 2018 & DCP~\cite{zhuangDiscriminationawareChannelPruning2018} & 93.99 & 94.57 & 0.58 & 398.00& 139.16 & 65.03 & 20.04 & 1.29 & 93.58 \\
2.4.1 & 2022 & SOSP~\cite{nonnenmacherSOSPEfficientlyCapturing2022} & 94.18 & 93.73 & -0.45 & 398.00& 168.19 & 57.74 & 20.04 & 2.55 & 87.29 \\
2.5.1 & 2021 & DCP-CAC~\cite{chenDynamicalChannelPruning2021} & 92.47 & 93.19 & 0.72 & 398.00& 195.00 & 51.01 & 20.04 & 5.51 & 72.53 \\
2.3.1 & 2017 & NS~\cite{liuLearningEfficientConvolutional2017} & 93.66 & 93.80 & 0.14 & 398.00& 196.98 & 50.51 & 20.04 & 2.30 & 88.52 \\
2.2.3 & 2018 & DCP~\cite{zhuangDiscriminationawareChannelPruning2018} & 93.99 & 94.16 & 0.17 & 398.00& 199.00 & 50.00 & 20.04 & 10.44 & 47.92 \\
2.4.1 & 2022 & SOSP~\cite{nonnenmacherSOSPEfficientlyCapturing2022} & 94.18 & 93.99 & -0.19 & 398.00& 215.08 & 45.96 & 20.04 & 2.86 & 85.75 \\
2.4.1 & 2019 & ED~\cite{wangEigenDamageStructuredPruning2019} & 93.71 & 93.88 & 0.17 & 398.00& 239.44 & 39.84 & 20.04 & 4.11 & 79.50 \\
2.4.1 & 2019 & ED~\cite{wangEigenDamageStructuredPruning2019} & 94.17 & 93.98 & -0.19 & 398.00& 250.22 & 37.13 & 20.04 & 4.37 & 78.18 \\
2.7.1 & 2022 & ProsPr~\cite{alizadehProspectPruningFinding2022} & 93.60 & 93.61 & 0.01 & 398.00& - & - & 20.04 & 4.01 & 80.00 \\
2.7.1 & 2022 & ProsPr~\cite{alizadehProspectPruningFinding2022} & 93.60 & 93.64 & 0.04 & 398.00& - & - & 20.04 & 2.00 & 90.00 \\
2.7.1 & 2022 & ProsPr~\cite{alizadehProspectPruningFinding2022} & 93.60 & 93.32 & -0.28 & 398.00& - & - & 20.04 & 1.00 & 95.00 \\
\bottomrule
\end{tabularx}

\captionof{table}{VGG-19 on CIFAR-10.}
\end{strip}

==> tables/cifar100/MobileNet.tex <==
\begin{strip}
\centering
\scriptsize
\begin{tabularx}{\textwidth}{@{}llllccccccccc@{}}
\toprule
\tabletitle \\
\midrule
\multicolumn{3}{l}{MobileNet-V1} \\
\midrule
2.7.3 & 2022 & DPP~\cite{gonzalez-carabarinDynamicProbabilisticPruning2022} & 72.35 & 72.50 & -0.15 & - & - & - & - & - & 60 \\
\midrule
\multicolumn{3}{l}{MobileNet-V2} \\
\midrule
2.4.2 & 2022 & EKG~\cite{leeEnsembleKnowledgeGuided2022} & 76.07 & 76.29 & 0.22 & 89.00 & 44.50 & 50.00 & 3.50 & - & - \\
2.6.2 & 2022 & DNCP~\cite{zhengModelCompressionBased2022} & 75.91 & 75.69 & -0.22 & 89.00 & 52.00 & 41.57 & 3.50 & - & - \\
\bottomrule
\end{tabularx}

\captionof{table}{MobileNet-V1/V2 on CIFAR-100.}
\end{strip}

==> tables/cifar100/Other.tex <==
\begin{strip}
\centering
\scriptsize
\begin{tabularx}{\textwidth}{@{}>{\hsize=0.067\hsize}X>{\hsize=0.067\hsize}X>{\hsize=0.2\hsize}X>{\hsize=0.067\hsize}X>{\hsize=0.067\hsize}X>{\hsize=0.067\hsize}X>{\hsize=0.067\hsize}X>{\hsize=0.067\hsize}X>{\hsize=0.067\hsize}X>{\hsize=0.067\hsize}X>{\hsize=0.067\hsize}X>{\hsize=0.067\hsize}X>{\hsize=0.067\hsize}X@{}}
\toprule
\tabletitle \\
\midrule
\multicolumn{3}{l}{DenseNet-40} \\
\midrule
2.3.1 & 2020 & SCP~\cite{kangOperationAwareSoftChannel2020} & 74.24 & 73.17 & 1.07 & 283.00 & 91.07 & 67.82 & 1.04 & 0.26 & 74.86 \\
2.3.1 & 2017 & NS~\cite{liuLearningEfficientConvolutional2017} & 74.64 & 74.28 & -0.36 & 283.00 & 149.20 & 47.28 & 1.04 & 0.45 & 56.60 \\
2.3.1 & 2020 & SCP~\cite{kangOperationAwareSoftChannel2020} & 74.24 & 73.84 & 0.40 & 283.00 & 152.11 & 46.25 & 1.04 & 0.47 & 55.22 \\
2.3.1 & 2017 & NS~\cite{liuLearningEfficientConvolutional2017} & 74.64 & 74.72 & 0.08 & 283.00 & 196.98 & 30.39 & 1.04 & 0.65 & 37.74 \\
2.4.1 & 2022 & SOSP~\cite{nonnenmacherSOSPEfficientlyCapturing2022} & 74.11 & 73.46 & -0.65 & 283.00 & 198.16 & 29.98 & 1.04 & - & - \\
2.4.1 & 2022 & SOSP~\cite{nonnenmacherSOSPEfficientlyCapturing2022} & 74.11 & 73.60 & -0.51 & 283.00 & 203.11 & 28.23 & 1.04 & - & - \\
2.4.2 & 2019 & VP~\cite{zhaoVariationalConvolutionalNeural2019} & 74.64 & 72.19 & -2.45 & 283.00 & 218.77 & 22.70 & 1.04 & 0.65 & 37.50 \\
\midrule
\multicolumn{3}{l}{PreResNet-29} \\
\midrule
2.4.1 & 2019 & ED~\cite{wangEigenDamageStructuredPruning2019} & 75.70 & 65.11 & -10.59 & 41.28 & 3.91 & 90.52 & 0.27 & - & - \\
2.4.1 & 2019 & ED~\cite{wangEigenDamageStructuredPruning2019} & 75.70 & 73.62 & -2.08 & 41.28 & 15.33 & 62.86 & 0.27 & - & - \\
\midrule
\multicolumn{3}{l}{PreResNet-101} \\
\midrule
2.7.1 & 2020 & EB~\cite{youDrawingEarlyBirdTickets2020} & - & 72.29 & - & 7595 & 3038.00 & 60.00 & 44.54 & 13.36 & 70 \\
2.7.1 & 2020 & EB~\cite{youDrawingEarlyBirdTickets2020} & - & 73.15 & - & 7595 & 5425.00 & 28.57 & 44.54 & 22.27 & 50 \\
2.7.1 & 2020 & EB~\cite{youDrawingEarlyBirdTickets2020} & - & 73.52 & - & 7595 & 6329.17 & 16.67 & 44.54 & 31.18 & 30 \\
\midrule
\multicolumn{3}{l}{ResNeXt-20} \\
\midrule
2.7.2 & 2020 & Hinge~\cite{liGroupSparsityHinge2020} & 71.95 & 71.26 & -0.69 & 36 & 19.29 & 46.41 & 0.21 & 0.14 & 34.76 \\
\midrule
\multicolumn{3}{l}{ResNeXt-164} \\
\midrule
2.7.2 & 2020 & Hinge~\cite{liGroupSparsityHinge2020} & 76.87 & 77.44 & 0.57 & 210 & 100.28 & 52.25 & 1.70 & 0.99 & 41.51 \\
\bottomrule
\end{tabularx}

\captionof{table}{Other models on CIFAR-100, including DenseNet-40, PreResNet-29/101, and ResNeXt-20/164.}
\end{strip}

==> tables/cifar100/ResNet-18.tex <==
\begin{strip}
\centering
\scriptsize
\begin{tabularx}{\textwidth}{@{}>{\hsize=0.067\hsize}X>{\hsize=0.067\hsize}X>{\hsize=0.2\hsize}X>{\hsize=0.067\hsize}X>{\hsize=0.067\hsize}X>{\hsize=0.067\hsize}X>{\hsize=0.067\hsize}X>{\hsize=0.067\hsize}X>{\hsize=0.067\hsize}X>{\hsize=0.067\hsize}X>{\hsize=0.067\hsize}X>{\hsize=0.067\hsize}X>{\hsize=0.067\hsize}X@{}}
\toprule
\tabletitle \\
\midrule
\multicolumn{3}{l}{ResNet-18} \\
\midrule
2.5.2 & 2022 & CDG~\cite{mengContrastiveDualGating2022} & 67.78 & 65.94 & -1.84 & 557.21 & 293.27 & 47.37 & 11.17 & - & - \\
2.6.3 & 2022 & EDropout~\cite{salehinejadEDropoutEnergyBasedDropout2022} & 69.03 & 67.06 & -1.97 & 557.21 & - & - & 11.17 & 5.39 & 51.79 \\
\midrule
\multicolumn{3}{l}{ResNet-34} \\
\midrule
2.6.3 & 2022 & EDropout~\cite{salehinejadEDropoutEnergyBasedDropout2022} & 69.96 & 64.79 & -5.17 & 1160.00 & - & - & 21.60 & 10.65 & 50.70 \\
\midrule
\multicolumn{3}{l}{ResNet-50} \\
\midrule
2.6.2 & 2022 & DNCP~\cite{zhengModelCompressionBased2022} & 79.01 & 79.22 & 0.21 & 1307.00 & 739.62 & 43.41 & 23.52 & - & - \\
2.6.3 & 2022 & EDropout~\cite{salehinejadEDropoutEnergyBasedDropout2022} & 71.22 & 61.91 & -9.31 & 1307.00 & - & - & 23.52 & 10.82 & 54.01 \\
\midrule
\multicolumn{3}{l}{ResNet-101} \\
\midrule
2.7.1 & 2020 & EB~\cite{youDrawingEarlyBirdTickets2020} & - & 72.29 & - & 7595.00 & 3038.00 & 60.00 & 44.54 & 13.36 & 70.00 \\
2.7.1 & 2020 & EB~\cite{youDrawingEarlyBirdTickets2020} & - & 73.15 & - & 7595.00 & 5425.00 & 28.57 & 44.54 & 22.27 & 50.00 \\
2.7.1 & 2020 & EB~\cite{youDrawingEarlyBirdTickets2020} & - & 73.52 & - & 7595.00 & 6329.17 & 16.67 & 44.54 & 31.18 & 30.00 \\
2.6.3 & 2022 & EDropout~\cite{salehinejadEDropoutEnergyBasedDropout2022} & 71.19 & 61.92 & -9.27 & 2520.00 & - & - & 42.51 & 18.56 & 56.34 \\
\bottomrule
\end{tabularx}

\captionof{table}{ResNet-18/34/50/101 on CIFAR-100.}
\end{strip}

==> tables/cifar100/ResNet-20.tex <==
\begin{strip}
\centering
\scriptsize
\begin{tabularx}{\textwidth}{@{}>{\hsize=0.067\hsize}X>{\hsize=0.067\hsize}X>{\hsize=0.2\hsize}X>{\hsize=0.067\hsize}X>{\hsize=0.067\hsize}X>{\hsize=0.067\hsize}X>{\hsize=0.067\hsize}X>{\hsize=0.067\hsize}X>{\hsize=0.067\hsize}X>{\hsize=0.067\hsize}X>{\hsize=0.067\hsize}X>{\hsize=0.067\hsize}X>{\hsize=0.067\hsize}X@{}}
\toprule
\tabletitle \\
\midrule
\multicolumn{3}{l}{ResNet-20} \\
\midrule
2.7.2 & 2020 & Hinge~\cite{liGroupSparsityHinge2020} & 68.83 & 66.34 & -2.49 & 40.81 & 13.44 & 67.06 & 0.27 & 0.09 & 66.36 \\
2.2.1 & 2022 & GCNP~\cite{jiangChannelPruningUsing2022} & 68.38 & 66.14 & -2.24 & 40.81 & 16.38 & 59.87 & 0.27 & 0.14 & 49.42 \\
2.6.2 & 2019 & TAS~\cite{dongNetworkPruningTransformable2019} & 68.69 & 68.90 & 0.21 & 40.81 & 22.45 & 45.00 & 0.27 & - & - \\
2.2.1 & 2022 & GCNP~\cite{jiangChannelPruningUsing2022} & 68.38 & 68.95 & 0.57 & 40.81 & 34.84 & 14.64 & 0.27 & 0.25 & 8.16 \\
\midrule
\multicolumn{3}{l}{ResNet-32} \\
\midrule
2.4.1 & 2019 & ED~\cite{wangEigenDamageStructuredPruning2019} & 78.17 & 65.72 & -12.45 & 69.12 & 3.72 & 94.62 & 0.47 & - & - \\
2.4.1 & 2022 & SOSP~\cite{nonnenmacherSOSPEfficientlyCapturing2022} & 76.80 & 75.33 & -1.47 & 69.12 & 17.78 & 74.28 & 0.47 & - & - \\
2.4.1 & 2019 & ED~\cite{wangEigenDamageStructuredPruning2019} & 78.17 & 75.51 & -2.66 & 69.12 & 19.62 & 71.62 & 0.47 & - & - \\
2.4.1 & 2022 & SOSP~\cite{nonnenmacherSOSPEfficientlyCapturing2022} & 76.80 & 75.52 & -1.28 & 69.12 & 19.63 & 71.60 & 0.47 & - & - \\
2.5.1 & 2021 & DCP-CAC~\cite{chenDynamicalChannelPruning2021} & 68.48 & 68.11 & -0.37 & 69.12 & 34.49 & 50.10 & 0.47 & 0.25 & 47.83 \\
2.6.2 & 2022 & DAIS~\cite{guanDAISAutomaticChannel2022} & 73.24 & 72.20 & -1.04 & 69.12 & 39.47 & 42.90 & 0.47 & - & - \\
2.6.2 & 2019 & TAS~\cite{dongNetworkPruningTransformable2019} & 70.61 & 72.41 & 1.80 & 69.12 & 42.51 & 38.50 & 0.47 & - & - \\
2.1.2 & 2019 & COP~\cite{wangCOPCustomizedDeep2019} & 68.74 & 68.29 & -0.45 & 69.12 & 45.48 & 34.20 & 0.47 & 0.30 & 35.20 \\
2.5.1 & 2021 & DCP-CAC~\cite{chenDynamicalChannelPruning2021} & 68.48 & 69.51 & 1.03 & 69.12 & 48.35 & 30.04 & 0.47 & 0.35 & 26.09 \\
\midrule
\multicolumn{3}{l}{ResNet-44} \\
\midrule
2.5.1 & 2021 & DCP-CAC~\cite{chenDynamicalChannelPruning2021} & 69.87 & 69.82 & -0.05 & 97.15 & 48.54 & 50.04 & 0.66 & 0.35 & 47.69 \\
2.5.1 & 2021 & DCP-CAC~\cite{chenDynamicalChannelPruning2021} & 69.87 & 70.85 & 0.98 & 97.15 & 67.97 & 30.04 & 0.66 & 0.46 & 30.77 \\
\midrule
\multicolumn{3}{l}{ResNet-56} \\
\midrule
2.3.3 & 2019 & OICSR~\cite{liOICSROutInChannelSparsity2019} & 75.87 & 73.10 & -2.77 & 125.75 & 3.52 & 97.20 & 0.86 & - & - \\
2.3.3 & 2019 & OICSR~\cite{liOICSROutInChannelSparsity2019} & 75.87 & 75.75 & -0.12 & 125.75 & 17.35 & 86.20 & 0.86 & - & - \\
2.6.2 & 2022 & DAIS~\cite{guanDAISAutomaticChannel2022} & 71.76 & 72.57 & 0.81 & 125.75 & 58.35 & 53.60 & 0.86 & - & - \\
2.2.1 & 2021 & LRMF~\cite{zhangFilterPruningLearned2021} & - & - & -0.44 & 125.75 & 59.61 & 52.60 & 0.86 & - & - \\
2.2.1 & 2022 & GCNP~\cite{jiangChannelPruningUsing2022} & 72.86 & 72.22 & -0.64 & 125.75 & 60.08 & 52.22 & 0.86 & 0.52 & 39.83 \\
2.6.2 & 2020 & LFPC~\cite{heLearningFilterPruning2020} & 70.25 & 70.83 & 0.58 & 125.75 & 60.86 & 51.60 & 0.86 & - & - \\
2.6.2 & 2019 & TAS~\cite{dongNetworkPruningTransformable2019} & 73.18 & 72.25 & -0.93 & 125.75 & 61.24 & 51.30 & 0.86 & - & - \\
2.5.1 & 2021 & DCP-CAC~\cite{chenDynamicalChannelPruning2021} & 70.90 & 70.10 & -0.80 & 125.75 & 62.82 & 50.04 & 0.86 & 0.44 & 49.41 \\
2.4.2 & 2022 & EKG~\cite{leeEnsembleKnowledgeGuided2022} & 72.62 & 72.93 & 0.31 & 125.75 & 62.88 & 50.00 & 0.86 & - & - \\
2.2.1 & 2022 & GCNP~\cite{jiangChannelPruningUsing2022} & 72.86 & 72.86 & 0.00 & 125.75 & 64.42 & 48.77 & 0.86 & 0.52 & 39.24 \\
2.3.3 & 2019 & OICSR~\cite{liOICSROutInChannelSparsity2019} & 75.87 & 76.23 & 0.36 & 125.75 & 77.34 & 38.50 & 0.86 & - & - \\
2.7.3 & 2019 & SDN~\cite{chenShallowingDeepNetworks2019} & 70.01 & 69.78 & -0.23 & 125.75 & 77.59 & 38.30 & 0.86 & 0.55 & 36.10 \\
2.5.1 & 2021 & DCP-CAC~\cite{chenDynamicalChannelPruning2021} & 70.90 & 71.31 & 0.41 & 125.75 & 88.01 & 30.01 & 0.86 & 0.60 & 30.59 \\
2.2.3 & 2022 & DLRFC~\cite{heFilterPruningFeature2022} & 71.14 & 71.41 & -0.27 & 125.75 & 93.68 & 25.50 & 0.86 & 0.64 & 25.90 \\
2.3.1 & 2020 & PR~\cite{zhuangNeuronlevelStructuredPruning2020} & 72.49 & 72.46 & 0.06 & 125.75 & 94.31 & 25.00 & 0.86 & - & - \\
\midrule
\multicolumn{3}{l}{ResNet-110} \\
\midrule
2.6.2 & 2022 & DAIS~\cite{guanDAISAutomaticChannel2022} & 75.34 & 74.69 & -0.65 & 253.15 & 109.61 & 56.70 & 1.73 & - & - \\
2.6.2 & 2019 & TAS~\cite{dongNetworkPruningTransformable2019} & 75.06 & 73.16 & -1.90 & 253.15 & 119.99 & 52.60 & 1.73 & - & - \\
2.5.1 & 2021 & DCP-CAC~\cite{chenDynamicalChannelPruning2021} & 72.53 & 72.16 & -0.37 & 253.15 & 126.52 & 50.02 & 1.73 & 0.89 & 48.84 \\
2.5.1 & 2021 & DCP-CAC~\cite{chenDynamicalChannelPruning2021} & 72.53 & 72.79 & 0.26 & 253.15 & 176.97 & 30.09 & 1.73 & 1.23 & 29.07 \\
\midrule
\multicolumn{3}{l}{ResNet-164} \\
\midrule
2.3.1 & 2020 & SCP~\cite{kangOperationAwareSoftChannel2020} & 77.24 & 75.05 & 2.19 & 247.65 & 86.85 & 64.93 & 1.70 & 0.79 & 53.30 \\
2.3.1 & 2017 & NS~\cite{liuLearningEfficientConvolutional2017} & 76.63 & 76.09 & -0.54 & 247.65 & 122.34 & 50.60 & 1.70 & 1.19 & 30.06 \\
2.3.1 & 2020 & SCP~\cite{kangOperationAwareSoftChannel2020} & 77.24 & 76.62 & 0.62 & 247.65 & 135.32 & 45.36 & 1.70 & 1.21 & 28.89 \\
2.7.2 & 2020 & Hinge~\cite{liGroupSparsityHinge2020} & 76.78 & 76.88 & 0.10 & 247.65 & 137.00 & 44.68 & 1.70 & 1.30 & 23.43 \\
2.3.1 & 2017 & NS~\cite{liuLearningEfficientConvolutional2017} & 76.63 & 77.13 & 0.50 & 247.65 & 164.93 & 33.40 & 1.70 & 1.43 & 15.61 \\
2.6.2 & 2019 & TAS~\cite{dongNetworkPruningTransformable2019} & 78.29 & 77.76 & -0.53 & 247.65 & 171.13 & 30.90 & 1.70 & - & - \\
2.4.2 & 2019 & VP~\cite{zhaoVariationalConvolutionalNeural2019} & 75.56 & 73.76 & -1.80 & 247.65 & 180.18 & 27.24 & 1.70 & 1.40 & 17.86 \\
\bottomrule
\end{tabularx}

\captionof{table}{ResNet-20/32/44/56/110/164 on CIFAR-100.}
\end{strip}

==> tables/cifar100/VGG-16.tex <==
\begin{strip}
\centering
\scriptsize
\begin{tabularx}{\textwidth}{@{}>{\hsize=0.067\hsize}X>{\hsize=0.067\hsize}X>{\hsize=0.2\hsize}X>{\hsize=0.067\hsize}X>{\hsize=0.067\hsize}X>{\hsize=0.067\hsize}X>{\hsize=0.067\hsize}X>{\hsize=0.067\hsize}X>{\hsize=0.067\hsize}X>{\hsize=0.067\hsize}X>{\hsize=0.067\hsize}X>{\hsize=0.067\hsize}X>{\hsize=0.067\hsize}X@{}}
\toprule
\tabletitle \\
\midrule
\multicolumn{3}{l}{VGG-16} \\
\midrule
2.3.1 & 2020 & SCP~\cite{kangOperationAwareSoftChannel2020} & 73.51 & 69.96 & 3.55 & 314.59 & 65.31 & 79.24 & 14.73 & 0.88 & 94.01 \\
2.2.1 & 2022 & GCNP~\cite{jiangChannelPruningUsing2022} & 72.00 & 71.64 & -0.36 & 314.59 & 99.91 & 68.24 & 14.73 & 1.70 & 88.46 \\
2.2.1 & 2022 & GCNP~\cite{jiangChannelPruningUsing2022} & 72.00 & 72.00 & 0.00 & 314.59 & 136.59 & 56.58 & 14.73 & 2.87 & 80.49 \\
2.3.1 & 2020 & SCP~\cite{kangOperationAwareSoftChannel2020} & 73.51 & 73.86 & -0.35 & 314.59 & 152.73 & 51.45 & 14.73 & 2.93 & 80.14 \\
2.2.3 & 2022 & DLRFC~\cite{heFilterPruningFeature2022} & 73.54 & 74.09 & -0.55 & 314.59 & 178.06 & 43.40 & 14.73 & 2.58 & 82.50 \\
2.1.2 & 2019 & COP~\cite{wangCOPCustomizedDeep2019} & 72.59 & 71.77 & -0.82 & 314.59 & 179.00 & 43.10 & 14.73 & 3.95 & 73.20 \\
2.3.1 & 2020 & PR~\cite{zhuangNeuronlevelStructuredPruning2020} & 73.83 & 74.25 & -0.42 & 314.59 & 179.32 & 43.00 & 14.73 & - & - \\
2.2.1 & 2021 & LRMF~\cite{zhangFilterPruningLearned2021} & - & - & 0.50 & 314.59 & 201.65 & 35.90 & 14.73 & - & - \\
2.7.1 & 2020 & EB~\cite{youDrawingEarlyBirdTickets2020} & - & 71.28 & - & 314.59 & 209.73 & 33.33 & 14.73 & 7.37 & 50.00 \\
2.7.3 & 2019 & SDN~\cite{chenShallowingDeepNetworks2019} & 72.38 & 73.43 & 1.05 & 314.59 & 211.09 & 32.90 & 14.73 & 3.11 & 78.90 \\
2.4.2 & 2019 & VP~\cite{zhaoVariationalConvolutionalNeural2019} & 73.26 & 73.33 & 0.07 & 314.59 & 257.30 & 18.21 & 14.73 & 9.15 & 37.87 \\
2.7.1 & 2020 & EB~\cite{youDrawingEarlyBirdTickets2020} & - & 72.17 & - & 314.59 & 262.16 & 16.67 & 14.73 & 10.31 & 30.00 \\
2.7.1 & 2020 & EB~\cite{youDrawingEarlyBirdTickets2020} & - & 71.81 & - & 314.59 & 285.99 & 9.09 & 14.73 & 13.26 & 10.00 \\
2.7.1 & 2022 & EarlyCroP~\cite{rachwanWinningLotteryAhead2022} & - & 62.20 & - & 314.59 & - & - & 14.73 & 0.31 & 97.90 \\
2.7.3 & 2022 & DPP~\cite{gonzalez-carabarinDynamicProbabilisticPruning2022} & 70.32 & 70.40 & 0.08 & 314.59 & - & - & 14.73 & 2.77 & 81.20 \\
\midrule
\multicolumn{3}{l}{VGG-19} \\
\midrule
2.3.3 & 2021 & GREG~\cite{wangNeuralPruningGrowing2022} & 74.02 & 67.55 & -6.47 & 398.00.00 & 45.01 & 88.69 & 20.04 & - & - \\
2.3.3 & 2021 & GREG~\cite{wangNeuralPruningGrowing2022} & 74.02 & 67.75 & -6.27 & 398.00 & 45.01 & 88.69 & 20.04 & - & - \\
2.4.1 & 2019 & ED~\cite{wangEigenDamageStructuredPruning2019} & 73.08 & 64.91 & -8.17 & 398.00 & 45.17 & 88.65 & 20.04 & - & - \\
2.4.1 & 2019 & ED~\cite{wangEigenDamageStructuredPruning2019} & 73.34 & 65.18 & -8.16 & 398.00 & 45.25 & 88.63 & 20.04 & - & - \\
2.5.1 & 2021 & SEP~\cite{dingWherePruneUsing2021} & 73.16 & 73.47 & 0.31 & 398.00 & 117.00 & 70.60 & 20.04 & 5.95 & 70.31 \\
2.3.1 & 2020 & SCP~\cite{kangOperationAwareSoftChannel2020} & 72.56 & 72.15 & 0.41 & 398.00 & 151.48 & 61.94 & 20.04 & 2.13 & 89.37 \\
2.4.1 & 2022 & SOSP~\cite{nonnenmacherSOSPEfficientlyCapturing2022} & 73.45 & 73.11 & -0.34 & 398.00 & 192.59 & 51.61 & 20.04 & - & - \\
2.4.1 & 2022 & SOSP~\cite{nonnenmacherSOSPEfficientlyCapturing2022} & 73.45 & 73.17 & -0.28 & 398.00 & 219.42 & 44.87 & 20.04 & - & - \\
2.3.1 & 2020 & SCP~\cite{kangOperationAwareSoftChannel2020} & 72.56 & 72.99 & -0.43 & 398.00 & 235.14 & 40.92 & 20.04 & 4.50 & 77.52 \\
2.4.1 & 2019 & ED~\cite{wangEigenDamageStructuredPruning2019} & 73.08 & 73.01 & -0.07 & 398.00 & 248.91 & 37.46 & 20.04 & - & - \\
2.4.1 & 2019 & ED~\cite{wangEigenDamageStructuredPruning2019} & 73.34 & 72.90 & -0.44 & 398.00 & 249.15 & 37.40 & 20.04 & - & - \\
2.3.1 & 2017 & NS~\cite{liuLearningEfficientConvolutional2017} & 73.26 & 73.48 & 0.22 & 398.00 & 250.19 & 37.14 & 20.04 & 4.99 & 75.10 \\
2.5.1 & 2021 & DCP-CAC~\cite{chenDynamicalChannelPruning2021} & 70.17 & 72.28 & 2.11 & 398.00 & 251.00 & 36.93 & 20.04 & 8.93 & 55.44 \\
2.7.1 & 2022 & ProsPr~\cite{alizadehProspectPruningFinding2022} & 72.50 & 72.29 & -0.21 & 398.00 & - & - & 20.04 & 4.01 & 80.00 \\
2.7.1 & 2022 & ProsPr~\cite{alizadehProspectPruningFinding2022} & 73.50 & 71.12 & -2.38 & 398.00 & - & - & 20.04 & 2.00 & 90.00 \\
2.7.1 & 2022 & ProsPr~\cite{alizadehProspectPruningFinding2022} & 74.50 & 68.03 & -6.47 & 398.00 & - & - & 20.04 & 1.00 & 95.00 \\
\bottomrule
\end{tabularx}

\captionof{table}{VGG-16/19 on CIFAR-100.}
\end{strip}

==> tables/imagenet/AlexNet.tex <==
\begin{strip}
\centering
\scriptsize
\begin{tabularx}{\textwidth}{@{}>{\hsize=0.067\hsize}X>{\hsize=0.067\hsize}X>{\hsize=0.2\hsize}X>{\hsize=0.067\hsize}X>{\hsize=0.067\hsize}X>{\hsize=0.067\hsize}X>{\hsize=0.067\hsize}X>{\hsize=0.067\hsize}X>{\hsize=0.067\hsize}X>{\hsize=0.067\hsize}X>{\hsize=0.067\hsize}X>{\hsize=0.067\hsize}X>{\hsize=0.067\hsize}X@{}}
\toprule
\tabletitle \\
\midrule
\multicolumn{3}{l}{AlexNet} \\
\midrule
2.3.3 & 2019 & OICSR~\cite{liOICSROutInChannelSparsity2019} & 56.98 & 53.78 & -3.20 & 7270.00 & 2304.59 & 68.30 & 17.69 & - & - \\
2.2.3 & 2018 & NISP~\cite{yuNISPPruningNetworks2018a} & - & - & 1.43 & 7270.00 & 2337.30 & 67.85 & 17.69 & 11.72 & 33.77 \\
2.5.1 & 2018 & GDP-Lin~\cite{linAcceleratingConvolutionalNetworks2018} & 56.60 & 54.82 & -1.78 & 7270.00 & 2621.26 & 63.94 & 17.69 & - & - \\
2.2.3 & 2018 & NISP~\cite{yuNISPPruningNetworks2018a} & - & - & 0.97 & 7270.00 & 2712.44 & 62.69 & 17.69 & 17.34 & 1.96 \\
2.3.3 & 2019 & OICSR~\cite{liOICSROutInChannelSparsity2019} & 56.98 & 56.83 & -0.15 & 7270.00 & 3344.20 & 54.00 & 17.69 & - & - \\
2.2.3 & 2018 & NISP~\cite{yuNISPPruningNetworks2018a} & - & - & 0.54 & 7270.00 & 3366.01 & 53.70 & 17.69 & 17.18 & 2.91 \\
2.5.1 & 2018 & GDP-Lin~\cite{linAcceleratingConvolutionalNetworks2018} & 56.60 & 55.83 & -0.77 & 7270.00 & 3469.12 & 52.28 & 17.69 & - & - \\
2.2.2 & 2019 & AOFP~\cite{dingApproximatedOracleFilter2019} & 55.71 & 56.17 & 0.46 & 7270.00 & 4268.31 & 41.29 & 17.69 & - & - \\
2.2.3 & 2018 & NISP~\cite{yuNISPPruningNetworks2018a} & - & - & 0.00 & 7270.00 & 4353.28 & 40.12 & 17.69 & 9.36 & 47.09 \\
2.5.1 & 2018 & GDP-Lin~\cite{linAcceleratingConvolutionalNetworks2018} & 56.60 & 56.46 & -0.14 & 7270.00 & 4535.16 & 37.62 & 17.69 & - & - \\
2.2.2 & 2019 & AOFP~\cite{dingApproximatedOracleFilter2019} & 55.71 & 56.54 & 0.83 & 7270.00 & 5014.39 & 31.03 & 17.69 & - & - \\
2.3.3 & 2019 & OICSR~\cite{liOICSROutInChannelSparsity2019} & 56.98 & 57.87 & 0.89 & 7270.00 & 5568.82 & 23.40 & 17.69 & - & - \\
\bottomrule
\end{tabularx}

\captionof{table}{AlexNet on ImageNet-1K.}
\end{strip}

==> tables/imagenet/MobileNet.tex <==
\begin{strip}
\centering
\scriptsize
\begin{tabularx}{\textwidth}{@{}>{\hsize=0.067\hsize}X>{\hsize=0.067\hsize}X>{\hsize=0.2\hsize}X>{\hsize=0.067\hsize}X>{\hsize=0.067\hsize}X>{\hsize=0.067\hsize}X>{\hsize=0.067\hsize}X>{\hsize=0.067\hsize}X>{\hsize=0.067\hsize}X>{\hsize=0.067\hsize}X>{\hsize=0.067\hsize}X>{\hsize=0.067\hsize}X>{\hsize=0.067\hsize}X@{}}
\toprule
\tabletitle \\
\midrule
\multicolumn{3}{l}{MobileNet-V1} \\
\midrule
2.6.3 & 2019 & MetaPruning~\cite{liuMetaPruningMetaLearning2019} & 70.60 & 57.20 & -13.40 & 569.00 & 41.00 & 92.79 & 4.20 & - & - \\
2.6.3 & 2019 & MetaPruning~\cite{liuMetaPruningMetaLearning2019} & 70.60 & 66.10 & -4.50 & 569.00 & 149.00 & 73.81 & 4.20 & - & - \\
2.5.1 & 2022 & SMCP~\cite{humbleSoftMaskingCostConstrained2022} & 72.60 & 68.30 & -4.30 & 569.00 & 208.00 & 63.44 & 4.20 & - & - \\
2.6.1 & 2018 & AMC~\cite{heAMCAutoMLModel2018} & 70.60 & 68.90 & -1.70 & 569.00 & 227.60 & 60.00 & 4.20 & - & - \\
2.6.1 & 2021 & AGMC~\cite{yuAutoGraphEncoderDecoder2021} & 70.60 & 69.40 & -1.20 & 569.00 & 227.60 & 60.00 & 4.20 & - & - \\
2.6.1 & 2022 & GNN-RL~\cite{yuTopologyAwareNetworkPruning2022} & 70.90 & 69.50 & -1.40 & 569.00 & 227.60 & 60.00 & 4.20 & - & - \\
2.3.1 & 2020 & EagleEye~\cite{liEagleEyeFastSubnet2020} & - & 70.90 & - & 569.00 & 284.00 & 50.09 & 4.20 & - & - \\
2.4.3 & 2022 & RollBack~\cite{fanBayesianOptimizationClustering2022} & - & 49.34 & - & 569.00 & 284.50 & 50.00 & 4.20 & - & - \\
2.5.2 & 2020 & DRLP~\cite{chenStorageEfficientDynamic2020} & 70.90 & 70.60 & -0.30 & 569.00 & 284.50 & 50.00 & 4.20 & - & - \\
2.6.1 & 2018 & AMC~\cite{heAMCAutoMLModel2018} & 70.60 & 70.20 & -0.40 & 569.00 & 284.50 & 50.00 & 4.20 & - & - \\
2.6.3 & 2019 & MetaPruning~\cite{liuMetaPruningMetaLearning2019} & 70.60 & 70.90 & 0.30 & 569.00 & 324.00 & 43.06 & 4.20 & - & - \\
2.5.2 & 2022 & FTWT~\cite{elkerdawyFireTogetherWire2022} & 69.57 & 69.66 & 0.09 & 569.00 & 335.31 & 41.07 & 4.20 & - & - \\
2.5.1 & 2022 & SMCP~\cite{humbleSoftMaskingCostConstrained2022} & 72.60 & 71.00 & -1.60 & 569.00 & 356.00 & 37.43 & 4.20 & - & - \\
2.7.3 & 2022 & 1xN~\cite{lin1xNPatternPruning2022} & 71.15 & 70.28 & -0.87 & 569.00 & - & - & 4.20 & 2.10 & 50 \\
\midrule
\multicolumn{3}{l}{MobileNet-V2} \\
\midrule
2.6.3 & 2019 & MetaPruning~\cite{liuMetaPruningMetaLearning2019} & 74.70 & 58.30 & -16.40 & 300.00& 22.05 & 92.65 & 3.50 & - & - \\
2.6.2 & 2020 & DMCP~\cite{guoDMCPDifferentiableMarkov2020} & 72.30 & 59.10 & -13.30 & 300.00& 43.00 & 85.67 & 3.50 & - & - \\
2.6.3 & 2019 & MetaPruning~\cite{liuMetaPruningMetaLearning2019} & 74.70 & 63.80 & -10.90 & 300.00& 43.08 & 85.64 & 3.50 & - & - \\
2.6.3 & 2019 & MetaPruning~\cite{liuMetaPruningMetaLearning2019} & 74.70 & 65.00 & -9.70 & 300.00& 53.85 & 82.05 & 3.50 & - & - \\
2.6.2 & 2020 & DMCP~\cite{guoDMCPDifferentiableMarkov2020} & 72.30 & 62.70 & -9.70 & 300.00& 59.00 & 80.33 & 3.50 & - & - \\
2.6.3 & 2019 & MetaPruning~\cite{liuMetaPruningMetaLearning2019} & 74.70 & 67.30 & -7.40 & 300.00& 63.59 & 78.80 & 3.50 & - & - \\
2.6.3 & 2019 & MetaPruning~\cite{liuMetaPruningMetaLearning2019} & 74.70 & 68.20 & -6.50 & 300.00& 71.79 & 76.07 & 3.50 & - & - \\
2.6.2 & 2020 & DMCP~\cite{guoDMCPDifferentiableMarkov2020} & 72.30 & 66.10 & -6.30 & 300.00& 87.00 & 71.00 & 3.50 & - & - \\
2.4.1 & 2021 & GFP~\cite{liuGroupFisherPruning2021} & 75.74 & 65.94 & -9.80 & 300.00& 90.00 & 70.00 & 3.50 & - & - \\
2.6.2 & 2022 & DNCP~\cite{zhengModelCompressionBased2022} & 72.30 & 66.50 & -5.80 & 300.00& 97.00 & 67.67 & 3.50 & - & - \\
2.6.2 & 2020 & DMCP~\cite{guoDMCPDifferentiableMarkov2020} & 72.30 & 67.00 & -5.30 & 300.00& 97.00 & 67.67 & 3.50 & - & - \\
2.2.2 & 2020 & GFS~\cite{yeGoodSubnetworksProvably2020} & 72.00 & 66.90 & -5.10 & 300.00& 102.23 & 65.92 & 3.50 & 1.90 & 45.71 \\
2.2.2 & 2020 & GFS~\cite{yeGoodSubnetworksProvably2020} & 72.00 & 68.80 & -3.20 & 300.00& 131.85 & 56.05 & 3.50 & 2.00 & 42.86 \\
2.2.2 & 2020 & GFS~\cite{yeGoodSubnetworksProvably2020} & 72.00 & 69.70 & -2.30 & 300.00& 145.22 & 51.59 & 3.50 & 2.20 & 37.14 \\
2.5.2 & 2021 & ManiDP~\cite{tangManifoldRegularizedDynamic2021} & 71.80 & 69.62 & -2.18 & 300.00& 146.40 & 51.20 & 3.50 & - & - \\
2.6.3 & 2019 & MetaPruning~\cite{liuMetaPruningMetaLearning2019} & 74.70 & 72.70 & -2.00 & 300.00& 149.23 & 50.26 & 3.50 & - & - \\
2.4.1 & 2021 & GFP~\cite{liuGroupFisherPruning2021} & 75.74 & 69.16 & -6.58 & 300.00& 150.00 & 50.00 & 3.50 & - & - \\
2.3.2 & 2020 & DMC~\cite{gaoDiscreteModelCompression2020} & 71.88 & 68.37 & -3.51 & 300.00& 162.00 & 46.00 & 3.50 & - & - \\
2.2.2 & 2020 & GFS~\cite{yeGoodSubnetworksProvably2020} & 72.00 & 70.40 & -1.60 & 300.00& 162.42 & 45.86 & 3.50 & 2.30 & 34.29 \\
2.5.2 & 2021 & DDG~\cite{liDynamicDualGating2021} & 71.88 & 71.62 & -0.26 & 300.00& 168.00 & 44.00 & 3.50 & - & - \\
2.6.1 & 2022 & GNN-RL~\cite{yuTopologyAwareNetworkPruning2022} & 71.87 & 70.04 & -1.83 & 300.00& 174.00 & 42.00 & 3.50 & - & - \\
2.4.2 & 2019 & RBP~\cite{zhouAccelerateCNNRecursive2019} & - & 69.70 & - & 300.00& 176.47 & 41.18 & 3.50 & - & - \\
2.4.3 & 2022 & RollBack~\cite{fanBayesianOptimizationClustering2022} & - & 52.86 & - & 300.00& 180.00 & 40.00 & 3.50 & - & - \\
2.5.2 & 2021 & ManiDP~\cite{tangManifoldRegularizedDynamic2021} & 71.80 & 71.42 & -0.38 & 300.00& 188.40 & 37.20 & 3.50 & - & - \\
2.2.2 & 2020 & GFS~\cite{yeGoodSubnetworksProvably2020} & 72.00 & 71.20 & -0.80 & 300.00& 192.04 & 35.99 & 3.50 & 2.70 & 22.86 \\
2.6.1 & 2021 & AGMC~\cite{yuAutoGraphEncoderDecoder2021} & 71.80 & 70.87 & -0.93 & 300.00& 210.00 & 30.00 & 3.50 & - & - \\
2.2.3 & 2022 & DLRFC~\cite{heFilterPruningFeature2022} & 71.80 & 71.88 & -0.08 & 300.00& 210.0 & 30.00 & - & - & - \\
2.6.1 & 2018 & AMC~\cite{heAMCAutoMLModel2018} & 71.80 & 70.80 & -1.00 & 300.00& 210.00 & 30.00 & 3.50 & - & - \\
2.2.2 & 2020 & GFS~\cite{yeGoodSubnetworksProvably2020} & 72.00 & 71.60 & -0.40 & 300.00& 210.19 & 29.94 & 3.50 & 2.90 & 17.14 \\
2.6.2 & 2022 & DNCP~\cite{zhengModelCompressionBased2022} & 72.30 & 72.70 & 0.40 & 300.00& 211.00 & 29.67 & 3.50 & - & - \\
2.6.2 & 2020 & DMCP~\cite{guoDMCPDifferentiableMarkov2020} & 72.30 & 73.50 & 1.20 & 300.00& 211.00 & 29.67 & 3.50 & - & - \\
2.6.2 & 2020 & DMCP~\cite{guoDMCPDifferentiableMarkov2020} & 72.30 & 72.40 & 0.10 & 300.00& 211.00 & 29.67 & 3.50 & - & - \\
2.6.2 & 2022 & DDNP~\cite{gaoDisentangledDifferentiableNetwork2022} & 72.05 & 72.20 & 0.15 & 300.00& 211.50 & 29.50 & 3.50 & - & - \\
2.7.1 & 2022 & RRCP~\cite{liRevisitingRandomChannel2022} & - & 70.90 & - & 300.00& 212.61 & 29.13 & 3.50 & - & - \\
2.7.2 & 2021 & CC~\cite{liCompactCNNsCollaborative2021} & 71.88 & 70.91 & -0.97 & 300.00& 215.00 & 28.33 & 3.50 & - & - \\
2.3.1 & 2020 & PR~\cite{zhuangNeuronlevelStructuredPruning2020} & 72.00 & 71.80 & 0.20 & 300.00& 216.00 & 28.00 & 3.50 & - & - \\
2.2.2 & 2020 & GFS~\cite{yeGoodSubnetworksProvably2020} & 72.00 & 71.90 & -0.10 & 300.00& 246.50 & 17.83 & 3.50 & 3.20 & 8.57 \\
2.6.2 & 2020 & DMCP~\cite{guoDMCPDifferentiableMarkov2020} & 72.30 & 73.90 & 1.60 & 300.00& 300.00 & 0.00 & 3.50 & - & - \\
2.6.2 & 2020 & DMCP~\cite{guoDMCPDifferentiableMarkov2020} & 72.30 & 74.60 & 2.30 & 300.00& 300.00 & 0.00 & 3.50 & - & - \\
2.7.3 & 2022 & 1xN~\cite{lin1xNPatternPruning2022} & 71.74 & 70.23 & -1.50 & 300.00& - & - & 3.50 & 1.75 & 50 \\
\midrule
\multicolumn{3}{l}{MobileNet-V3-Small} \\
\midrule
2.2.2 & 2020 & GFS~\cite{yeGoodSubnetworksProvably2020} & 67.50 & 65.80 & -1.70 & - & - & 23.44 & - & - & 20.00 \\
% \midrule
\bottomrule
\end{tabularx}

\captionof{table}{MobileNet-V1/V2/V3-Small on ImageNet-1K.}
\end{strip}

==> tables/imagenet/Other.tex <==
\begin{strip}
\setlength{\tabcolsep}{0.4em} 
\centering
\scriptsize
\begin{tabularx}{\textwidth}{@{}>{\hsize=0.067\hsize}X>{\hsize=0.067\hsize}X>{\hsize=0.2\hsize}X>{\hsize=0.067\hsize}X>{\hsize=0.067\hsize}X>{\hsize=0.067\hsize}X>{\hsize=0.067\hsize}X>{\hsize=0.067\hsize}X>{\hsize=0.067\hsize}X>{\hsize=0.067\hsize}X>{\hsize=0.067\hsize}X>{\hsize=0.067\hsize}X>{\hsize=0.067\hsize}X@{}}
\toprule
\tabletitle \\
\midrule
\multicolumn{3}{l}{ProxylessNet-Mobile} \\
\midrule
2.2.2 & 2020 & GFS~\cite{yeGoodSubnetworksProvably2020} & 74.60 & 74.00 & -0.60 & 324.00 & 232.00 & 28.40 & 4.10 & 3.40 & 17.07 \\
\midrule
\multicolumn{3}{l}{GoogLeNet} \\
\midrule
2.2.3 & 2018 & NISP~\cite{yuNISPPruningNetworks2018a} & - & - & 0.21 & 1560.00 & 649.90 & 58.34 & 6.80 & 4.50 & 33.76 \\
\midrule
\multicolumn{3}{l}{ResNeXt-50} \\
\midrule
2.4.1 & 2021 & GFP~\cite{liuGroupFisherPruning2021} & 77.97 & 77.53 & -0.44 & 4230.00 & 2110.00 & 50.12 & 25.02 & - & - \\
\midrule
\multicolumn{3}{l}{NAS} \\
\midrule
2.7.2 & 2021 & NPAS~\cite{liNPASCompilerAwareFramework2021} & - & 68.30 & - & - & 98.00 & - & - & 2.80 & - \\
2.7.1 & 2022 & SuperTickets~\cite{youSuperTicketsDrawingTaskAgnostic2022} & - & 74.20 & - & - & 125 & - & - & 2.70 & - \\
2.7.2 & 2021 & NPAS~\cite{liNPASCompilerAwareFramework2021} & - & 70.90 & - & - & 147.00 & - & - & 3.00 & - \\
2.7.2 & 2021 & NPAS~\cite{liNPASCompilerAwareFramework2021} & - & 75.00 & - & - & 201.00 & - & - & 3.50 & - \\
2.7.2 & 2021 & NPAS~\cite{liNPASCompilerAwareFramework2021} & - & 78.20 & - & - & 385.00 & - & - & 5.30 & - \\
2.6.2 & 2022 & ReCNAS~\cite{pengReCNASResourceConstrainedNeural2022} & - & 76.90 & - & - & - & - & - & 6.30 & - \\
2.6.2 & 2022 & ReCNAS~\cite{pengReCNASResourceConstrainedNeural2022} & - & 75.20 & - & - & - & - & - & 5.20 & - \\
2.6.2 & 2022 & ReCNAS~\cite{pengReCNASResourceConstrainedNeural2022} & - & 77.10 & - & - & - & - & - & 6.80 & - \\
\bottomrule
\end{tabularx}

\captionof{table}{Other models on ImageNet-1K, including ProxylessNet-Mobile, GoogLeNet, ResNeXt-50, and models searched by Neural Architecture Search (NAS).}
\end{strip}

==> tables/imagenet/ResNet-101.tex <==
\begin{strip}
\centering
\scriptsize
\begin{tabularx}{\textwidth}{@{}>{\hsize=0.067\hsize}X>{\hsize=0.067\hsize}X>{\hsize=0.2\hsize}X>{\hsize=0.067\hsize}X>{\hsize=0.067\hsize}X>{\hsize=0.067\hsize}X>{\hsize=0.067\hsize}X>{\hsize=0.067\hsize}X>{\hsize=0.067\hsize}X>{\hsize=0.067\hsize}X>{\hsize=0.067\hsize}X>{\hsize=0.067\hsize}X>{\hsize=0.067\hsize}X@{}}
\toprule
\tabletitle \\
\midrule
\multicolumn{3}{l}{ResNet-101} \\
\midrule
2.4.1 & 2019 & Mol-19~\cite{molchanovImportanceEstimationNeural2019} & 77.37 & 74.16 & -3.21 & 7801.00 & 1760.23 & 77.44 & 44.55 & 13.55 & 69.57 \\
2.5.1 & 2022 & CHEX~\cite{houCHEXCHannelEXploration2022} & - & 77.60 & - & 7801.00 & 1957.98 & 74.90 & 44.55 & - & - \\
2.6.3 & 2020 & ABCPruner~\cite{linChannelPruningAutomatic2020} & 77.38 & 74.76 & -2.62 & 7801.00 & 1958.69 & 74.89 & 44.55 & 12.94 & 70.95 \\
2.5.1 & 2022 & SMCP~\cite{humbleSoftMaskingCostConstrained2022} & 77.40 & 76.80 & -0.60 & 7801.00 & 2000.26 & 74.36 & 44.55 & - & - \\
2.4.1 & 2019 & Mol-19~\cite{molchanovImportanceEstimationNeural2019} & 77.37 & 75.38 & -1.99 & 7801.00 & 2470.32 & 68.33 & 44.55 & 17.74 & 60.18 \\
2.5.1 & 2022 & SMCP~\cite{humbleSoftMaskingCostConstrained2022} & 77.40 & 77.30 & -0.10 & 7801.00 & 2600.33 & 66.67 & 44.55 & - & - \\
2.4.1 & 2019 & Mol-19~\cite{molchanovImportanceEstimationNeural2019} & 77.37 & 75.27 & -2.10 & 7801.00 & 2850.37 & 63.46 & 44.55 & 20.63 & 53.69 \\
2.3.2 & 2020 & SCOP~\cite{tangSCOPScientificControl2020} & 77.37 & 77.36 & -0.01 & 7801.00 & 3104.80 & 60.20 & 44.55 & 18.80 & 57.80 \\
2.6.3 & 2020 & ABCPruner~\cite{linChannelPruningAutomatic2020} & 77.38 & 75.82 & -1.56 & 7801.00 & 3137.80 & 59.78 & 44.55 & 17.72 & 60.22 \\
2.3.2 & 2020 & DMC~\cite{gaoDiscreteModelCompression2020} & 77.37 & 77.40 & 0.03 & 7801.00 & 3432.44 & 56.00 & 44.55 & - & - \\
2.5.1 & 2022 & CHEX~\cite{houCHEXCHannelEXploration2022} & - & 78.80 & - & 7801.00 & 3503.75 & 55.09 & 44.55 & - & - \\
2.5.1 & 2022 & SMCP~\cite{humbleSoftMaskingCostConstrained2022} & 77.40 & 77.80 & 0.40 & 7801.00 & 3600.46 & 53.85 & 44.55 & - & - \\
2.3.1 & 2018 & RSNLI~\cite{yeRethinkingSmallernormlessinformativeAssumption2018} & 76.40 & 74.56 & -1.84 & 7801.00 & 3690.47 & 52.69 & 44.55 & 17.37 & 61.00 \\
2.2.2 & 2019 & AOFP~\cite{dingApproximatedOracleFilter2019} & 76.63 & 76.40 & -0.23 & 7801.00 & 3885.04 & 50.20 & 44.55 & - & - \\
2.4.1 & 2021 & GFP~\cite{liuGroupFisherPruning2021} & 78.29 & 78.33 & 0.04 & 7801.00 & 3900.00 & 50.01 & 44.55 & - & - \\
2.3.1 & 2018 & RSNLI~\cite{yeRethinkingSmallernormlessinformativeAssumption2018} & 76.40 & 75.27 & -1.13 & 7801.00 & 3962.55 & 49.20 & 44.55 & 23.61 & 47.00 \\
2.5.1 & 2022 & SMCP~\cite{humbleSoftMaskingCostConstrained2022} & 77.40 & 78.10 & 0.70 & 7801.00 & 4000.51 & 48.72 & 44.55 & - & - \\
2.3.2 & 2020 & SCOP~\cite{tangSCOPScientificControl2020} & 77.37 & 77.75 & 0.38 & 7801.00 & 4009.71 & 48.60 & 44.55 & 23.70 & 46.80 \\
2.1.2 & 2019 & FPGM~\cite{heFilterPruningGeometric2019} & 77.37 & 77.32 & -0.05 & 7801.00 & 4134.53 & 47.00 & 44.55 & - & - \\
2.2.3 & 2020 & PFP~\cite{liebenweinProvableFilterPruning2020} & 77.37 & 76.43 & -0.94 & 7801.00 & 4284.31 & 45.08 & 44.55 & 22.07 & 50.45 \\
2.5.1 & 2018 & SFP~\cite{heSoftFilterPruning2018} & 77.37 & 77.51 & 0.14 & 7801.00 & 4508.98 & 42.20 & 44.55 & - & - \\
2.5.1 & 2018 & SFP~\cite{heSoftFilterPruning2018} & 77.37 & 77.03 & -0.34 & 7801.00 & 4508.98 & 42.20 & 44.55 & - & - \\
2.4.1 & 2019 & Mol-19~\cite{molchanovImportanceEstimationNeural2019} & 77.37 & 77.35 & -0.02 & 7801.00 & 4700.60 & 39.74 & 44.55 & 31.10 & 30.20 \\
2.2.2 & 2019 & AOFP~\cite{dingApproximatedOracleFilter2019} & 76.63 & 76.88 & 0.25 & 7801.00 & 5451.43 & 30.12 & 44.55 & - & - \\
2.2.3 & 2020 & PFP~\cite{liebenweinProvableFilterPruning2020} & 77.37 & 76.78 & -0.59 & 7801.00 & 5509.07 & 29.38 & 44.55 & 29.83 & 33.04 \\
2.6.3 & 2022 & EDropout~\cite{salehinejadEDropoutEnergyBasedDropout2022} & 75.94 & 73.94 & -2.00 & 7801.00 & - & - & 44.55 & 19.13 & 57.07 \\
\midrule
\multicolumn{3}{l}{ResNet-152} \\
\midrule
2.6.3 & 2020 & ABCPruner~\cite{linChannelPruningAutomatic2020} & 78.31 & 76.00 & -2.31 & 11514.00 & 2697.93 & 76.57 & 60.19 & 15.62 & 74.05 \\
2.2.2 & 2019 & AOFP~\cite{dingApproximatedOracleFilter2019} & 77.37 & 76.40 & -0.97 & 11514.00 & 2858.09 & 75.18 & 60.19 & - & - \\
2.2.2 & 2019 & AOFP~\cite{dingApproximatedOracleFilter2019} & 77.37 & 77.00 & -0.37 & 11514.00 & 4215.68 & 63.39 & 60.19 & - & - \\
2.6.3 & 2020 & ABCPruner~\cite{linChannelPruningAutomatic2020} & 78.31 & 77.12 & -1.19 & 11514.00 & 4275.39 & 62.87 & 60.19 & 24.07 & 60.01 \\
2.2.2 & 2019 & AOFP~\cite{dingApproximatedOracleFilter2019} & 77.37 & 77.47 & 0.10 & 11514.00 & 6246.96 & 45.74 & 60.19 & - & - \\
\bottomrule
\end{tabularx}

\captionof{table}{ResNet-101/152 on ImageNet-1K.}
\end{strip}

==> tables/imagenet/ResNet-18.tex <==
\begin{strip}
\centering
\scriptsize
\begin{tabularx}{\textwidth}{@{}>{\hsize=0.067\hsize}X>{\hsize=0.067\hsize}X>{\hsize=0.2\hsize}X>{\hsize=0.067\hsize}X>{\hsize=0.067\hsize}X>{\hsize=0.067\hsize}X>{\hsize=0.067\hsize}X>{\hsize=0.067\hsize}X>{\hsize=0.067\hsize}X>{\hsize=0.067\hsize}X>{\hsize=0.067\hsize}X>{\hsize=0.067\hsize}X>{\hsize=0.067\hsize}X@{}}
\toprule
\tabletitle \\
\midrule
\multicolumn{3}{l}{ResNet-18} \\
\midrule
2.5.2 & 2021 & DDG~\cite{liDynamicDualGating2021} & 69.76 & 69.38 & -0.38 & 1814.00 & 758.25 & 58.20 & 11.69 & - & - \\
2.5.2 & 2021 & ManiDP~\cite{tangManifoldRegularizedDynamic2021} & 69.76 & 68.35 & -1.41 & 1814.00 & 814.49 & 55.10 & 11.69 & - & - \\
2.7.3 & 2022 & SOKS~\cite{liuSOKSAutomaticSearching2022} & 70.42 & 69.16 & -1.26 & 1814.00 & 817.30 & 54.95 & 11.69 & 6.27 & 46.36 \\
2.7.3 & 2020 & SWP~\cite{mengPruningFilterFilter2020} & 69.76 & 69.72 & -0.04 & 1814.00 & 823.92 & 54.58 & 11.69 & - & - \\
2.2.1 & 2021 & LRMF~\cite{zhangFilterPruningLearned2021} & 70.28 & 67.87 & -2.41 & 1814.00 & 847.14 & 53.30 & 11.69 & - & - \\
2.6.2 & 2022 & MFP~\cite{heFilterPruningSwitching2022} & 70.28 & 67.11 & -3.17 & 1814.00 & 874.35 & 51.80 & 11.69 & - & - \\
2.5.2 & 2022 & FTWT~\cite{elkerdawyFireTogetherWire2022} & 69.76 & 67.49 & -2.27 & 1814.00 & 878.70 & 51.56 & 11.69 & - & - \\
2.6.1 & 2022 & GNN-RL~\cite{yuTopologyAwareNetworkPruning2022} & 69.76 & 68.66 & -1.10 & 1814.00 & 888.86 & 51.00 & 11.69 & - & - \\
2.5.2 & 2021 & ManiDP~\cite{tangManifoldRegularizedDynamic2021} & 69.76 & 68.88 & -0.88 & 1814.00 & 888.86 & 51.00 & 11.69 & - & - \\
2.7.3 & 2020 & SWP~\cite{mengPruningFilterFilter2020} & 69.76 & 69.98 & 0.22 & 1814.00 & 898.29 & 50.48 & 11.69 & - & - \\
2.4.3 & 2022 & EKG~\cite{leeEnsembleKnowledgeGuided2022} & 70.38 & 69.39 & -0.99 & 1814.00 & 905.19 & 50.10 & 11.69 & - & - \\
2.5.2 & 2019 & FBS~\cite{gaoDynamicChannelPruning2019} & 70.71 & 68.17 & -2.54 & 1814.00 & 916.16 & 49.49 & 11.69 & - & - \\
2.5.2 & 2021 & DDG~\cite{liDynamicDualGating2021} & 69.76 & 70.12 & 0.36 & 1814.00 & 917.88 & 49.40 & 11.69 & - & - \\
2.5.2 & 2020 & DRLP~\cite{chenStorageEfficientDynamic2020} & 69.76 & 68.73 & -1.03 & 1814.00 & 935.05 & 48.45 & 11.69 & - & - \\
2.6.3 & 2020 & ABCPruner~\cite{linChannelPruningAutomatic2020} & 69.66 & 67.80 & -1.86 & 1814.00 & 962.55 & 46.94 & 11.69 & 9.50 & 18.73 \\
2.6.2 & 2021 & EE~\cite{zhangExplorationEstimationModel2021} & 70.28 & 68.27 & -2.01 & 1814.00 & 968.68 & 46.60 & 11.69 & - & - \\
2.3.2 & 2020 & SCOP~\cite{tangSCOPScientificControl2020} & 69.76 & 68.62 & -1.14 & 1814.00 & 997.70 & 45.00 & 11.69 & 6.60 & 43.50 \\
2.6.3 & 2020 & ABCPruner~\cite{linChannelPruningAutomatic2020} & 69.66 & 67.28 & -2.38 & 1814.00 & 999.91 & 44.88 & 11.69 & 6.60 & 43.54 \\
2.3.2 & 2021 & ABP~\cite{tianAddingPruningSparse2021} & 70.29 & 67.83 & -2.46 & 1814.00 & 1021.28 & 43.70 & 11.69 & 6.31 & 46.00 \\
2.6.2 & 2022 & DAIS~\cite{guanDAISAutomaticChannel2022} & 65.36 & 67.56 & 2.20 & 1814& 1028.54 & 43.30 & 11.69 & - & - \\
2.1.2 & 2019 & COP~\cite{wangCOPCustomizedDeep2019} & 70.29 & 66.98 & -3.31 & 1814.00 & 1028.54 & 43.30 & 11.69 & 6.42 & 45.10 \\
2.2.3 & 2020 & PFP~\cite{liebenweinProvableFilterPruning2020} & 69.74 & 65.65 & -4.09 & 1814.00 & 1031.80 & 43.12 & 11.69 & 4.62 & 60.48 \\
2.6.2 & 2022 & DNCP~\cite{zhengModelCompressionBased2022} & 70.10 & 69.20 & -0.90 & 1814.00 & 1048.09 & 42.22 & 11.69 & - & - \\
2.6.2 & 2020 & DMCP~\cite{guoDMCPDifferentiableMarkov2020} & 70.10 & 68.40 & -1.90 & 1814.00 & 1048.09 & 42.22 & 11.69 & - & - \\
2.6.2 & 2022 & MFP~\cite{heFilterPruningSwitching2022} & 70.28 & 67.66 & -2.62 & 1814.00 & 1055.75 & 41.80 & 11.69 & - & - \\
2.5.1 & 2018 & SFP~\cite{heSoftFilterPruning2018} & 70.28 & 67.10 & -3.18 & 1814.00 & 1055.75 & 41.80 & 11.69 & - & - \\
2.1.2 & 2019 & FPGM~\cite{heFilterPruningGeometric2019} & 70.28 & 68.41 & -1.87 & 1814.00 & 1055.75 & 41.80 & 11.69 & - & - \\
2.6.2 & 2022 & MFP~\cite{heFilterPruningSwitching2022} & 70.28 & 68.31 & -1.97 & 1814.00 & 1055.75 & 41.80 & 11.69 & - & - \\
2.6.2 & 2020 & DSA~\cite{ningDSAMoreEfficient2020} & 69.72 & 68.61 & -1.11 & 1814.00 & 1088.40 & 40.00 & 11.69 & - & - \\
2.3.2 & 2020 & SCOP~\cite{tangSCOPScientificControl2020} & 69.76 & 69.18 & -0.58 & 1814.00 & 1110.17 & 38.80 & 11.69 & 7.10 & 39.30 \\
2.6.2 & 2019 & TAS~\cite{dongNetworkPruningTransformable2019} & 67.65 & 69.15 & 1.50 & 1814.00 & 1209.94 & 33.30 & 11.69 & - & - \\
2.2.3 & 2020 & PFP~\cite{liebenweinProvableFilterPruning2020} & 69.74 & 67.38 & -2.36 & 1814.00 & 1282.50 & 29.30 & 11.69 & 6.57 & 43.80 \\
2.4.1 & 2022 & SOSP~\cite{nonnenmacherSOSPEfficientlyCapturing2022} & 69.76 & 68.78 & -0.98 & 1814.00 & 1287.94 & 29.00 & 11.69 & 6.43 & 45.00 \\
2.5.1 & 2021 & DCP-CAC~\cite{chenDynamicalChannelPruning2021} & 68.46 & 68.17 & -0.29 & 1814.00 & 1310.11 & 27.78 & 11.69 & 7.49 & 35.94 \\
2.7.1 & 2020 & EB~\cite{youDrawingEarlyBirdTickets2020} & 69.57 & 68.28 & -1.29 & 1814.00 & 1372.19 & 24.36 & 11.69 & 8.18 & 30.00 \\
2.4.1 & 2022 & SOSP~\cite{nonnenmacherSOSPEfficientlyCapturing2022} & 69.76 & 69.63 & -0.13 & 1814.00 & 1378.64 & 24.00 & 11.69 & 7.13 & 39.00 \\
2.7.2 & 2020 & DJPQ~\cite{wangDifferentiableJointPruning2020} & 69.74 & 69.27 & -0.47 & 1814.00 & 1393.07 & 23.20 & 11.69 & - & - \\
2.2.3 & 2020 & PFP~\cite{liebenweinProvableFilterPruning2020} & 69.74 & 68.66 & -1.08 & 1814.00 & 1451.38 & 19.99 & 11.69 & 8.06 & 31.03 \\
2.5.1 & 2021 & DCP-CAC~\cite{chenDynamicalChannelPruning2021} & 68.46 & 68.62 & 0.16 & 1814.00 & 1612.44 & 11.11 & 11.69 & 9.44 & 19.22 \\
2.7.1 & 2020 & EB~\cite{youDrawingEarlyBirdTickets2020} & 69.57 & 69.84 & 0.27 & 1814.00 & 1695.89 & 6.51 & 11.69 & 10.52 & 10.00 \\
2.5.1 & 2022 & CHEX~\cite{houCHEXCHannelEXploration2022} & - & 69.60 & - & 1814.00 & - & - & 11.69 & - & - \\
2.6.3 & 2022 & EDropout~\cite{salehinejadEDropoutEnergyBasedDropout2022} & 68.48 & 65.43 & -3.05 & 1814.00 & - & - & 11.69 & 5.39 & 53.91 \\
\bottomrule
\end{tabularx}

\captionof{table}{ResNet-18 on ImageNet-1K.}
\end{strip}

==> tables/imagenet/ResNet-34.tex <==
\begin{strip}
\centering
\scriptsize
\begin{tabularx}{\textwidth}{@{}>{\hsize=0.067\hsize}X>{\hsize=0.067\hsize}X>{\hsize=0.2\hsize}X>{\hsize=0.067\hsize}X>{\hsize=0.067\hsize}X>{\hsize=0.067\hsize}X>{\hsize=0.067\hsize}X>{\hsize=0.067\hsize}X>{\hsize=0.067\hsize}X>{\hsize=0.067\hsize}X>{\hsize=0.067\hsize}X>{\hsize=0.067\hsize}X>{\hsize=0.067\hsize}X@{}}
\toprule
\tabletitle \\
\midrule
\multicolumn{3}{l}{ResNet-34} \\
\midrule
2.5.2 & 2021 & DDG~\cite{liDynamicDualGating2021} & 73.31 & 71.95 & -1.36 & 3663 .00 & 1201.46 & 67.20 & 21.80 & - & - \\
2.5.2 & 2021 & DDG~\cite{liDynamicDualGating2021} & 73.31 & 73.01 & -0.30 & 3663 .00 & 1490.84 & 59.30 & 21.80 & - & - \\
2.6.3 & 2020 & ABCPruner~\cite{linChannelPruningAutomatic2020} & 73.28 & 70.45 & -2.83 & 3663 .00 & 1503.10 & 58.97 & 21.80 & 10.47 & 51.96 \\
2.7.3 & 2022 & SOKS~\cite{liuSOKSAutomaticSearching2022} & 74.01 & 73.52 & -0.49 & 3663 .00 & 1612.52 & 55.98 & 21.80 & 11.27 & 48.30 \\
2.5.2 & 2021 & ManiDP~\cite{tangManifoldRegularizedDynamic2021} & 73.31 & 72.74 & -0.57 & 3663 .00 & 1637.36 & 55.30 & 21.80 & - & - \\
2.5.2 & 2022 & FTWT~\cite{elkerdawyFireTogetherWire2022} & 73.30 & 71.71 & -1.59 & 3663 .00 & 1749.45 & 52.24 & 21.80 & - & - \\
2.3.2 & 2021 & ABP~\cite{tianAddingPruningSparse2021} & 73.86 & 72.15 & -1.71 & 3663 .00 & 1923.08 & 47.50 & 21.80 & 10.75 & 50.70 \\
2.5.2 & 2022 & FTWT~\cite{elkerdawyFireTogetherWire2022} & 73.30 & 72.17 & -1.13 & 3663 .00 & 1926.01 & 47.42 & 21.80 & - & - \\
2.5.2 & 2021 & ManiDP~\cite{tangManifoldRegularizedDynamic2021} & 73.31 & 73.30 & -0.01 & 3663 .00 & 1948.72 & 46.80 & 21.80 & - & - \\
2.5.1 & 2022 & CHEX~\cite{houCHEXCHannelEXploration2022} & - & 73.50 & - & 3663 .00 & 1990.76 & 45.65 & 21.80 & - & - \\
2.4.3 & 2022 & EKG~\cite{leeEnsembleKnowledgeGuided2022} & 73.85 & 73.51 & -0.34 & 3663 .00 & 2010.99 & 45.10 & 21.80 & - & - \\
2.3.2 & 2020 & SCOP~\cite{tangSCOPScientificControl2020} & 73.31 & 72.62 & -0.69 & 3663 .00 & 2021.98 & 44.80 & 21.80 & 11.86 & 45.60 \\
2.6.2 & 2022 & DDNP~\cite{gaoDisentangledDifferentiableNetwork2022} & 73.31 & 73.03 & -0.28 & 3663 .00 & 2043.95 & 44.20 & 21.80 & - & - \\
2.2.3 & 2018 & NISP~\cite{yuNISPPruningNetworks2018a} & - & - & 0.92 & 3663 .00 & 2060.07 & 43.76 & 21.80 & 12.28 & 43.68 \\
2.2.2 & 2020 & GFS~\cite{yeGoodSubnetworksProvably2020} & 73.40 & 71.90 & -1.50 & 3663 .00 & 2060.44 & 43.75 & 21.80 & 14.70 & 32.57 \\
2.3.2 & 2020 & DMC~\cite{gaoDiscreteModelCompression2020} & 73.30 & 72.57 & -0.73 & 3663 .00 & 2073.26 & 43.40 & 21.80 & - & - \\
2.6.3 & 2022 & CCEP~\cite{shangNeuralNetworkPruning2022} & 73.30 & 72.67 & -0.63 & 3663 .00 & 2120.88 & 42.10 & 21.80 & - & - \\
2.6.2 & 2022 & DAIS~\cite{guanDAISAutomaticChannel2022} & 72.23 & 72.77 & 0.54 & 3663 .00 & 2128.20 & 41.90 & 21.80 & - & - \\
2.5.1 & 2018 & SFP~\cite{heSoftFilterPruning2018} & 73.92 & 71.83 & -2.09 & 3663 .00 & 2157.51 & 41.10 & 21.80 & - & - \\
2.1.2 & 2019 & FPGM~\cite{heFilterPruningGeometric2019} & 73.92 & 72.63 & -1.29 & 3663 .00 & 2157.51 & 41.10 & 21.80 & - & - \\
2.6.3 & 2020 & ABCPruner~\cite{linChannelPruningAutomatic2020} & 73.28 & 70.98 & -2.30 & 3663 .00 & 2161.19 & 41.00 & 21.80 & 10.07 & 53.79 \\
2.3.2 & 2020 & SCOP~\cite{tangSCOPScientificControl2020} & 73.31 & 72.93 & -0.38 & 3663 .00 & 2230.77 & 39.10 & 21.80 & 13.15 & 39.70 \\
2.5.2 & 2022 & FTWT~\cite{elkerdawyFireTogetherWire2022} & 73.30 & 72.79 & -0.51 & 3663 .00 & 2279.48 & 37.77 & 21.80 & - & - \\
2.2.2 & 2020 & GFS~\cite{yeGoodSubnetworksProvably2020} & 73.40 & 73.50 & 0.10 & 3663 .00 & 2627.80 & 28.26 & 21.80 & 17.20 & 21.10 \\
2.2.3 & 2018 & NISP~\cite{yuNISPPruningNetworks2018a} & - & - & 0.28 & 3663 .00 & 2662.27 & 27.32 & 21.80 & 15.88 & 27.14 \\
2.5.2 & 2022 & FTWT~\cite{elkerdawyFireTogetherWire2022} & 73.30 & 73.25 & -0.05 & 3663 .00 & 2715.75 & 25.86 & 21.80 & - & - \\
2.6.3 & 2022 & CCEP~\cite{shangNeuralNetworkPruning2022} & 73.30 & 73.64 & 0.34 & 3663 .00 & 2731.13 & 25.44 & 21.80 & - & - \\
2.3.3 & 2021 & GREG~\cite{wangNeuralPruningGrowing2022} & 73.31 & 73.61 & 0.30 & 3663 .00 & 2775.00 & 24.24 & 21.80 & - & - \\
2.1.1 & 2017 & PFEC~\cite{liPruningFiltersEfficient2017} & 73.23 & 72.17 & -1.06 & 3663 .00 & 2776.55 & 24.20 & 21.80 & 19.45 & 10.80 \\
2.4.1 & 2019 & Mol-19~\cite{molchanovImportanceEstimationNeural2019} & 73.31 & 72.83 & -0.48 & 3663 .00 & 2847.88 & 22.25 & 21.80 & 17.20 & 21.10 \\
2.7.1 & 2022 & PaT~\cite{shenWhenPrunePolicy2022} & - & 73.50 & - & 3663 .00 & 2897.55 & 20.90 & 21.80 & - & - \\
2.1.1 & 2017 & PFEC~\cite{liPruningFiltersEfficient2017} & 73.23 & 72.56 & -0.67 & 3663 .00 & 3099.46 & 15.38 & 21.80 & 20.08 & 7.87 \\
2.6.3 & 2022 & EDropout~\cite{salehinejadEDropoutEnergyBasedDropout2022} & 73.42 & 71.82 & -1.60 & 3663 .00 & - & - & 21.80 & 9.59 & 56.02 \\
2.7.2 & 2020 & NM~\cite{kimNeuronMergingCompensating2020} & 73.31 & 66.77 & -6.54 & 3663 .00 & - & - & 21.80 & 19.72 & 9.52 \\
2.7.2 & 2020 & NM~\cite{kimNeuronMergingCompensating2020} & 73.31 & 55.70 & -17.61 & 3663 .00 & - & - & 21.80 & 17.65 & 19.05 \\
2.7.2 & 2020 & NM~\cite{kimNeuronMergingCompensating2020} & 73.31 & 37.43 & -35.88 & 3663 .00 & - & - & 21.80 & 15.57 & 28.57 \\
\bottomrule
\end{tabularx}

\captionof{table}{ResNet-34 on ImageNet-1K.}
\end{strip}

==> tables/imagenet/ResNet-50-P1.tex <==
\begin{strip}
\centering
\scriptsize
\begin{tabularx}{\textwidth}{@{}>{\hsize=0.067\hsize}X>{\hsize=0.067\hsize}X>{\hsize=0.2\hsize}X>{\hsize=0.067\hsize}X>{\hsize=0.067\hsize}X>{\hsize=0.067\hsize}X>{\hsize=0.067\hsize}X>{\hsize=0.067\hsize}X>{\hsize=0.067\hsize}X>{\hsize=0.067\hsize}X>{\hsize=0.067\hsize}X>{\hsize=0.067\hsize}X>{\hsize=0.067\hsize}X@{}}
\toprule
\tabletitle \\
\midrule
\multicolumn{3}{l}{ResNet-50} \\
\midrule
2.6.2 & 2020 & DMCP~\cite{guoDMCPDifferentiableMarkov2020} & 76.60 & 66.40 & -10.00 & 4089.00 & 277.25 & 93.22 & 25.56 & - & - \\
2.7.3 & 2021 & JMDP~\cite{liuJointMultiDimensionPruning2021} & 76.60 & 73.50 & -3.10 & 4089.00 & 897.59 & 78.05 & 25.56 & - & - \\
2.5.1 & 2022 & SMCP~\cite{humbleSoftMaskingCostConstrained2022} & 77.20 & 74.40 & -2.80 & 4089.00 & 897.59 & 78.05 & 25.56 & - & - \\
2.1.2 & 2022 & CLR-RNF~\cite{linPruningNetworksCrossLayer2022} & 76.01 & 71.11 & -4.90 & 4089.00 & 925.25 & 77.37 & 25.56 & 6.90 & 73.00 \\
2.2.1 & 2021 & CHIP~\cite{suiCHIPCHannelIndependencebased2021} & 76.15 & 73.30 & -2.85 & 4089.00 & 952.74 & 76.70 & 25.56 & 8.03 & 68.60 \\
2.2.1 & 2020 & HRank~\cite{linHRankFilterPruning2020} & 76.15 & 69.10 & -7.05 & 4089.00 & 979.76 & 76.04 & 25.56 & 8.29 & 67.57 \\
2.5.1 & 2022 & SMCP~\cite{humbleSoftMaskingCostConstrained2022} & 76.20 & 74.60 & -1.60 & 4089.00 & 997.32 & 75.61 & 25.56 & - & - \\
2.5.1 & 2022 & CHEX~\cite{houCHEXCHannelEXploration2022} & - & 76.00 & - & 4089.00 & 997.32 & 75.61 & 25.56 & - & - \\
2.3.1 & 2020 & EagleEye~\cite{liEagleEyeFastSubnet2020} & - & 74.20 & - & 4089.00 & 997.32 & 75.61 & 25.56 & - & - \\
2.6.3 & 2019 & MetaPruning~\cite{liuMetaPruningMetaLearning2019} & 76.60 & 73.40 & -3.20 & 4089.00 & 997.32 & 75.61 & 25.56 & - & - \\
2.6.2 & 2022 & PaS~\cite{liPruningasSearchEfficientNeural2022} & 74.68 & 74.80 & 0.12 & 4089.00 & 997.32 & 75.61 & 25.56 & - & - \\
2.4.1 & 2021 & GFP~\cite{liuGroupFisherPruning2021} & 76.79 & 73.94 & -2.85 & 4089.00 & 1020.00 & 75.06 & 25.56 & - & - \\
2.6.2 & 2022 & DNCP~\cite{zhengModelCompressionBased2022} & 76.60 & 74.30 & -2.30 & 4089.00 & 1097.05 & 73.17 & 25.56 & - & - \\
2.6.2 & 2020 & DMCP~\cite{guoDMCPDifferentiableMarkov2020} & 76.60 & 74.40 & -2.20 & 4089.00 & 1097.05 & 73.17 & 25.56 & - & - \\
2.3.2 & 2019 & GAL~\cite{linOptimalStructuredCNN2019} & 76.15 & 69.31 & -6.84 & 4089.00 & 1109.73 & 72.86 & 25.56 & 10.22 & 60.00 \\
2.2.2 & 2017 & ThiNet~\cite{luoThiNetFilterLevel2017} & 72.88 & 68.42 & -4.46 & 4089.00 & 1165.26 & 71.50 & 25.56 & 8.68 & 66.04 \\
2.6.1 & 2022 & DECORE~\cite{alwaniDECOREDeepCompression2022} & 76.15 & 69.71 & -6.44 & 4089.00 & 1189.71 & 70.90 & 25.56 & 6.13 & 76.00 \\
2.1.2 & 2022 & CLR-RNF~\cite{linPruningNetworksCrossLayer2022} & 76.01 & 73.34 & -2.67 & 4089.00 & 1223.72 & 70.07 & 25.56 & 9.00 & 64.79 \\
2.1.2 & 2022 & CLR-RNF~\cite{linPruningNetworksCrossLayer2022} & 76.01 & 72.67 & -3.34 & 4089.00 & 1223.72 & 70.07 & 25.56 & 9.00 & 64.79 \\
2.7.1 & 2020 & EB~\cite{youDrawingEarlyBirdTickets2020} & 75.99 & 70.16 & -5.83 & 4089.00 & 1282.37 & 68.64 & 25.56 & 7.67 & 70.00 \\
2.5.2 & 2021 & DDG~\cite{liDynamicDualGating2021} & 76.13 & 75.12 & -1.01 & 4089.00 & 1312.57 & 67.90 & 25.56 & - & - \\
2.3.3 & 2021 & GREG~\cite{wangNeuralPruningGrowing2022} & 76.13 & 73.90 & -2.23 & 4089.00 & 1336.27 & 67.32 & 25.56 & - & - \\
2.4.1 & 2019 & Mol-19~\cite{molchanovImportanceEstimationNeural2019} & 76.18 & 71.69 & -4.49 & 4089.00 & 1339.67 & 67.24 & 25.56 & 7.89 & 69.14 \\
2.4.1 & 2022 & HAP~\cite{yuHessianAwarePruningOptimal2022} & 75.62 & 71.18 & -4.44 & 4089.00 & 1343.24 & 67.15 & 25.56 & 5.23 & 79.53 \\
2.3.3 & 2021 & OTO~\cite{chenOnlyTrainOnce2021} & 76.10 & 75.10 & -1.00 & 4089.00 & 1410.71 & 65.50 & 25.56 & 9.07 & 64.50 \\
2.3.3 & 2021 & OTO~\cite{chenOnlyTrainOnce2021} & 76.10 & 74.70 & -1.40 & 4089.00 & 1410.71 & 65.50 & 25.56 & 9.07 & 64.50 \\
2.6.3 & 2022 & CCEP~\cite{shangNeuralNetworkPruning2022} & 76.13 & 74.87 & -1.26 & 4089.00 & 1468.36 & 64.09 & 25.56 & - & - \\
2.3.2 & 2022 & WhiteBox~\cite{zhangCarryingOutCNN2022} & 76.15 & 74.21 & -1.94 & 4089.00 & 1492.49 & 63.50 & 25.56 & - & - \\
2.2.1 & 2021 & CHIP~\cite{suiCHIPCHannelIndependencebased2021} & 76.15 & 75.26 & -0.89 & 4089.00 & 1521.11 & 62.80 & 25.56 & 11.07 & 56.70 \\
2.7.2 & 2021 & CC~\cite{liCompactCNNsCollaborative2021} & 76.15 & 74.54 & -1.61 & 4089.00 & 1525.90 & 62.68 & 25.56 & 10.58 & 58.61 \\
2.2.1 & 2020 & HRank~\cite{linHRankFilterPruning2020} & 76.15 & 71.98 & -4.17 & 4089.00 & 1549.62 & 62.10 & 25.56 & 13.80 & 46.00 \\
2.3.2 & 2021 & ResRep~\cite{dingResRepLosslessCNN2021} & 76.15 & 75.30 & -0.85 & 4089.00 & 1549.73 & 62.10 & 25.56 & - & - \\
2.3.2 & 2019 & GAL~\cite{linOptimalStructuredCNN2019} & 76.15 & 69.88 & -6.27 & 4089.00 & 1579.61 & 61.37 & 25.56 & 14.70 & 42.47 \\
2.3.3 & 2021 & GREG~\cite{wangNeuralPruningGrowing2022} & 76.13 & 74.93 & -1.20 & 4089.00 & 1597.27 & 60.94 & 25.56 & - & - \\
2.6.1 & 2022 & DECORE~\cite{alwaniDECOREDeepCompression2022} & 76.15 & 72.06 & -4.09 & 4089.00 & 1599.61 & 60.88 & 25.56 & 8.89 & 65.22 \\
2.6.2 & 2020 & LFPC~\cite{heLearningFilterPruning2020} & 76.15 & 74.46 & -1.69 & 4089.00 & 1602.89 & 60.80 & 25.56 & - & - \\
2.6.2 & 2020 & LFPC~\cite{heLearningFilterPruning2020} & 76.15 & 74.18 & -1.97 & 4089.00 & 1602.89 & 60.80 & 25.56 & - & - \\
2.5.2 & 2021 & DDG~\cite{liDynamicDualGating2021} & 76.13 & 76.41 & 0.28 & 4089.00 & 1647.87 & 59.70 & 25.56 & - & - \\
2.4.1 & 2022 & HAP~\cite{yuHessianAwarePruningOptimal2022} & 75.62 & 74.00 & -1.62 & 4089.00 & 1653.59 & 59.56 & 25.56 & 8.88 & 65.26 \\
2.5.1 & 2018 & GDP-Lin~\cite{linAcceleratingConvolutionalNetworks2018} & 75.13 & 70.93 & -4.20 & 4089.00 & 1663.14 & 59.33 & 25.56 & - & - \\
2.4.1 & 2022 & SOSP~\cite{nonnenmacherSOSPEfficientlyCapturing2022} & 76.15 & 73.38 & -2.77 & 4089.00 & 1676.49 & 59.00 & 25.56 & 9.97 & 61.00 \\
2.7.1 & 2022 & PaT~\cite{shenWhenPrunePolicy2022} & - & 74.85 & - & 4089.00 & 1690.45 & 58.66 & 25.56 & - & - \\
2.2.2 & 2019 & AOFP~\cite{dingApproximatedOracleFilter2019} & 75.34 & 75.11 & -0.23 & 4089.00 & 1763.05 & 56.88 & 25.56 & - & - \\
2.3.3 & 2021 & GREG~\cite{wangNeuralPruningGrowing2022} & 75.40 & 75.22 & -0.18 & 4089.00 & 1770.13 & 56.71 & 25.56 & - & - \\
2.6.3 & 2020 & ABCPruner~\cite{linChannelPruningAutomatic2020} & 76.01 & 73.52 & -2.49 & 4089.00 & 1774.19 & 56.61 & 25.56 & 11.24 & 56.03 \\
2.6.3 & 2022 & CCEP~\cite{shangNeuralNetworkPruning2022} & 76.13 & 75.55 & -0.58 & 4089.00 & 1784.85 & 56.35 & 25.56 & - & - \\
2.3.2 & 2021 & ResRep~\cite{dingResRepLosslessCNN2021} & 76.15 & 75.97 & -0.18 & 4089.00 & 1794.66 & 56.11 & 25.56 & - & - \\
2.6.2 & 2021 & EE~\cite{zhangExplorationEstimationModel2021} & 76.15 & 75.66 & -0.49 & 4089.00 & 1799.16 & 56.00 & 25.56 & - & - \\
2.2.2 & 2017 & ThiNet~\cite{luoThiNetFilterLevel2017} & 72.88 & 71.01 & -1.87 & 4089.00 & 1806.15 & 55.83 & 25.56 & 12.41 & 51.45 \\
2.4.3 & 2019 & C-SGD~\cite{dingCentripetalSGDPruning2019} & 75.33 & 74.54 & -0.79 & 4089.00 & 1808.97 & 55.76 & 25.56 & - & - \\
2.5.1 & 2021 & DCP-CAC~\cite{chenDynamicalChannelPruning2021} & - & - & -0.79 & 4089.00 & 1817.33 & 55.56 & 25.56 & 12.35 & 51.69 \\
2.2.3 & 2018 & DCP~\cite{zhuangDiscriminationawareChannelPruning2018} & - & - & 1.06 & 4089.00 & 1817.33 & 55.56 & 25.56 & 12.41 & 51.46 \\
2.6.2 & 2022 & DAIS~\cite{guanDAISAutomaticChannel2022} & 72.75 & 74.45 & 1.70 & 4089.00 & 1827.78 & 55.30 & 25.56 & - & - \\
2.1.2 & 2021 & SRR~\cite{wangConvolutionalNeuralNetwork2021} & 76.13 & 75.11 & -1.02 & 4089.00 & 1835.96 & 55.10 & 25.56 & - & - \\
2.3.1 & 2019 & GBN~\cite{youGateDecoratorGlobal2019} & 74.51 & 75.18 & 0.67 & 4089.00 & 1837.60 & 55.06 & 25.56 & 11.91 & 53.40 \\
2.3.2 & 2019 & GAL~\cite{linOptimalStructuredCNN2019} & 76.15 & 71.80 & -4.35 & 4089.00 & 1839.55 & 55.01 & 25.56 & 19.36 & 24.27 \\
2.3.2 & 2020 & DMC~\cite{gaoDiscreteModelCompression2020} & 76.15 & 75.35 & -0.80 & 4089.00 & 1840.05 & 55.00 & 25.56 & - & - \\
2.4.3 & 2022 & EKG~\cite{leeEnsembleKnowledgeGuided2022} & 77.00 & 76.60 & -0.40 & 4089.00 & 1840.05 & 55.00 & 25.56 & - & - \\
2.6.1 & 2022 & RL-MCTS~\cite{wangChannelPruningLookahead2022} & 77.34 & 76.46 & -0.88 & 4089.00 & 1840.05 & 55.00 & 25.56 & - & - \\
2.6.2 & 2022 & DDNP~\cite{gaoDisentangledDifferentiableNetwork2022} & 76.13 & 75.89 & -0.24 & 4089.00 & 1840.05 & 55.00 & 25.56 & - & - \\
2.3.2 & 2020 & SCOP~\cite{tangSCOPScientificControl2020} & 76.15 & 75.26 & -0.89 & 4089.00 & 1856.41 & 54.60 & 25.56 & 12.32 & 51.80 \\
2.4.2 & 2019 & RBP~\cite{zhouAccelerateCNNRecursive2019} & - & 73.00 & - & 4089.00 & 1858.64 & 54.55 & 25.56 & - & - \\
2.3.2 & 2021 & ResRep~\cite{dingResRepLosslessCNN2021} & 76.15 & 76.15 & 0.00 & 4089.00 & 1858.86 & 54.54 & 25.56 & - & - \\
2.3.1 & 2020 & SCP~\cite{kangOperationAwareSoftChannel2020} & 75.89 & 74.20 & 1.69 & 4089.00 & 1868.67 & 54.30 & 25.56 & - & - \\
2.3.1 & 2020 & SCP~\cite{kangOperationAwareSoftChannel2020} & 75.89 & 75.27 & 0.62 & 4089.00 & 1868.67 & 54.30 & 25.56 & - & - \\
2.6.3 & 2020 & ABCPruner~\cite{linChannelPruningAutomatic2020} & 76.01 & 73.86 & -2.15 & 4089.00 & 1869.25 & 54.29 & 25.56 & 11.75 & 54.03 \\
2.4.1 & 2019 & CCP~\cite{pengCollaborativeChannelPruning2019} & 76.15 & 76.98 & 0.83 & 4089.00 & 1876.85 & 54.10 & 25.56 & - & - \\
2.3.1 & 2020 & PR~\cite{zhuangNeuronlevelStructuredPruning2020} & 76.15 & 75.63 & 0.52 & 4089.00 & 1880.94 & 54.00 & 25.56 & - & - \\
2.2.3 & 2022 & DLRFC~\cite{heFilterPruningFeature2022} & 76.13 & 75.84 & 0.29 & 4089.00 & 1880.94 & 54.00 & 25.56 & 15.34 & 40.00 \\
2.7.3 & 2021 & JMDP~\cite{liuJointMultiDimensionPruning2021} & 76.60 & 76.00 & -0.60 & 4089.00 & 1894.90 & 53.66 & 25.56 & - & - \\
2.5.1 & 2022 & SMCP~\cite{humbleSoftMaskingCostConstrained2022} & 77.20 & 76.60 & -0.60 & 4089.00 & 1894.90 & 53.66 & 25.56 & - & - \\
\midrule
\multicolumn{12}{l}{Continue on the next page...}\\
\bottomrule
\end{tabularx}

\captionof{table}{ResNet-50 on ImageNet-1K. (Part 1)}
\end{strip}

\addtocounter{table}{-1}

==> tables/imagenet/ResNet-50-P2.tex <==
\begin{strip}
\centering
\scriptsize
\begin{tabularx}{\textwidth}{@{}>{\hsize=0.067\hsize}X>{\hsize=0.067\hsize}X>{\hsize=0.2\hsize}X>{\hsize=0.067\hsize}X>{\hsize=0.067\hsize}X>{\hsize=0.067\hsize}X>{\hsize=0.067\hsize}X>{\hsize=0.067\hsize}X>{\hsize=0.067\hsize}X>{\hsize=0.067\hsize}X>{\hsize=0.067\hsize}X>{\hsize=0.067\hsize}X>{\hsize=0.067\hsize}X@{}}
\toprule
\tabletitle \\
\midrule
\multicolumn{3}{l}{ResNet-50 (cont.)} \\
\midrule
2.6.2 & 2022 & MFP~\cite{heFilterPruningSwitching2022} & 76.15 & 74.13 & -2.02 & 4089.00 & 1901.38 & 53.50 & 25.56 & - & - \\
2.6.2 & 2022 & MFP~\cite{heFilterPruningSwitching2022} & 76.15 & 74.86 & -1.29 & 4089.00 & 1901.38 & 53.50 & 25.56 & - & - \\
2.1.2 & 2019 & FPGM~\cite{heFilterPruningGeometric2019} & 76.15 & 75.59 & -0.56 & 4089.00 & 1901.38 & 53.50 & 25.56 & - & - \\
2.7.2 & 2020 & Hinge~\cite{liGroupSparsityHinge2020} & - & 74.70 & - & 4089.00 & 1903.43 & 53.45 & 25.56 & - & - \\
2.6.1 & 2022 & GNN-RL~\cite{yuTopologyAwareNetworkPruning2022} & 76.10 & 74.28 & -1.82 & 4089.00 & 1921.83 & 53.00 & 25.56 & - & - \\
2.7.2 & 2021 & CC~\cite{liCompactCNNsCollaborative2021} & 76.15 & 75.59 & -0.56 & 4089.00 & 1924.82 & 52.93 & 25.56 & 13.20 & 48.36 \\
2.2.1 & 2021 & LRMF~\cite{zhangFilterPruningLearned2021} & 76.15 & 74.70 & -1.45 & 4089.00 & 1934.10 & 52.70 & 25.56 & - & - \\
2.5.1 & 2018 & GDP-Lin~\cite{linAcceleratingConvolutionalNetworks2018} & 75.13 & 71.89 & -3.24 & 4089.00 & 1991.53 & 51.30 & 25.56 & - & - \\
2.5.1 & 2022 & SMCP~\cite{humbleSoftMaskingCostConstrained2022} & 76.20 & 76.80 & 0.60 & 4089.00 & 1994.63 & 51.22 & 25.56 & - & - \\
2.5.1 & 2022 & CHEX~\cite{houCHEXCHannelEXploration2022} & - & 77.40 & - & 4089.00 & 1994.63 & 51.22 & 25.56 & - & - \\
2.3.1 & 2020 & EagleEye~\cite{liEagleEyeFastSubnet2020} & - & 76.40 & - & 4089.00 & 1994.63 & 51.22 & 25.56 & - & - \\
2.6.3 & 2019 & MetaPruning~\cite{liuMetaPruningMetaLearning2019} & 76.60 & 75.40 & -1.20 & 4089.00 & 1994.63 & 51.22 & 25.56 & - & - \\
2.6.2 & 2022 & PaS~\cite{liPruningasSearchEfficientNeural2022} & 76.65 & 76.70 & 0.05 & 4089.00 & 1994.63 & 51.22 & 25.56 & - & - \\
2.7.1 & 2022 & RRCP~\cite{liRevisitingRandomChannel2022} & - & 75.13 & - & 4089.00 & 2003.20 & 51.01 & 25.56 & 13.83 & 45.88 \\
2.4.1 & 2022 & SOSP~\cite{nonnenmacherSOSPEfficientlyCapturing2022} & 76.15 & 74.39 & -1.76 & 4089.00 & 2003.61 & 51.00 & 25.56 & 11.76 & 54.00 \\
2.4.1 & 2021 & GFP~\cite{liuGroupFisherPruning2021} & 76.79 & 76.42 & -0.37 & 4089.00 & 2040.00 & 50.11 & 25.56 & - & - \\
2.6.2 & 2020 & DSA~\cite{ningDSAMoreEfficient2020} & 76.02 & 74.69 & -1.33 & 4089.00 & 2044.50 & 50.00 & 25.56 & - & - \\
2.3.3 & 2019 & OICSR~\cite{liOICSROutInChannelSparsity2019} & 76.31 & 75.95 & -0.36 & 4089.00 & 2044.50 & 50.00 & 25.56 & - & - \\
2.4.1 & 2019 & CCP~\cite{pengCollaborativeChannelPruning2019} & 76.15 & 76.80 & 0.65 & 4089.00 & 2093.57 & 48.80 & 25.56 & - & - \\
2.2.1 & 2021 & CHIP~\cite{suiCHIPCHannelIndependencebased2021} & 76.15 & 76.15 & 0.00 & 4089.00 & 2097.66 & 48.70 & 25.56 & 14.26 & 44.20 \\
2.6.2 & 2022 & DNCP~\cite{zhengModelCompressionBased2022} & 76.60 & 76.30 & -0.30 & 4089.00 & 2194.10 & 46.34 & 25.56 & - & - \\
2.6.2 & 2020 & DMCP~\cite{guoDMCPDifferentiableMarkov2020} & 76.60 & 76.20 & -0.40 & 4089.00 & 2194.10 & 46.34 & 25.56 & - & - \\
2.4.3 & 2019 & C-SGD~\cite{dingCentripetalSGDPruning2019} & 75.33 & 74.93 & -0.40 & 4089.00 & 2198.25 & 46.24 & 25.56 & - & - \\
2.6.2 & 2021 & EE~\cite{zhangExplorationEstimationModel2021} & 76.15 & 76.05 & -0.10 & 4089.00 & 2203.97 & 46.10 & 25.56 & - & - \\
2.6.1 & 2022 & RL-MCTS~\cite{wangChannelPruningLookahead2022} & 77.34 & 76.80 & -0.54 & 4089.00 & 2203.97 & 46.10 & 25.56 & - & - \\
2.3.2 & 2022 & WhiteBox~\cite{zhangCarryingOutCNN2022} & 76.15 & 75.32 & -0.83 & 4089.00 & 2224.42 & 45.60 & 25.56 & - & - \\
2.3.2 & 2020 & SCOP~\cite{tangSCOPScientificControl2020} & 76.15 & 75.95 & -0.20 & 4089.00 & 2236.68 & 45.30 & 25.56 & 14.62 & 42.80 \\
2.4.1 & 2022 & SOSP~\cite{nonnenmacherSOSPEfficientlyCapturing2022} & 76.15 & 75.21 & -0.94 & 4089.00 & 2248.95 & 45.00 & 25.56 & 13.04 & 49.00 \\
2.4.1 & 2019 & Mol-19~\cite{molchanovImportanceEstimationNeural2019} & 76.18 & 74.50 & -1.68 & 4089.00 & 2249.45 & 44.99 & 25.56 & 14.18 & 44.53 \\
2.2.1 & 2021 & CHIP~\cite{suiCHIPCHannelIndependencebased2021} & 76.15 & 76.30 & 0.15 & 4089.00 & 2257.13 & 44.80 & 25.56 & 15.13 & 40.80 \\
2.6.3 & 2022 & CCEP~\cite{shangNeuralNetworkPruning2022} & 76.13 & 76.06 & -0.07 & 4089.00 & 2266.94 & 44.56 & 25.56 & - & - \\
2.4.1 & 2022 & HAP~\cite{yuHessianAwarePruningOptimal2022} & 75.62 & 75.36 & -0.26 & 4089.00 & 2268.99 & 44.51 & 25.56 & 13.74 & 46.26 \\
2.3.3 & 2019 & OICSR~\cite{liOICSROutInChannelSparsity2019} & 76.31 & 76.30 & -0.01 & 4089.00 & 2273.48 & 44.40 & 25.56 & - & - \\
2.1.2 & 2021 & SRR~\cite{wangConvolutionalNeuralNetwork2021} & 76.13 & 75.76 & -0.37 & 4089.00 & 2285.75 & 44.10 & 25.56 & - & - \\
2.2.3 & 2018 & NISP~\cite{yuNISPPruningNetworks2018a} & - & - & 0.89 & 4089.00 & 2289.43 & 44.01 & 25.56 & 14.36 & 43.82 \\
2.2.1 & 2020 & HRank~\cite{linHRankFilterPruning2020} & 76.15 & 74.98 & -1.17 & 4089.00 & 2299.44 & 43.77 & 25.56 & 16.19 & 36.67 \\
2.6.2 & 2019 & TAS~\cite{dongNetworkPruningTransformable2019} & 74.94 & 76.20 & 1.26 & 4089.00 & 2310.28 & 43.50 & 25.56 & - & - \\
2.3.2 & 2019 & GAL~\cite{linOptimalStructuredCNN2019} & 76.15 & 71.95 & -4.20 & 4089.00 & 2329.43 & 43.03 & 25.56 & 21.25 & 16.86 \\
2.5.1 & 2021 & SEP~\cite{dingWherePruneUsing2021} & 76.12 & 75.22 & -0.90 & 4089.00 & 2330.73 & 43.00 & 25.56 & - & - \\
2.3.2 & 2021 & ABP~\cite{tianAddingPruningSparse2021} & 75.88 & 74.80 & -1.08 & 4089.00 & 2338.91 & 42.80 & 25.56 & 13.04 & 49.00 \\
2.6.1 & 2022 & DECORE~\cite{alwaniDECOREDeepCompression2022} & 76.15 & 74.58 & -1.57 & 4089.00 & 2359.42 & 42.30 & 25.56 & 14.13 & 44.71 \\
2.6.2 & 2022 & MFP~\cite{heFilterPruningSwitching2022} & 76.15 & 75.67 & -0.48 & 4089.00 & 2363.44 & 42.20 & 25.56 & - & - \\
2.5.1 & 2018 & GDP-Lin~\cite{linAcceleratingConvolutionalNetworks2018} & 75.13 & 72.61 & -2.52 & 4089.00 & 2372.89 & 41.97 & 25.56 & - & - \\
2.5.1 & 2018 & SFP~\cite{heSoftFilterPruning2018} & 76.15 & 62.14 & -14.01 & 4089.00 & 2379.80 & 41.80 & 25.56 & - & - \\
2.5.1 & 2018 & SFP~\cite{heSoftFilterPruning2018} & 76.15 & 74.61 & -1.54 & 4089.00 & 2379.80 & 41.80 & 25.56 & - & - \\
2.3.1 & 2019 & GBN~\cite{youGateDecoratorGlobal2019} & 76.50 & 76.19 & -0.31 & 4089.00 & 2431.32 & 40.54 & 25.56 & 17.42 & 31.83 \\
2.1.2 & 2022 & CLR-RNF~\cite{linPruningNetworksCrossLayer2022} & 76.01 & 74.85 & -1.16 & 4089.00 & 2437.48 & 40.39 & 25.56 & 16.92 & 33.80 \\
2.6.2 & 2020 & DSA~\cite{ningDSAMoreEfficient2020} & 76.02 & 75.10 & -0.92 & 4089.00 & 2453.40 & 40.00 & 25.56 & - & - \\
2.7.1 & 2020 & EB~\cite{youDrawingEarlyBirdTickets2020} & 75.99 & 73.35 & -2.64 & 4089.00 & 2474.71 & 39.48 & 25.56 & 12.78 & 50.00 \\
2.3.3 & 2019 & OICSR~\cite{liOICSROutInChannelSparsity2019} & 76.31 & 76.53 & 0.22 & 4089.00 & 2563.80 & 37.30 & 25.56 & - & - \\
2.2.2 & 2017 & ThiNet~\cite{luoThiNetFilterLevel2017} & 72.88 & 72.04 & -0.84 & 4089.00 & 2584.76 & 36.79 & 25.56 & 16.98 & 33.57 \\
2.4.3 & 2019 & C-SGD~\cite{dingCentripetalSGDPruning2019} & 75.33 & 75.27 & -0.06 & 4089.00 & 2586.29 & 36.75 & 25.56 & - & - \\
2.4.1 & 2019 & Mol-19~\cite{molchanovImportanceEstimationNeural2019} & 76.18 & 75.48 & -0.70 & 4089.00 & 2659.35 & 34.96 & 25.56 & 17.87 & 30.08 \\
2.7.3 & 2022 & GKP-TMI~\cite{zhongRevisitKernelPruning2022} & 76.15 & 75.53 & -0.62 & 4089.00 & 2709.37 & 33.74 & 25.56 & 17.07 & 33.21 \\
2.2.2 & 2019 & AOFP~\cite{dingApproximatedOracleFilter2019} & 75.34 & 75.63 & 0.29 & 4089.00 & 2740.16 & 32.99 & 25.56 & - & - \\
2.3.3 & 2021 & GREG~\cite{wangNeuralPruningGrowing2022} & 76.13 & 76.13 & 0.00 & 4089.00 & 2744.30 & 32.89 & 25.56 & - & - \\
2.7.3 & 2021 & JMDP~\cite{liuJointMultiDimensionPruning2021} & 76.60 & 76.50 & -0.10 & 4089.00 & 2792.49 & 31.71 & 25.56 & - & - \\
2.6.2 & 2020 & DMCP~\cite{guoDMCPDifferentiableMarkov2020} & 76.60 & 77.00 & 0.40 & 4089.00 & 2792.49 & 31.71 & 25.56 & - & - \\
2.2.3 & 2020 & PFP~\cite{liebenweinProvableFilterPruning2020} & 76.13 & 75.21 & -0.92 & 4089.00 & 2860.26 & 30.05 & 25.56 & 14.30 & 44.04 \\
2.4.1 & 2022 & SOSP~\cite{nonnenmacherSOSPEfficientlyCapturing2022} & 76.15 & 76.60 & 0.45 & 4089.00 & 2944.08 & 28.00 & 25.56 & 17.89 & 30.00 \\
2.2.3 & 2018 & NISP~\cite{yuNISPPruningNetworks2018a} & - & - & 0.21 & 4089.00 & 2972.29 & 27.31 & 25.56 & 18.63 & 27.12 \\
2.4.1 & 2022 & SOSP~\cite{nonnenmacherSOSPEfficientlyCapturing2022} & 76.15 & 75.85 & -0.30 & 4089.00 & 2984.97 & 27.00 & 25.56 & 15.34 & 40.00 \\
2.6.3 & 2019 & MetaPruning~\cite{liuMetaPruningMetaLearning2019} & 76.60 & 76.20 & -0.40 & 4089.00 & 2991.95 & 26.83 & 25.56 & - & - \\
2.6.2 & 2022 & PaS~\cite{liPruningasSearchEfficientNeural2022} & 77.53 & 77.60 & 0.07 & 4089.00 & 2991.95 & 26.83 & 25.56 & - & - \\
2.5.1 & 2022 & SMCP~\cite{humbleSoftMaskingCostConstrained2022} & 76.20 & 77.10 & 0.90 & 4089.00 & 2991.95 & 26.83 & 25.56 & - & - \\
2.3.1 & 2020 & EagleEye~\cite{liEagleEyeFastSubnet2020} & - & 77.10 & - & 4089.00 & 2991.95 & 26.83 & 25.56 & - & - \\
2.4.1 & 2021 & GFP~\cite{liuGroupFisherPruning2021} & 76.79 & 76.95 & 0.16 & 4089.00 & 3060.00 & 25.17 & 25.56 & - & - \\
2.5.1 & 2022 & SMCP~\cite{humbleSoftMaskingCostConstrained2022} & 77.20 & 77.60 & 0.40 & 4089.00 & 3091.68 & 24.39 & 25.56 & - & - \\
2.7.3 & 2022 & GKP-TMI~\cite{zhongRevisitKernelPruning2022} & 76.15 & 75.96 & -0.19 & 4089.00 & 3168.98 & 22.50 & 25.56 & 19.91 & 22.10 \\
2.7.1 & 2020 & EB~\cite{youDrawingEarlyBirdTickets2020} & 75.99 & 73.86 & -2.13 & 4089.00 & 3228.48 & 21.04 & 25.56 & 17.89 & 30.00 \\
2.4.1 & 2022 & SOSP~\cite{nonnenmacherSOSPEfficientlyCapturing2022} & 76.15 & 76.56 & 0.41 & 4089.00 & 3230.31 & 21.00 & 25.56 & 19.94 & 22.00 \\
2.4.1 & 2019 & Mol-19~\cite{molchanovImportanceEstimationNeural2019} & 76.18 & 76.43 & 0.25 & 4089.00 & 3269.20 & 20.05 & 25.56 & 22.56 & 11.72 \\
2.6.1 & 2022 & DECORE~\cite{alwaniDECOREDeepCompression2022} & 76.15 & 76.31 & 0.16 & 4089.00 & 3539.13 & 13.45 & 25.56 & 22.74 & 11.02 \\
2.2.3 & 2020 & PFP~\cite{liebenweinProvableFilterPruning2020} & 76.13 & 75.91 & -0.22 & 4089.00 & 3646.57 & 10.82 & 25.56 & 20.96 & 18.01 \\
2.6.3 & 2022 & EDropout~\cite{salehinejadEDropoutEnergyBasedDropout2022} & 75.27 & 73.72 & -1.55 & 4089.00 & - & - & 25.56 & 10.86 & 57.50 \\
2.7.3 & 2022 & 1xN~\cite{lin1xNPatternPruning2022} & 77.01 & 76.65 & -0.35 & 4089.00 & - & - & 25.56 & 12.78 & 50.00 \\
\bottomrule
\end{tabularx}

\captionof{table}{ResNet-50 on ImageNet-1K. (Part 2)}
\end{strip}

==> tables/imagenet/VGG.tex <==
\begin{strip}
\centering
\scriptsize
\begin{tabularx}{\textwidth}{@{}>{\hsize=0.067\hsize}X>{\hsize=0.067\hsize}X>{\hsize=0.2\hsize}X>{\hsize=0.067\hsize}X>{\hsize=0.067\hsize}X>{\hsize=0.067\hsize}X>{\hsize=0.1\hsize}X>{\hsize=0.067\hsize}X>{\hsize=0.067\hsize}X>{\hsize=0.067\hsize}X>{\hsize=0.067\hsize}X>{\hsize=0.067\hsize}X>{\hsize=0.067\hsize}X@{}}
\toprule
\tabletitle \\
\midrule
\multicolumn{3}{l}{VGG-11} \\
\midrule
2.1.2 & 2019 & COP~\cite{wangCOPCustomizedDeep2019} & 63.60 & 62.38 & -1.22 & 7630.00 & 4211.76 & 44.80 & 132.86 & 22.32 & 83.20 \\
2.6.2 & 2021 & EE~\cite{zhangExplorationEstimationModel2021} & 70.84 & 71.15 & 0.31 & 7630.00 & 5035.80 & 34.00 & 132.86 & - & - \\
2.4.1 & 2019 & Mol-19~\cite{molchanovImportanceEstimationNeural2019} & 70.84 & 70.65 & -0.19 & 7630.00 & 6948.21 & 8.94 & 132.86 & 31.79 & 76.07 \\
\midrule
\multicolumn{3}{l}{VGG-16} \\
\midrule
2.6.1 & 2022 & GNN-RL~\cite{yuTopologyAwareNetworkPruning2022} & 70.50 & 70.99 & 0.49 & 15500 .00 & 3100.00 & 80.00 & 138.40 & - & - \\
2.4.2 & 2019 & RBP~\cite{zhouAccelerateCNNRecursive2019} & - & 69.20 & - & 15500 .00 & 3100.00 & 80.00 & 138.40 & - & - \\
2.6.1 & 2018 & AMC~\cite{heAMCAutoMLModel2018} & 70.50 & 69.10 & -1.40 & 15500 .00 & 3100.00 & 80.00 & 138.40 & - & - \\
2.6.1 & 2021 & AGMC~\cite{yuAutoGraphEncoderDecoder2021} & 70.50 & 70.35 & -0.15 & 15500 .00 & 3100.00 & 80.00 & 138.40 & - & - \\
2.5.1 & 2018 & GDP-Lin~\cite{linAcceleratingConvolutionalNetworks2018} & 70.32 & 67.51 & -2.81 & 15500 .00 & 3800.00 & 75.48 & 138.40 & - & - \\
2.6.2 & 2022 & DAIS~\cite{guanDAISAutomaticChannel2022} & - & - & 2.91 & 15500 .00 & 3875.00 & 75.00 & 138.40 & - & - \\
2.2.2 & 2017 & ThiNet~\cite{luoThiNetFilterLevel2017} & 68.34 & 67.34 & -1.00 & 15500 .00 & 4679.06 & 69.81 & 138.40 & 8.32 & 93.99 \\
2.2.2 & 2017 & ThiNet~\cite{luoThiNetFilterLevel2017} & 68.34 & 69.80 & 1.46 & 15500 .00 & 4799.29 & 69.04 & 138.40 & 131.50 & 4.99 \\
2.5.1 & 2019 & DSG~\cite{liuDynamicSparseGraph2019} & - & 71.44 & - & 15500 .00 & 5747.40 & 62.92 & 138.40 & - & - \\
2.5.1 & 2018 & GDP-Lin~\cite{linAcceleratingConvolutionalNetworks2018} & 70.32 & 68.80 & -1.52 & 15500 .00 & 6400.00 & 58.71 & 138.40 & - & - \\
2.7.2 & 2021 & CC~\cite{liCompactCNNsCollaborative2021} & 71.59 & 68.81 & -2.78 & 15500 .00 & 7379.52 & 52.39 & 138.40 & 8.37 & 93.95 \\
2.5.1 & 2018 & GDP-Lin~\cite{linAcceleratingConvolutionalNetworks2018} & 70.32 & 69.88 & -0.44 & 15500 .00 & 7500.00 & 51.61 & 138.40 & - & - \\
2.6.2 & 2022 & DAIS~\cite{guanDAISAutomaticChannel2022} & - & - & 1.64 & 15500 .00 & 7750.00 & 50.00 & 138.40 & - & - \\
2.3.2 & 2018 & SSS~\cite{huangDataDrivenSparseStructure2018} & - & 68.53 & - & 15500 .00 & - & - & 138.40 & - & - \\
2.7.1 & 2022 & EarlyCroP~\cite{rachwanWinningLotteryAhead2022} & - & 61.43 & - & 15500 .00 & - & - & 138.40 & 69.20 & 50.00 \\
2.7.2 & 2020 & NM~\cite{kimNeuronMergingCompensating2020} & 73.36 & 61.18 & -12.18 & 15500 .00 & - & - & 138.40 & 85.25 & 38.41 \\
2.7.2 & 2020 & NM~\cite{kimNeuronMergingCompensating2020} & 73.36 & 54.13 & -19.23 & 15500 .00 & - & - & 138.40 & 55.16 & 60.14 \\
2.7.2 & 2020 & NM~\cite{kimNeuronMergingCompensating2020} & 73.36 & 43.99 & -29.37 & 15500 .00 & - & - & 138.40 & 64.19 & 53.62 \\
\bottomrule
\end{tabularx}

\captionof{table}{VGG-11/16 on ImageNet-1K.}
\end{strip}

==> tables/summary.tex <==
\begin{table}[H]
\centering
\begin{tabular}{@{}lccc@{}}
\toprule
Section & \#. methods & \#. models & \#. results \\ \midrule
2.1.1   & 1           & 4          & 7           \\
2.1.2   & 5           & 11         & 30          \\
2.2.1   & 4           & 9          & 53          \\
2.2.2   & 3           & 9          & 30          \\
2.2.3   & 4           & 13         & 36          \\
2.3.1   & 6           & 9          & 44          \\
2.3.2   & 9           & 12         & 72          \\
2.3.3   & 3           & 7          & 26          \\
2.4.1   & 6           & 12         & 62          \\
2.4.2   & 4           & 8          & 18          \\
2.4.3   & 4           & 11         & 19          \\
2.5.1   & 7           & 13         & 71          \\
2.5.2   & 6           & 10         & 39          \\
2.6.1   & 6           & 13         & 51          \\
2.6.2   & 10          & 12         & 94          \\
2.6.3   & 4           & 11         & 46          \\
2.7.1   & 6           & 9          & 33          \\
2.7.2   & 7           & 13         & 41          \\
2.7.3   & 7           & 10         & 35          \\ \midrule
total   & 102         & -          & 807         \\ \bottomrule
\end{tabular}
\captionof{table}{
Summary of collected experiments results for each sub-section.
Note the numbers do not reflect the total number of experiments.
}
\label{tab: summary}
\end{table}
